Stream Members Only: Data-Driven Characterization of Stellar Streams with Mixture Density Networks

Stellar streams are sensitive probes of the Milky Way's gravitational potential. The mean track of a stream constrains global properties of the potential, while its fine-grained surface density constrains galactic substructure. A precise characterization of streams from potentially noisy data marks a crucial step in inferring galactic structure, including the dark matter, across orders of magnitude in mass scales. Here we present a new method for constructing a smooth probability density model of stellar streams using all of the available astrometric and photometric data. To characterize a stream's morphology and kinematics, we utilize mixture density networks to represent its on-sky track, width, stellar number density, and kinematic distribution. We model the photometry for each stream as a single-stellar population, with a distance track that is simultaneously estimated from the stream's inferred distance modulus (using photometry) and parallax distribution (using astrometry). We use normalizing flows to characterize the distribution of background stars. We apply the method to the stream GD-1, and the tidal tails of Palomar 5. For both streams we obtain a catalog of stellar membership probabilities that are made publicly available. Importantly, our model is capable of handling data with incomplete phase-space observations, making our method applicable to the growing census of Milky Way stellar streams. When applied to a population of streams, the resulting membership probabilities from our model form the required input to infer the Milky Way's dark matter distribution from the scale of the stellar halo down to subhalos.

==> listofitems.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "listofitems"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\loiname                 {listofitems}                           %
\def\loiver                      {1.63}                              %
%                                                                    %
\def\loidate                  {2019/08/21}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea, Steven B. Segletes (contributor) %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
%              steven.b.segletes.civ@mail.mil                        %
% Package URL: https://www.ctan.org/pkg/listofitems                  %
% Bug tracker: https://framagit.org/unbonpetit/listofitems/issues    %
% Repository : https://framagit.org/unbonpetit/listofitems/tree/master
% Copyright  : Christian Tellechea 2016-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) listofitems.tex                                    %
%              2) listofitems.sty                                    %
%              3) listofitems-fr.tex                                 %
%              4) listofitems-fr.pdf                                 %
%              5) listofitems-en.tex                                 %
%              6) listofitems-en.pdf                                 %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\expandafter\edef\csname loi_restorecatcode\endcsname{\catcode\number`\_=\number\catcode`\_\relax}
\catcode`\_11

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% gestion des erreurs + annonce package %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\unless\ifdefined\loi_fromsty
	\immediate\write -1 {Package: \loidate\space v\loiver\space Grab items in lists using user-specified sep char (CT)}%
\fi

\ifdefined\PackageError
	\def\loi_error#1{\PackageError\loiname{#1}{Read the \loiname\space manual}}% pour LaTeX
\else
	\def\loi_error#1{\errmessage{Package \loiname\space Error: #1^^J}}% pour TeX
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% verification des prerequis %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_checkprimitive#1#2#3{% Verifie que #1 est une primitive et sinon, emet le message #2 et execute #3
	\begingroup
		\edef\__tempa{\meaning#1}\edef\__tempb{\string#1}\expandafter
	\endgroup
	\ifx\__tempa\__tempb\else
		\loi_error{#2}%
		\def\loi_temp{#3}%
		\loi_restorecatcode\expandafter\loi_temp
	\fi
}
\loi_checkprimitive\eTeXversion
	{You are not using an eTeX engine, listofitems cannot work.}
	{\endinput}%
\loi_checkprimitive\expanded
	{the \string\expanded\space primitive is not provided by your TeX engine, listofitems v\loiver\space cannot work: loading listofitems v1.61}
	{\input listofitemsold.tex\relax\endinput}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macros auxiliaires %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_quark{\loi_quark}
\long\def\loi_identity#1{#1}
\long\def\loi_gobarg#1{}
\long\def\loi_first#1#2{#1}
\long\def\loi_second#1#2{#2}
\long\def\loi_firsttonil#1#2\_nil{#1}
\long\def\loi_antefi#1#2\fi{#2\fi#1}
\long\def\loi_exparg#1#2{\expandafter\loi_exparg_a\expandafter{#2}{#1}}% \loi_exparg{<a>}{<b>} devient <a>{<*b>}
\long\def\loi_exparg_a#1#2{#2{#1}}
\long\def\loi_expafter#1#2{\expandafter\loi_expafter_a\expandafter{#2}{#1}}% \loi_expafter{<a>}{<b>} devient <a><*b>
\long\def\loi_expafter_a#1#2{#2#1}
\def\loi_macroname{\loi_ifinrange\escapechar[[0:255]]{\expandafter\loi_gobarg}{}\string}
\def\loi_argcsname#1#{\loi_argcsname_a{#1}}
\def\loi_argcsname_a#1#2{\loi_expafter{#1}{\csname#2\endcsname}}
\long\def\loi_addtomacro#1#2{\loi_exparg{\def#1}{#1#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macros de test %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifnum#1{\ifnum#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifx#1{\ifx#1\expandafter\loi_first\else\expandafter\loi_second\fi}
\long\def\loi_ifempty#1{\loi_exparg\loi_ifx{\expandafter\relax\detokenize{#1}\relax}}
\def\loi_ifstar#1#2{\def\loi_ifstar_a{\loi_ifx{*\loi_nxttok}{\loi_first{#1}}{#2}}\futurelet\loi_nxttok\loi_ifstar_a}
\edef\loi_escapechar{\expandafter\loi_gobarg\string\\}
\long\def\loi_ifcsexpandable#1{% #1 est-il constitue d'une seule sc _developpable_ ?
	\loi_ifempty{#1}
		{\loi_second
		}
		{\loi_ifspacefirst{#1}
			{\loi_second% si espace en 1er, faux
			}
			{\csname loi_\if\loi_escapechar\expandafter\loi_firsttonil\detokenize{#1}\_nil first\else second\fi\endcsname
				{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul arg commeneant par "\" ?
					{\def\loi_tempa{#1}\loi_exparg{\def\loi_tempb}{#1}% est-il developpable ?
					\expandafter\unless\loi_ifx{\loi_tempa\loi_tempb}%
					}
					{\loi_second
					}%
				}
				{\loi_second
				}%
			}%
		}%
}
\def\loi_ifinrange#1[[#2:#3]]{\expandafter\unless\loi_ifnum{\numexpr(#1-#2)*(#1-#3)>0 }}
\def\loi_ifstring#1#2{% si la chaine #1 est contenue dans #2
	\def\loi_ifstring_a##1#1##2\_nil{\loi_ifempty{##2}\loi_second\loi_first}%
	\loi_ifstring_a#2#1\_nil% appel de la macro auxiliaire
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \loi_foreach %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_cnt_foreach_nest \loi_cnt_foreach_nest=0
\def\end_foreach{\end_foreach}
\def\loi_def_foreachsep#1{%
	\long\def\loi_foreach##1\in##2##3{%
		\global\advance\loi_cnt_foreach_nest1
		\loi_argcsname\def{loop_code_\number\loi_cnt_foreach_nest}{##3}%
		\loi_foreach_a##1##2#1\end_foreach#1%
		\loi_argcsname\let{loop_code_\number\loi_cnt_foreach_nest}\empty
		\global\advance\loi_cnt_foreach_nest-1
	}%
	\long\def\loi_foreach_a##1##2#1{%
		\def##1{##2}%
		\loi_ifx{\end_foreach##1}
			{}
			{\csname loop_code_\number\loi_cnt_foreach_nest\endcsname% execute le code
			\loi_foreach_a##1%
			}%
	}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macros gerant l'appariement %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\defpair#1{%
	\let\loi_listofpair\empty
	\loi_ifempty{#1}
		{}
		{\defpair_a{}#1\loi_quark\loi_quark}%
}
\long\def\defpair_a#1#2#3{%
	\loi_ifx{\loi_quark#2}
		{\def\loi_sanitizelist##1,\_nil{\def\loi_listofpair{##1}}%
		\loi_sanitizelist#1\_nil
		}
		{\loi_if_validpair#2#3%
			{\long\def\loi_paired_a{#2}\long\def\loi_paired_b{#3}%
			\loi_ifx{\loi_paired_a\loi_paired_b}
				{\loi_error{Paired tokens must not be equal, the pair \detokenize{#2#3} is ignored}%
				\defpair_a{#1}%
				}
				{\defpair_a{#1#2#3,}%
				}%
			}
			{\loi_error{Invalid paired tokens, the pair "\detokenize{#2}" and "\detokenize{#3}" is ignored}%
			\defpair_a{#1}%
			}%
		}%
}
\long\def\loi_if_validpair#1#2{%
	\def\loi_validpair{1}%
	\loi_if_invalid_pairtoken{#1}{\def\loi_validpair{0}}%
	\loi_if_invalid_pairtoken{#2}{\def\loi_validpair{0}}%
	\loi_ifnum{\loi_validpair=1 }
}
\long\def\loi_if_invalid_pairtoken#1{%
	\loi_ifempty{#1}
		{\loi_identity
		}
		{\loi_ifspacefirst{#1}
			{\loi_identity
			}
			{\loi_exparg\loi_ifempty{\loi_gobarg#1}% 1 seul token ?
				{\ifcat\relax\noexpand#1\expandafter\loi_identity\else\expandafter\loi_gobarg\fi}
				{\loi_identity}% si plusieurs tokens, faux
			}%
		}%
}
\long\def\loi_count_occur#1\in#2:#3{% compte le nombre d'occurrences de #1 dans #2 et met le resultat dans la macro #3
	\long\def\loi_count_occur_a##1##2#1##3\_nil{%
		\loi_ifempty{##3}
			{\def#3{##1}}
			{\expandafter\loi_count_occur_a\number\numexpr##1+1\relax##3\_nil}%
	}%
	\loi_count_occur_a0#2#1\_nil
}
\long\def\loi_check_pair#1#2\in#3{% teste l'appariement de #1 et #2 dans #3
	\loi_ifempty{#3}
		{\loi_second
		}
		{\loi_count_occur#1\in#3:\loi_tempa
		\loi_count_occur#2\in#3:\loi_tempb
		\loi_ifnum{\loi_tempa=\loi_tempb\relax}%
		}%
}
\long\def\loi_grabpaired_expr#1#2#3#4#5{% #1=liste de paires  #2=expression  #3=separateur   #4=resultat    #5=ce qui reste
	\let#4\empty
	\def\loi_remain{#2#3}%
	\loi_foreach\loi_pair\in{#1}{\expandafter\loi_grabpaired_expr_a\loi_pair{#3}#4}%
	\def\loi_remove_lastsep##1#3\_nil{\def#4{##1}}%
	\expandafter\loi_remove_lastsep#4\_nil
	\loi_expafter{\long\def\loi_grab_remain}#4##1\_nil{%
		\loi_ifempty{##1}
			{\let#5\empty}
			{\loi_exparg{\def#5}{\loi_gobarg##1}}%
	}%
	\loi_grab_remain#2\_nil
}
\long\def\loi_grabpaired_expr_a#1#2#3#4{% #1#2=paire en cours  #3=separateur   #4=resultat
	\loi_exparg{\loi_check_pair#1#2\in}#4% si les paires sont appariees dans le resultat
		{}% passer e la paire suivante
		{\long\def\loi_grabpaired_expr_b##1#3##2\_nil{%
			\loi_addtomacro#4{##1#3}% ajouter au resultat ce qui est jusqu'au prochain separateur
			\def\loi_remain{##2}%
			\loi_exparg{\loi_check_pair#1#2\in}{#4}
				{}
				{\loi_ifempty{##2}
					{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired}}
					{\loi_grabpaired_expr_b##2\_nil}%
				}%
			}%
		\expandafter\loi_grabpaired_expr_b\loi_remain\_nil
		}%
}
\def\insidepair#1#2#3#4{% #1#2=paire  #3=expr  #4=macro reeevant le resultat
	\loi_if_validpair#1#2%
		{\loi_ifcsexpandable{#3}
			{\loi_exparg{\insidepair#1#2}{#3}#4%
			}
			{\loi_check_pair#1#2\in{#3}% si les paires sont appariees dans le resultat
				{\def\insidepair_a##1#1##2\_nil{\insidepair_b##2\_nil{#1}}%
				\def\insidepair_b##1#2##2\_nil##3{%
					\loi_check_pair#1#2\in{##3##1#2}
						{\loi_exparg{\def#4}{\loi_gobarg##3##1}%
						\def\loi_remainafterparen{##2}%
						}%
						{\insidepair_b##2\_nil{##3##1#2}%
						}%
					}%
				\insidepair_a#3\_nil
				}
				{\loi_error{"\detokenize{#1}" and "\detokenize{#2}" are not paired in "#3"}%
				}%
			}%
		}
		{\loi_error{Invalid paired tokens "\detokenize{#1}" and "\detokenize{#2}", empty \string#4 returned}% et bim
		\let#4\empty% voile, bien fait pour vos gueules
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% macro \loi_fornum %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_fornum#1=#2to#3\do{%
	\edef#1{\number\numexpr#2}%
	\expandafter\loi_fornum_a
		\csname loi_fornum_\string#1\expandafter\endcsname\expandafter
		{\number\numexpr#3\expandafter}%
		\expanded{\ifnum#1<\numexpr#3\relax>+\else<-\fi}%
		#1%
}
\long\def\loi_fornum_a#1#2#3#4#5#6{%
	\def#1{%
		\unless\ifnum#5#3#2\relax
			\loi_antefi{#6\edef#5{\number\numexpr#5#41\relax}#1}%
		\fi}%
	#1%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%% macro retirant les espaces extremes %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\long\def\loi_ifspacefirst#1{\expandafter\loi_ifspacefirst_a\detokenize{#10} \_nil}
\long\def\loi_ifspacefirst_a#1 #2\_nil{\loi_ifempty{#1}}
\loi_expafter{\def\loi_gobspace}\space{}
\long\def\loi_removefirstspaces#1{\loi_ifspacefirst{#1}{\loi_exparg\loi_removefirstspaces{\loi_gobspace#1}}{\unexpanded{#1}}}%##BUGFIX v1.63
\begingroup
	\catcode0 12
	\long\gdef\loi_removelastspaces#1{\loi_removelastspaces_a#1^^00 ^^00\_nil}
	\long\gdef\loi_removelastspaces_a#1 ^^00{\loi_removelastspaces_b#1^^00}
	\long\gdef\loi_removelastspaces_b#1^^00#2\_nil{\loi_ifspacefirst{#2}{\loi_removelastspaces_a#1^^00 ^^00\_nil}{\unexpanded{#1}}}
\endgroup
\long\def\loi_removeextremespaces#1{\expanded{\loi_exparg\loi_removelastspaces{\expanded{\loi_removefirstspaces{#1}}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% macro publique \setsepchar %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\setsepchar{\futurelet\loi_nxttok\setsepchar_a}
\def\setsepchar_a{\loi_ifx{[\loi_nxttok}\setsepchar_b{\setsepchar_b[/]}}
\long\def\setsepchar_b[#1]#2{% #1=sepcar de <liste des sepcar>  #2=<liste des sepcar>
	\loi_ifempty{#1}
		{\loi_error{Empty separator not allowed, separator "/" used}%
		\setsepchar_b[/]{#2}%
		}
		{\def\loi_currentsep{#1}%
		\_removeextremespacesfalse
		\loi_nestcnt1 % reinitaliser niveau initial e 1
		\def\nestdepth{1}%
		\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
		\def\loi_listname{loi_listofsep}%
		\let\loi_def\def \let\loi_edef\edef \let\loi_let\let
		\let\loi_listofpair_saved\loi_list_ofpair
		\let\loi_list_ofpair\empty
		\loi_ifempty{#2}
			{\loi_error{Empty list of separators not allowed, "," used}%
			\readlist_g1{,}%
			}
			{\readlist_g1{#2}%
			}%
		\loi_argcsname\let\nestdepth{loi_listofseplen[0]}%
		\loi_argcsname\let\loi_currentsep{loi_listofsep[1]}% 1er car de separation
		\let\loi_listofpair\loi_listofpair_saved
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro normalisant l'index %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\loi_normalizeindex#1#2{% #1=macroname  #2=liste d'index  --> renvoie {err}{indx norm}
	\loi_ifempty{#2}
		{{}{}}
		{\loi_exparg{\loi_normalizeindex_a1{}}{\number\csname#1nest\endcsname}{#1}#2,\loi_quark,}%
}%
\def\loi_normalizeindex_a#1#2#3#4#5,{% #1=compteur de profondeur #2=index precedents  #3=profondeur max #4=macroname  #5=index courant
	\loi_ifx{\loi_quark#5}
		{\loi_normalizeindex_c#2\loi_quark% supprimer la derniere virgule
		}
		{\loi_ifnum{#1>#3 }
			{\loi_invalidindex{Too deeply nested index, index [.] retained}{#2}% si profondeur trop grande
			}
			{\loi_ifinrange\ifnum\numexpr#5<0 -1*\fi(#5)[[1:\csname #4len[#20]\endcsname]]% si abs(#5) hors de [1,len]
				{\loi_exparg\loi_normalizeindex_b{\number\numexpr#5\ifnum\numexpr#5<0 +\csname #4len[#20]\endcsname+1\fi}{#1}{#2}{#3}{#4}}
				{\loi_invalidindex{#5 is an invalid index, index [.] retained}{#2}}%
			}%
		}%
}
\def\loi_normalizeindex_b#1#2#3{\loi_exparg\loi_normalizeindex_a{\number\numexpr#2+1}{#3#1,}}% #1=index e rajouter  #2=compteur de profondeur #3=index precedents
\def\loi_normalizeindex_c#1,\loi_quark{{}{#1}}
\def\loi_invalidindex#1#2{\loi_ifempty{#2}{\loi_invalidindex_a{#1},}\loi_invalidindex_a{#1}{#2}}
\def\loi_invalidindex_a#1#2{\loi_invalidindex_b#1\loi_quark#2\loi_quark}
\def\loi_invalidindex_b#1[.]#2\loi_quark#3,\loi_quark#4\loi_quark,{{#1[#3]#2}{#3}}% #4= index ignores

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%% macro publique \readlist %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcount\loi_nestcnt
\def\greadlist{\let\loi_def\gdef\let\loi_edef\xdef\def\loi_let{\global\let}\readlist_a}%
\def\readlist{\let\loi_def\def\let\loi_edef\edef\let\loi_let\let\readlist_a}
\def\readlist_a{%
	\loi_nestcnt1 % niveau initial = 1
	\loi_argcsname\let{loi_previndex[\number\loi_nestcnt]}\empty
	\loi_ifstar{\_removeextremespacestrue\readlist_b}{\_removeextremespacesfalse\readlist_b}%
}
\long\def\readlist_b#1#2{% #1=macro stockant les elements  #2=liste des elements
	\loi_ifcsexpandable{#2}
		{\loi_exparg{\readlist_b#1}{#2}%
		}
		{\loi_edef\loi_listname{\loi_macroname#1}%
		\loi_exparg{\readlist_c#1{#2}}{\loi_listname}%%
		}%
}
\long\def\readlist_c#1#2#3{% #1=macro stockant les elements  #2=liste des elements #3=macroname
	\loi_argcsname\loi_let{#3nest}\nestdepth
	\loi_argcsname\loi_def{#3[]}{#2}% la liste entiere
	\loi_argcsname\loi_def{#3sep[]}{}% separateur vide
	\loi_ifempty{#2}
		{\loi_def#1[##1]{}%
		\loi_argcsname\loi_def{#3len}{0}\loi_argcsname\loi_def{#3len[0]}{0}%
		\loi_error{Empty list ignored, nothing to do}%
		}
		{\loi_def#1[##1]{\expanded{\expandafter\readlist_d\expanded{\loi_normalizeindex{#3}{##1}}{#3}}}%
		\loi_argcsname\loi_def{#3sep}[##1]{\expanded{\expandafter\readlist_d\expanded{\loi_normalizeindex{#3}{##1}}{#3sep}}}%
		\readlist_e{#2}%
		\loi_argcsname\loi_argcsname\loi_let{#3len}{#3len[0]}% longueur du niveau 0
		}%
}
\def\readlist_d#1#2#3{%
	\unexpanded\expandafter\expandafter\expandafter{\csname#3[#2]\expandafter\endcsname\expandafter}%
	\expanded{\loi_ifempty{#1}{}{\unexpanded{\unexpanded{\loi_error{#1}}}}}%
}
\def\readlist_e{%
	\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
	\expandafter\readlist_f\loi_currentsep||\_nil
}
\long\def\readlist_f#1||#2\_nil#3{\readlist_g1{#3#1}}% #1=<sep courant simple>  #3=liste -> rajoute un element vide pour le test \ifempty ci dessous
\long\def\readlist_g#1#2{% #1=compteur d'index  #2=liste d'elements e examiner terminee par <sep courant simple> >>RIEN laisse apres
	\loi_ifempty{#2}
		{\loi_argcsname\loi_edef{\loi_listname len[\csname loi_previndex[\number\loi_nestcnt]\endcsname0]}{\number\numexpr#1-1\relax}%
		\loi_argcsname\loi_let{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname\number\numexpr#1-1\relax]}\empty% le dernier <sep> est <vide> ##NEW v1.52
		\advance\loi_nestcnt-1
		\loi_argcsname\loi_let\loi_currentsep{loi_listofsep[\number\loi_nestcnt]}%
		}
		{\loi_expafter{\readlist_h{#2}{}}\loi_currentsep||\loi_quark||#2\_nil{#1}% aller isoler le 1er item
		}%
}
\long\def\readlist_h#1#2#3||{% #1=liste restante   #2=<dernier sep utilise>  #3=<sep courant>
	\loi_ifx{\loi_quark#3}% on a epuise tous les <separateurs> ? RESTE e lire <expr+sep1>\_nil{<compteur>}
		{\loi_ifempty{#2}% si #2 vide, aucun <sep utilise> n'a ete trouve, il reste e lire "<liste complete>\_nil"
			{\long\def\readlist_i##1\_nil##2{\loi_exparg{\readlist_j{##2}{}}{\loi_gobarg##1}{#2}}% ##2=compteur d'index
			}
			{\loi_ifx{\loi_listofpair\empty}% paires definies ?
				{\long\def\readlist_i##1#2##2\_nil##3{\loi_exparg{\readlist_j{##3}{##2}}{\loi_gobarg##1}{#2}}%
				}
				{\long\def\readlist_i##1\_nil##2{%
					\loi_exparg{\loi_exparg\loi_grabpaired_expr\loi_listofpair}{\loi_gobarg##1}{#2}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_exparg{\loi_exparg{\readlist_j{##2}}{\loi_grabpaired_remain}}{\loi_grabpaired_result}{#2}}%{#}
				}%
			}%
		\readlist_i\relax% le \relax meuble l'argument delimite
		}
		{\long\def\readlist_i##1#3##2\_nil{%
			\loi_ifempty{##2}% si <liste restante> ne contient pas le <sep courant>
				{\readlist_h{#1}{#2}% recommencer avec le meme <sep utile>
				}%
				{\loi_ifx{\loi_listofpair\empty}% si pas de paires definies
					{\loi_exparg\readlist_h{\loi_gobarg##1#3}{#3}% raccourcir <liste restante> et <sep courant>:=<sep utile>% ##BUGFIX v1.53
					}%
					{\loi_exparg\loi_grabpaired_expr\loi_listofpair{#1#3}{#3}\loi_grabpaired_result\loi_grabpaired_remain
					\loi_ifx{\loi_grabpaired_remain\empty}% si liste non raccourcie #BUGFIX 1.63
						{\loi_exparg\readlist_h{\loi_grabpaired_result}{#2}}% garder le precedent <sep>
						{\loi_exparg\readlist_h{\loi_grabpaired_result}{#3}}%
					}%
				}%
			}%
		\readlist_i\relax#1#3\_nil% ##BUGFIX v1.53
		}%
}
\long\def\readlist_j#1#2#3{% #1=compteur d'index  #2=liste restante  #3=element courant
	\loi_ifnum{0\loi_exparg\loi_ifspacefirst{\loi_currentsep}{}1\if_removeextremespaces1\fi=11 }% s'il faur retirer les espaces extremes
		{\loi_exparg{\loi_exparg{\readlist_k{#1}{#2}}}{\loi_removeextremespaces{#3}}}% redefinir l'element courant
		{\readlist_k{#1}{#2}{#3}}%
}
\long\def\readlist_k#1#2#3#4{% #1=compteur d'index  #2=liste restante  #3=element courant   #4=sep utilise
	\loi_ifnum{0\if_ignoreemptyitems1\fi\loi_ifempty{#3}1{}=11 }
		{\readlist_g{#1}{#2}% si l'on n'ignore pas les elements vides
		}%
		{\loi_argcsname\loi_def{\loi_listname[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#3}% assignation
		\loi_argcsname\loi_def{\loi_listname sep[\csname loi_previndex[\number\loi_nestcnt]\endcsname#1]}{#4}% assignation du <sep> actuel e la macro \<macrolist>sep
		\loi_ifnum{\loi_nestcnt<\nestdepth\relax}% si imbrication max non atteinte
			{\advance\loi_nestcnt1
			\loi_argcsname\edef{loi_previndex[\number\loi_nestcnt]}{\csname loi_previndex[\number\numexpr\loi_nestcnt-1]\endcsname#1,}%
			\readlist_e{#3}% recommencer avec l'element courant
			}
			{}%
		\loi_exparg\readlist_g{\number\numexpr#1+1}{#2}% puis chercher l'element suivant dans la liste restante
		}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% macro \listlen %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\listlen#1[#2]{%
	\expanded{%
		\loi_ifempty{#2}
			{\csname\loi_macroname#1len[0]\endcsname}
			{\loi_exparg\listlen_a{\expanded{\loi_macroname#1}}{#2}}%
	}%
}
\def\listlen_a#1#2{% #1=macro name   #2=index non normalise    prendre <profondeur max-1>
	\expandafter\listlen_b\expanded{\loi_normalizeindex{#1}{#2}}{#1}%
}
\def\listlen_b#1#2#3{% #1=err   #2=index normalise  #3=macroname
	\csname#3len[#2,0]\expandafter\endcsname
	\expanded{\loi_ifempty{#1}{}{\unexpanded{\unexpanded{\loi_error{#1}}}}}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \foreachitem %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\foreachitem#1\in#2{%
	\edef\foreachitem_a{\noexpand\foreachitem_c\noexpand#1{\expandafter\noexpand\csname\loi_macroname#1cnt\endcsname}{\loi_macroname#2}}%
	\futurelet\loi_nxttok\foreachitem_b
}
\def\foreachitem_b{\loi_ifx{\loi_nxttok[}\foreachitem_a{\foreachitem_a[]}}
\def\foreachitem_c#1#2#3[#4]{% prendre <profondeur max-1>
	\expandafter\foreachitem_d\expanded{\loi_normalizeindex{#3}{#4}}#1{#2}{#3}%
}
\def\foreachitem_d#1#2{\loi_ifempty{#2}{\foreachitem_e{#1}{}}{\foreachitem_e{#1}{#2,}}}% #1=err  #2=index norm
\long\def\foreachitem_e#1#2#3#4#5#6{% #1=err  #2=index norm  #3=macroiter  #4=compteur associe  #5=nom de macrolist  #6=code
	\loi_ifnum{\csname#5len[#20]\endcsname>0 }
		{\loi_ifempty{#1}{}{\loi_error{#1}}%
		\loi_fornum#4=1to\csname#5len[#20]\endcsname\do{\loi_argcsname\let#3{#5[#2#4]}#6}%
		}
		{}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%% macro \showitem %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\showitems{\loi_ifstar{\let\showitems_cmd\detokenize\showitems_a}{\let\showitems_cmd\loi_identity\showitems_a}}
\def\showitems_a#1{\def\showitems_b{\showitems_d#1}\futurelet\loi_nxttok\showitems_c}
\def\showitems_c{\loi_ifx{\loi_nxttok[}\showitems_b{\showitems_b[]}}
\def\showitems_d#1[#2]{\foreachitem\showitems_iter\in#1[#2]{\showitemsmacro{\expandafter\showitems_cmd\expandafter{\showitems_iter}}}}
\unless\ifdefined\fbox
	\newdimen\fboxrule \newdimen\fboxsep \fboxrule=.4pt \fboxsep=3pt % reglages identiques e LaTeX
	\def\fbox#1{% imitation de la macro \fbox de LaTeX, voir pages 271 e 274 de "Apprendre e programmer en TeX"
		\hbox{%
			\vrule width\fboxrule
			\vtop{%
				\vbox{\hrule height\fboxrule \kern\fboxsep \hbox{\kern\fboxsep#1\kern\fboxsep}}%
				\kern\fboxsep \hrule height\fboxrule
			}\vrule width\fboxrule
		}%
	}
\fi
\def\showitemsmacro#1{% encadrement par defaut
	\begingroup\fboxsep=0.25pt \fboxrule=0.5pt \fbox{\strut#1}\endgroup
	\hskip0.25em\relax
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% macro \itemtomacro %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemtomacro#1[#2]{% #1[#2]=item  non encore lu: #3=macro
	\edef\loi_listname{\loi_macroname#1}%
	\expandafter\itemtomacro_a\expanded{\loi_normalizeindex{\loi_listname}{#2}}\let
}
\def\gitemtomacro#1[#2]{% #1[#2]=item
	\xdef\loi_listname{\loi_macroname#1}%
	\expandafter\itemtomacro_a\expanded{\loi_normalizeindex{\loi_listname}{#2}}{\global\let}%
}
\def\itemtomacro_a#1#2#3#4{%
	\loi_ifempty{#1}{}{\loi_error{#1}}%
	\loi_argcsname#3#4{\loi_listname[#2]}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% reglages par defaut %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if_removeextremespaces
\newif\if_ignoreemptyitems
\let\ignoreemptyitems\_ignoreemptyitemstrue
\let\reademptyitems\_ignoreemptyitemsfalse
\loi_def_foreachsep{,}
\loi_restorecatcode
\reademptyitems
\setsepchar{,}
\defpair{}
\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%  historique %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
v1.0    19/8/2016
  - Premiere version publique
----------------------------------------------------------------------
v1.1    01/09/2016
  - Stockage des separateurs dans <macrolist>sep
  - bug corrige dans \loi_restorecatcode
----------------------------------------------------------------------
v1.2    22/10/2016
  - macros \greadlist et \gitemtomacro pour la globalite
----------------------------------------------------------------------
v1.3    18/11/2016
  - bugs corriges dans la gestion de la globalite
----------------------------------------------------------------------
v1.4    05/10/2017
  - test \loi_ifprimitive ajoute au test \loi_ifcs
  - suppression de \loi_expafternil, creation de \loi_expafter,
    modification de \loi_argcsname
  - correction d'un bug : \setsepchar{\par} ne provoque plus d'erreur.
    \loi_ifnum devient \long
----------------------------------------------------------------------
v1.5    06/10/2017
  - correction d'un bug dans \loi_ifcs
----------------------------------------------------------------------
v1.51   24/10/2017
  - correction d'un bug dans \loi_ifcs
----------------------------------------------------------------------
v1.52   13/01/2018
  - le dernier separateur est <vide>
----------------------------------------------------------------------
v1.53   13/03/2018
  - correction d'un bug dans \readlist_i
----------------------------------------------------------------------
v1.6    01/11/2018
  - possibilite d'appariement de tokens dans les items
----------------------------------------------------------------------
v1.61   03/03/2019
  - la macro \loi_ifcs contient une erreur de conception. Il faut
    tester si le token est un sc && s'il est developpable pour
    renvoyer vrai car il existe des sc non developpables && qui ne
    sont _pas_ des primitives.
    Macro rebaptisee \loi_ifcsexpandable
----------------------------------------------------------------------
v1.62   18/05/2019
  - utilisation de la nouvelle primitive \expanded au lieu du
    desormais obsolete \romannumeral
  - bug corrige dans \loi_ifcsexpandable
----------------------------------------------------------------------
v1.63   21/08/2019
  - bug corrige dans \readlist_h avec les tokens apparies
  - bug corrige \loi_removefirstspaces est desormais \long


==> output/pal5/member_table_full.tex <==
\begin{table*}
\centering
\small
\addtolength{\tabcolsep}{-1pt}
\newcommand\capitem{\\$\phantom{+}\ast$\ }

\caption{Subset of Membership Table.
\\ This table includes a selection of candidate member stars for the GD-1
stream, based on the membership likelihoods.  For each star we include the Gaia
DR3 source ID and astrometric solution, the Pan-STARRS1 photometry, and the
membership likelihoods for the stream and background. The likelihoods are
computed using the trained model described in \autoref{ssub:trained_pal5} and we
include a quality flag ${\rm dim}(\boldsymbol{x})$, indicating the number of
features used by the model.  For most stars all features are measured. We use
dropout regularization to estimate the uncertainty in the likelihoods, and
report the 5\% and 95\% quantiles of the distribution, as well as the
dropout-disabled maximum-likelihood estimate (MLE) of the likelihood.  For
convenience we round the likelihoods to 2 decimal places, and only show the
value and uncertainty when it is non-zero.\\ \textit{The full table is
available online.}
}
\begin{tabular}{@{}r*{4}{c}*{2}{c}c*{2}{l}@{}}
\toprule
\multicolumn{5}{c}{Gaia} & \multicolumn{2}{c}{PS-1} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{Likelihood (${\rm MLE}_{5\%}^{95\%}$)}\\
\cmidrule(lr){1-5} \cmidrule(lr){6-7} \cmidrule(lr){9-11}
\texttt{source\_id} & $\alpha$ [$\mathrm{{}^{\circ}}$] & $\delta$ [$\mathrm{{}^{\circ}}$] & $\mu_{\alpha}^{*}$ [$\frac{\rm{mas}}{\rm{yr}}$] & $\mu_{\delta}$ [$\frac{\rm{mas}}{\rm{yr}}$] & g [mag] & r [mag] & ${\rm dim}(\boldsymbol{x})$ & $\mathcal{L}_{\rm stream}$ & $\mathcal{L}_{\rm background}$ \\
\midrule
4426379452583612672 & 238.26 & 5.30 & $-2.87 \pm 0.09$ & $-1.97 \pm 0.08$ & $17.69 \pm 0.01$ & $17.13 \pm 0.00$ & 6 & $0.75_{-0.11}^{+0.09}$ & $1.00_{-0.84}^{-0.64}$ \\
4426348528819597440 & 237.79 & 5.06 & $-3.05 \pm 0.41$ & $-1.86 \pm 0.40$ & $19.69 \pm 0.02$ & $19.40 \pm 0.01$ & 6 & $0.77_{-0.10}^{+0.08}$ & $1.00_{-0.85}^{-0.67}$ \\
4424757462474093952 & 236.12 & 4.36 & $-2.93 \pm 0.16$ & $-2.17 \pm 0.13$ & $18.44 \pm 0.01$ & $17.98 \pm 0.00$ & 6 & $0.74_{-0.10}^{+0.10}$ & $1.00_{-0.84}^{-0.64}$ \\
4427116365888010496 & 233.13 & 2.93 & $-3.01 \pm 0.43$ & $-1.71 \pm 0.41$ & $19.67 \pm 0.01$ & $19.32 \pm 0.01$ & 6 & $0.73_{-0.13}^{+0.09}$ & $1.00_{-0.83}^{-0.60}$ \\
4421111898528957312 & 232.53 & 2.66 & $-2.65 \pm 0.34$ & $-2.41 \pm 0.25$ & $19.35 \pm 0.01$ & $19.03 \pm 0.01$ & 6 & $0.75_{-0.11}^{+0.09}$ & $1.00_{-0.85}^{-0.64}$ \\
4420968923362678912 & 232.17 & 2.21 & $-2.36 \pm 0.74$ & $-3.05 \pm 0.76$ & $nan \pm 0.05$ & $nan \pm 0.04$ & 4 & $0.80_{-0.11}^{+0.06}$ & $1.00_{-0.86}^{-0.69}$ \\
4420984939295809024 & 232.03 & 2.29 & $-3.06 \pm 0.23$ & $-2.48 \pm 0.20$ & $18.83 \pm 0.01$ & $18.36 \pm 0.01$ & 6 & $0.72_{-0.15}^{+0.09}$ & $1.00_{-0.81}^{-0.57}$ \\
4420966312022528256 & 232.07 & 2.11 & $-2.70 \pm 0.50$ & $-2.48 \pm 0.47$ & $20.06 \pm 0.02$ & $19.68 \pm 0.01$ & 6 & $0.75_{-0.13}^{+0.07}$ & $1.00_{-0.82}^{-0.62}$ \\
4421172642250281728 & 231.81 & 2.30 & $-2.81 \pm 0.46$ & $-2.43 \pm 0.39$ & $20.16 \pm 0.01$ & $19.75 \pm 0.01$ & 6 & $0.75_{-0.11}^{+0.08}$ & $1.00_{-0.83}^{-0.64}$ \\
4420970057233967360 & 231.88 & 2.02 & $-2.81 \pm 0.17$ & $-2.40 \pm 0.15$ & $18.58 \pm 0.01$ & $18.09 \pm 0.01$ & 6 & $0.87_{-0.08}^{+0.05}$ & $1.00_{-0.91}^{-0.79}$ \\
4420974523999996032 & 231.81 & 2.11 & $-2.38 \pm 0.38$ & $-2.31 \pm 0.33$ & $19.69 \pm 0.02$ & $19.27 \pm 0.01$ & 6 & $0.77_{-0.10}^{+0.07}$ & $1.00_{-0.84}^{-0.67}$ \\
4420974077323374464 & 231.82 & 2.06 & $-2.59 \pm 0.22$ & $-2.57 \pm 0.19$ & $19.05 \pm 0.01$ & $18.62 \pm 0.02$ & 6 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.92}$ \\
4420974798877893504 & 231.75 & 2.09 & $-2.44 \pm 0.46$ & $-2.29 \pm 0.36$ & $19.86 \pm 0.01$ & $19.51 \pm 0.01$ & 6 & $0.78_{-0.11}^{+0.07}$ & $1.00_{-0.85}^{-0.67}$ \\
4421139175865071360 & 231.67 & 2.09 & $-2.80 \pm 0.40$ & $-2.29 \pm 0.32$ & $19.51 \pm 0.01$ & $19.33 \pm 0.01$ & 6 & $0.82_{-0.09}^{+0.06}$ & $1.00_{-0.88}^{-0.73}$ \\
4420948170080600704 & 231.63 & 1.96 & $-2.77 \pm 0.49$ & $-2.17 \pm 0.42$ & $19.98 \pm 0.02$ & $19.60 \pm 0.01$ & 6 & $0.76_{-0.13}^{+0.08}$ & $1.00_{-0.83}^{-0.62}$ \\
4421137904555364992 & 231.50 & 2.03 & $-2.62 \pm 0.36$ & $-2.32 \pm 0.29$ & $19.38 \pm 0.01$ & $18.95 \pm 0.01$ & 6 & $0.84_{-0.09}^{+0.06}$ & $1.00_{-0.90}^{-0.75}$ \\
4421137526598235520 & 231.50 & 2.02 & $-2.95 \pm 0.27$ & $-2.26 \pm 0.25$ & $19.33 \pm 0.01$ & $18.89 \pm 0.01$ & 6 & $0.74_{-0.12}^{+0.08}$ & $1.00_{-0.81}^{-0.62}$ \\
4420942432004721408 & 231.52 & 1.92 & $-2.63 \pm 0.22$ & $-2.69 \pm 0.20$ & $18.83 \pm 0.01$ & $18.37 \pm 0.00$ & 6 & $0.80_{-0.09}^{+0.06}$ & $1.00_{-0.86}^{-0.71}$ \\
4420936384690721280 & 231.62 & 1.76 & $-2.58 \pm 0.21$ & $-2.44 \pm 0.18$ & $18.71 \pm 0.01$ & $18.29 \pm 0.01$ & 6 & $0.82_{-0.11}^{+0.06}$ & $1.00_{-0.88}^{-0.71}$ \\
4421130487147097472 & 231.43 & 1.93 & $-2.89 \pm 0.19$ & $-2.74 \pm 0.16$ & $18.64 \pm 0.01$ & $18.16 \pm 0.01$ & 6 & $0.72_{-0.11}^{+0.09}$ & $1.00_{-0.81}^{-0.61}$ \\
4420934048228488320 & 231.50 & 1.67 & $-2.72 \pm 0.07$ & $-2.61 \pm 0.06$ & $16.95 \pm 0.00$ & $16.34 \pm 0.00$ & 6 & $0.88_{-0.08}^{+0.04}$ & $1.00_{-0.92}^{-0.80}$ \\
4421128077670137472 & 231.36 & 1.85 & $-2.78 \pm 0.29$ & $-2.24 \pm 0.24$ & $19.41 \pm 0.02$ & $18.94 \pm 0.01$ & 6 & $0.85_{-0.09}^{+0.05}$ & $1.00_{-0.90}^{-0.77}$ \\
4421145811590429696 & 231.21 & 2.02 & $-2.78 \pm 0.02$ & $-2.50 \pm 0.02$ & $15.31 \pm 0.00$ & $14.34 \pm 0.00$ & 6 & $0.75_{-0.12}^{+0.08}$ & $1.00_{-0.84}^{-0.63}$ \\
4420752147773103616 & 231.31 & 1.80 & $-2.59 \pm 0.48$ & $-2.89 \pm 0.42$ & $20.07 \pm 0.02$ & $19.65 \pm 0.02$ & 6 & $0.78_{-0.11}^{+0.07}$ & $1.00_{-0.85}^{-0.67}$ \\
4420750739023778432 & 231.10 & 1.72 & $-2.38 \pm 0.22$ & $-2.65 \pm 0.20$ & $18.72 \pm 0.01$ & $18.28 \pm 0.01$ & 6 & $0.79_{-0.10}^{+0.07}$ & $1.00_{-0.86}^{-0.69}$ \\
4420754862192806528 & 231.04 & 1.78 & $-2.34 \pm 0.58$ & $-3.09 \pm 0.58$ & $20.07 \pm 0.01$ & $19.80 \pm 0.01$ & 6 & $0.73_{-0.11}^{+0.09}$ & $1.00_{-0.82}^{-0.62}$ \\
4420755072645928448 & 230.98 & 1.79 & $-2.56 \pm 0.06$ & $-2.85 \pm 0.06$ & $16.77 \pm 0.01$ & $16.38 \pm 0.01$ & 6 & $0.75_{-0.12}^{+0.07}$ & $1.00_{-0.83}^{-0.63}$ \\
4420553479766045824 & 231.07 & 1.56 & $-2.55 \pm 0.29$ & $-2.95 \pm 0.27$ & $19.46 \pm 0.01$ & $19.04 \pm 0.01$ & 6 & $0.82_{-0.09}^{+0.06}$ & $1.00_{-0.88}^{-0.73}$ \\
4420552418908966912 & 231.02 & 1.47 & $-2.75 \pm 0.08$ & $-2.48 \pm 0.08$ & $17.45 \pm 0.00$ & $16.91 \pm 0.00$ & 6 & $0.73_{-0.11}^{+0.08}$ & $1.00_{-0.81}^{-0.62}$ \\
4420740912138482944 & 230.97 & 1.55 & $-2.62 \pm 0.13$ & $-2.73 \pm 0.12$ & $18.16 \pm 0.00$ & $17.66 \pm 0.01$ & 6 & $0.82_{-0.10}^{+0.05}$ & $1.00_{-0.87}^{-0.72}$ \\
4420524445786697344 & 231.05 & 1.37 & $-2.67 \pm 0.09$ & $-2.54 \pm 0.08$ & $17.36 \pm 0.00$ & $16.82 \pm 0.01$ & 6 & $0.90_{-0.06}^{+0.03}$ & $1.00_{-0.93}^{-0.84}$ \\
4420717139494655360 & 230.90 & 1.49 & $-2.51 \pm 0.15$ & $-2.31 \pm 0.14$ & $18.32 \pm 0.01$ & $17.82 \pm 0.01$ & 6 & $0.71_{-0.11}^{+0.10}$ & $1.00_{-0.81}^{-0.60}$ \\
4420721464526574976 & 230.83 & 1.56 & $-2.67 \pm 0.38$ & $-2.35 \pm 0.31$ & $19.35 \pm 0.01$ & $19.02 \pm 0.01$ & 6 & $0.85_{-0.08}^{+0.05}$ & $1.00_{-0.90}^{-0.76}$ \\
4420528568955338112 & 230.90 & 1.42 & $-2.76 \pm 0.19$ & $-2.34 \pm 0.18$ & $18.87 \pm 0.00$ & $18.39 \pm 0.00$ & 6 & $0.72_{-0.11}^{+0.09}$ & $1.00_{-0.81}^{-0.62}$ \\
4420734662961249280 & 230.75 & 1.63 & $-2.64 \pm 0.08$ & $-2.56 \pm 0.07$ & $17.28 \pm 0.00$ & $16.69 \pm 0.00$ & 6 & $0.77_{-0.13}^{+0.07}$ & $1.00_{-0.84}^{-0.64}$ \\
4420512522957298176 & 230.86 & 1.13 & $-2.80 \pm 0.19$ & $-2.47 \pm 0.18$ & $18.75 \pm 0.01$ & $18.23 \pm 0.00$ & 6 & $0.78_{-0.12}^{+0.07}$ & $1.00_{-0.85}^{-0.66}$ \\
4420708888861661440 & 230.63 & 1.35 & $-2.50 \pm 0.14$ & $-2.21 \pm 0.12$ & $18.27 \pm 0.00$ & $17.86 \pm 0.00$ & 6 & $0.74_{-0.12}^{+0.09}$ & $1.00_{-0.83}^{-0.62}$ \\
4420517681213474304 & 230.68 & 1.22 & $-2.68 \pm 0.07$ & $-2.53 \pm 0.06$ & $17.05 \pm 0.00$ & $16.53 \pm 0.00$ & 6 & $0.84_{-0.09}^{+0.06}$ & $1.00_{-0.89}^{-0.75}$ \\
4420711259683622400 & 230.49 & 1.38 & $-2.79 \pm 0.14$ & $-2.55 \pm 0.12$ & $18.22 \pm 0.00$ & $17.71 \pm 0.00$ & 6 & $0.95_{-0.04}^{+0.02}$ & $1.00_{-0.97}^{-0.91}$ \\
4420615396014658432 & 230.44 & 1.23 & $-2.46 \pm 0.35$ & $-2.74 \pm 0.31$ & $19.52 \pm 0.01$ & $19.08 \pm 0.01$ & 6 & $0.88_{-0.08}^{+0.05}$ & $1.00_{-0.92}^{-0.79}$ \\
4420608700160449280 & 230.46 & 1.08 & $-2.78 \pm 0.09$ & $-2.63 \pm 0.08$ & $17.50 \pm 0.01$ & $16.95 \pm 0.00$ & 6 & $0.85_{-0.08}^{+0.05}$ & $1.00_{-0.91}^{-0.77}$ \\
4420608562721387776 & 230.44 & 1.06 & $-2.42 \pm 0.18$ & $-2.61 \pm 0.15$ & $18.57 \pm 0.01$ & $18.10 \pm 0.01$ & 6 & $0.75_{-0.12}^{+0.10}$ & $1.00_{-0.84}^{-0.62}$ \\
4420607768151633408 & 230.21 & 1.13 & $-2.92 \pm 0.16$ & $-2.61 \pm 0.16$ & $18.20 \pm 0.01$ & $17.69 \pm 0.00$ & 6 & $0.69_{-0.12}^{+0.12}$ & $1.00_{-0.81}^{-0.58}$ \\
4420577192280259840 & 230.19 & 0.92 & $-2.78 \pm 0.03$ & $-2.65 \pm 0.03$ & $15.66 \pm 0.00$ & $14.85 \pm 0.00$ & 6 & $0.81_{-0.11}^{+0.08}$ & $1.00_{-0.89}^{-0.70}$ \\
4420385323205469568 & 230.15 & 0.73 & $-2.76 \pm 0.22$ & $-2.42 \pm 0.20$ & $18.98 \pm 0.00$ & $18.52 \pm 0.01$ & 6 & $0.73_{-0.13}^{+0.09}$ & $1.00_{-0.83}^{-0.61}$ \\
4420579460023004800 & 230.01 & 0.92 & $-2.58 \pm 0.08$ & $-2.72 \pm 0.07$ & $17.25 \pm 0.01$ & $16.79 \pm 0.00$ & 6 & $0.96_{-0.02}^{+0.02}$ & $1.00_{-0.98}^{-0.94}$ \\
4420577948194795648 & 230.04 & 0.87 & $-2.97 \pm 0.41$ & $-2.40 \pm 0.33$ & $19.56 \pm 0.01$ & $19.12 \pm 0.01$ & 6 & $0.73_{-0.12}^{+0.09}$ & $1.00_{-0.82}^{-0.61}$ \\
4420376527112384128 & 229.98 & 0.58 & $-2.57 \pm 0.23$ & $-2.67 \pm 0.18$ & $19.01 \pm 0.00$ & $18.74 \pm 0.01$ & 6 & $0.83_{-0.10}^{+0.06}$ & $1.00_{-0.89}^{-0.73}$ \\
4420565677471968384 & 229.87 & 0.65 & $-2.81 \pm 0.38$ & $-2.33 \pm 0.31$ & $19.53 \pm 0.01$ & $19.21 \pm 0.01$ & 6 & $0.78_{-0.10}^{+0.08}$ & $1.00_{-0.86}^{-0.69}$ \\
4419063504070321664 & 229.86 & 0.60 & $-2.68 \pm 0.26$ & $-2.67 \pm 0.22$ & $19.21 \pm 0.01$ & $18.74 \pm 0.00$ & 6 & $0.91_{-0.06}^{+0.04}$ & $1.00_{-0.95}^{-0.85}$ \\
4419064053826136064 & 229.77 & 0.60 & $-2.71 \pm 0.39$ & $-2.26 \pm 0.32$ & $19.61 \pm 0.02$ & $19.35 \pm 0.01$ & 6 & $0.79_{-0.10}^{+0.08}$ & $1.00_{-0.87}^{-0.68}$ \\
4419078145614843776 & 229.61 & 0.64 & $-2.87 \pm 0.30$ & $-2.51 \pm 0.26$ & $19.41 \pm 0.01$ & $18.81 \pm 0.00$ & 6 & $0.73_{-0.14}^{+0.10}$ & $1.00_{-0.83}^{-0.58}$ \\
4419055055870634368 & 229.65 & 0.45 & $-2.70 \pm 0.04$ & $-2.69 \pm 0.03$ & $15.89 \pm 0.00$ & $15.17 \pm 0.00$ & 6 & $0.83_{-0.10}^{+0.06}$ & $1.00_{-0.89}^{-0.73}$ \\
4419058487549267584 & 229.56 & 0.49 & $-2.29 \pm 0.52$ & $-2.98 \pm 0.52$ & $19.84 \pm 0.01$ & $19.42 \pm 0.01$ & 6 & $0.81_{-0.10}^{+0.07}$ & $1.00_{-0.88}^{-0.70}$ \\
4419059797514551168 & 229.52 & 0.55 & $-2.77 \pm 0.07$ & $-2.62 \pm 0.07$ & $17.10 \pm 0.00$ & $16.54 \pm 0.00$ & 6 & $0.76_{-0.11}^{+0.10}$ & $1.00_{-0.86}^{-0.65}$ \\
4419028250978701952 & 229.51 & 0.30 & $-2.76 \pm 0.29$ & $-2.46 \pm 0.29$ & $19.17 \pm 0.01$ & $18.72 \pm 0.02$ & 6 & $0.79_{-0.11}^{+0.08}$ & $1.00_{-0.87}^{-0.68}$ \\
4419027804302099712 & 229.48 & 0.27 & $-2.75 \pm 0.53$ & $-2.45 \pm 0.54$ & $19.98 \pm 0.01$ & $19.66 \pm 0.02$ & 6 & $0.77_{-0.12}^{+0.07}$ & $1.00_{-0.84}^{-0.65}$ \\
4419025300337195264 & 229.39 & 0.17 & $-2.75 \pm 0.10$ & $-2.59 \pm 0.08$ & $17.44 \pm 0.00$ & $16.88 \pm 0.00$ & 6 & $0.87_{-0.07}^{+0.06}$ & $1.00_{-0.93}^{-0.80}$ \\
4419023234457620352 & 229.24 & 0.20 & $-2.69 \pm 0.14$ & $-2.41 \pm 0.11$ & $18.20 \pm 0.01$ & $17.74 \pm 0.00$ & 6 & $0.83_{-0.09}^{+0.06}$ & $1.00_{-0.90}^{-0.74}$ \\
4418926855391616000 & 229.07 & 0.06 & $-2.60 \pm 0.30$ & $-2.81 \pm 0.24$ & $19.37 \pm 0.02$ & $18.94 \pm 0.01$ & 6 & $0.95_{-0.07}^{+0.04}$ & $1.00_{-0.99}^{-0.87}$ \\
4418926477434478080 & 229.07 & 0.04 & $-1.65 \pm 0.57$ & $-2.68 \pm 0.42$ & $20.12 \pm 0.02$ & $19.71 \pm 0.01$ & 6 & $0.61_{-0.29}^{+0.20}$ & $1.00_{-0.82}^{-0.32}$ \\
4418926374355250432 & 229.07 & 0.03 & $-2.50 \pm 0.67$ & $-2.50 \pm 0.54$ & $19.94 \pm 0.02$ & $19.63 \pm 0.01$ & 6 & $0.93_{-0.16}^{+0.05}$ & $1.00_{-0.97}^{-0.76}$ \\
4418928165356912000 & 229.02 & 0.09 & $-2.72 \pm 0.04$ & $-2.66 \pm 0.03$ & $16.11 \pm 0.00$ & $15.51 \pm 0.00$ & 6 & $0.88_{-0.16}^{+0.07}$ & $1.00_{-0.95}^{-0.72}$ \\
4418923007100469760 & 229.08 & -0.02 & $-2.65 \pm 0.11$ & $-2.62 \pm 0.09$ & $17.77 \pm 0.00$ & $17.30 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920361400550912 & 229.12 & -0.07 & $-2.69 \pm 0.96$ & $-2.85 \pm 0.75$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.94_{-0.07}^{+0.03}$ & $1.00_{-0.97}^{-0.87}$ \\
4418926339995504512 & 229.05 & 0.03 & $-1.12 \pm 0.89$ & $-2.68 \pm 0.76$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.78_{-0.19}^{+0.08}$ & $1.00_{-0.86}^{-0.59}$ \\
4418732207473429632 & 229.14 & -0.12 & $-1.57 \pm 0.89$ & $-1.38 \pm 0.75$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.79_{-0.15}^{+0.07}$ & $1.00_{-0.87}^{-0.64}$ \\
4418920636278474880 & 229.10 & -0.06 & $-2.70 \pm 0.11$ & $-2.71 \pm 0.09$ & $17.78 \pm 0.01$ & $17.26 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418921529631708416 & 229.07 & -0.03 & $-1.62 \pm 0.56$ & $-2.43 \pm 0.43$ & $19.90 \pm 0.04$ & $19.45 \pm 0.01$ & 6 & $0.92_{-0.07}^{+0.03}$ & $1.00_{-0.95}^{-0.85}$ \\
4418920331336673024 & 229.11 & -0.08 & $-3.45 \pm 0.84$ & $-2.19 \pm 0.72$ & $nan \pm 0.04$ & $nan \pm 0.01$ & 4 & $0.94_{-0.05}^{+0.02}$ & $1.00_{-0.96}^{-0.88}$ \\
4418926236916260736 & 229.05 & 0.01 & $-2.86 \pm 1.01$ & $-2.64 \pm 0.84$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.94_{-0.04}^{+0.02}$ & $1.00_{-0.96}^{-0.90}$ \\
4418921529631707136 & 229.07 & -0.03 & $-2.17 \pm 0.45$ & $-2.17 \pm 0.38$ & $19.66 \pm 0.04$ & $19.35 \pm 0.01$ & 6 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418921735790148864 & 229.06 & -0.02 & $-2.43 \pm 0.47$ & $-2.68 \pm 0.39$ & $19.81 \pm 0.02$ & $19.35 \pm 0.01$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418921426552475392 & 229.07 & -0.04 & $-3.38 \pm 1.51$ & $-1.03 \pm 1.36$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418926511794191232 & 229.03 & 0.02 & $-2.54 \pm 0.64$ & $-1.73 \pm 0.50$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.92_{-0.05}^{+0.03}$ & $1.00_{-0.94}^{-0.87}$ \\
4418921529631697152 & 229.06 & -0.04 & $-1.49 \pm 1.16$ & $-2.08 \pm 0.95$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.93_{-0.04}^{+0.02}$ & $1.00_{-0.95}^{-0.89}$ \\
4418732551070815360 & 229.11 & -0.11 & $-3.37 \pm 0.68$ & $-2.29 \pm 0.60$ & $20.07 \pm 0.01$ & $19.71 \pm 0.01$ & 6 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.91}$ \\
4418921426552478336 & 229.06 & -0.04 & $-1.30 \pm 0.86$ & $-3.04 \pm 0.75$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.92_{-0.04}^{+0.03}$ & $1.00_{-0.95}^{-0.88}$ \\
4418730764364400512 & 229.15 & -0.18 & $-2.65 \pm 0.92$ & $-1.57 \pm 0.77$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.74_{-0.11}^{+0.08}$ & $1.00_{-0.82}^{-0.63}$ \\
4418921495271963136 & 229.06 & -0.03 & $-2.82 \pm 0.17$ & $-2.74 \pm 0.15$ & $18.37 \pm 0.01$ & $17.93 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418732177408528512 & 229.13 & -0.14 & $-3.25 \pm 1.11$ & $-3.53 \pm 0.93$ & $nan \pm 0.04$ & $nan \pm 0.05$ & 4 & $0.83_{-0.08}^{+0.05}$ & $1.00_{-0.89}^{-0.76}$ \\
4418927649960836352 & 228.98 & 0.07 & $-2.38 \pm 0.27$ & $-2.28 \pm 0.24$ & $19.28 \pm 0.02$ & $18.82 \pm 0.01$ & 6 & $0.86_{-0.06}^{+0.05}$ & $1.00_{-0.91}^{-0.80}$ \\
4418920189601805824 & 229.09 & -0.10 & $-2.40 \pm 1.02$ & $-1.54 \pm 0.91$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.93}$ \\
4418920189601804544 & 229.09 & -0.11 & $-2.07 \pm 0.65$ & $-2.78 \pm 0.53$ & $20.11 \pm 0.02$ & $19.76 \pm 0.02$ & 6 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418920567558981760 & 229.07 & -0.07 & $-1.67 \pm 0.74$ & $-2.71 \pm 0.71$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.96_{-0.02}^{+0.02}$ & $1.00_{-0.97}^{-0.93}$ \\
4418920189601820928 & 229.08 & -0.10 & $-3.06 \pm 0.61$ & $-1.06 \pm 0.51$ & $20.14 \pm 0.02$ & $19.77 \pm 0.02$ & 6 & $0.76_{-0.10}^{+0.08}$ & $1.00_{-0.85}^{-0.66}$ \\
4418920258323013504 & 229.08 & -0.10 & $-2.06 \pm 1.01$ & $-3.20 \pm 0.84$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418920498839492736 & 229.07 & -0.08 & $-3.44 \pm 0.68$ & $-1.42 \pm 0.65$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418921392192734592 & 229.05 & -0.05 & $-2.86 \pm 0.35$ & $-2.55 \pm 0.30$ & $19.21 \pm 0.01$ & $18.83 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418731799452216064 & 229.11 & -0.15 & $-2.82 \pm 1.94$ & $-1.68 \pm 1.24$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.91_{-0.05}^{+0.03}$ & $1.00_{-0.94}^{-0.86}$ \\
4418921392194337152 & 229.05 & -0.05 & $-2.21 \pm 0.55$ & $-2.45 \pm 0.52$ & $19.87 \pm 0.02$ & $19.54 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418921701430402560 & 229.03 & -0.03 & $-2.77 \pm 0.57$ & $-1.92 \pm 0.51$ & $19.92 \pm 0.01$ & $19.55 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418921323473240192 & 229.05 & -0.06 & $-3.50 \pm 0.69$ & $-1.44 \pm 0.65$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418920567558985472 & 229.06 & -0.07 & $-1.84 \pm 0.43$ & $-2.82 \pm 0.38$ & $19.72 \pm 0.01$ & $19.30 \pm 0.01$ & 6 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418920189601803008 & 229.08 & -0.11 & $-3.16 \pm 0.84$ & $-2.37 \pm 0.62$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.02}^{+0.01}$ & $1.00_{-0.99}^{-0.96}$ \\
4418925858959184128 & 228.98 & 0.04 & $-2.87 \pm 0.10$ & $-2.70 \pm 0.08$ & $17.63 \pm 0.00$ & $17.11 \pm 0.00$ & 6 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418921396488436352 & 229.04 & -0.04 & $-2.69 \pm 0.06$ & $-2.68 \pm 0.05$ & $16.52 \pm 0.00$ & $15.97 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418732138753953920 & 229.09 & -0.12 & $-2.76 \pm 0.67$ & $-2.36 \pm 0.53$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418926138132347008 & 228.97 & 0.06 & $-2.66 \pm 0.05$ & $-2.74 \pm 0.04$ & $16.24 \pm 0.00$ & $15.56 \pm 0.00$ & 6 & $0.96_{-0.03}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418920258321297792 & 229.07 & -0.10 & $-3.02 \pm 0.66$ & $-2.09 \pm 0.60$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418732070034473856 & 229.09 & -0.13 & $-1.68 \pm 1.73$ & $-2.74 \pm 1.11$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.92}$ \\
4418919811644676480 & 229.08 & -0.11 & $-2.50 \pm 0.76$ & $-2.44 \pm 0.61$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418731829516302848 & 229.10 & -0.14 & $-2.73 \pm 0.11$ & $-2.54 \pm 0.09$ & $17.42 \pm 0.01$ & $17.05 \pm 0.04$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418732143049556096 & 229.09 & -0.13 & $-2.74 \pm 0.16$ & $-2.56 \pm 0.13$ & $18.12 \pm 0.00$ & $17.63 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418921598351163008 & 229.03 & -0.05 & $-2.43 \pm 0.35$ & $-2.04 \pm 0.32$ & $19.39 \pm 0.02$ & $18.98 \pm 0.01$ & 6 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.92}$ \\
4418925068685178368 & 228.98 & 0.02 & $-2.88 \pm 0.36$ & $-2.39 \pm 0.30$ & $19.47 \pm 0.01$ & $19.07 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418919880364162048 & 229.07 & -0.10 & $-1.54 \pm 0.82$ & $-2.52 \pm 0.73$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418921289115106048 & 229.04 & -0.07 & $-2.85 \pm 0.80$ & $-1.24 \pm 0.77$ & $nan \pm 0.07$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418920155242104064 & 229.05 & -0.08 & $-1.28 \pm 0.64$ & $-3.15 \pm 0.62$ & $20.10 \pm 0.02$ & $19.72 \pm 0.01$ & 6 & $0.90_{-0.05}^{+0.03}$ & $1.00_{-0.94}^{-0.85}$ \\
4418921667070659840 & 229.02 & -0.03 & $-3.10 \pm 0.87$ & $-3.47 \pm 0.81$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418921289115105792 & 229.04 & -0.07 & $-2.04 \pm 0.58$ & $-2.63 \pm 0.53$ & $19.99 \pm 0.02$ & $19.69 \pm 0.01$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.99}$ \\
4418920533199234048 & 229.05 & -0.08 & $-2.36 \pm 0.76$ & $-2.86 \pm 0.66$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418919880365871232 & 229.07 & -0.11 & $-3.82 \pm 1.62$ & $-2.67 \pm 1.13$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920086522610048 & 229.05 & -0.09 & $-2.76 \pm 0.87$ & $-2.90 \pm 0.68$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.99}$ \\
4418919777284924416 & 229.07 & -0.12 & $-3.26 \pm 0.80$ & $-2.86 \pm 0.57$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418732104394214272 & 229.07 & -0.12 & $-2.95 \pm 0.22$ & $-2.62 \pm 0.17$ & $18.44 \pm 0.01$ & $17.96 \pm 0.00$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418920086522602880 & 229.06 & -0.10 & $-2.09 \pm 0.82$ & $-1.80 \pm 0.72$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418732039970339968 & 229.09 & -0.15 & $-2.67 \pm 0.04$ & $-2.66 \pm 0.03$ & $15.88 \pm 0.00$ & $15.11 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418921357832971264 & 229.03 & -0.06 & $-2.76 \pm 0.81$ & $-2.11 \pm 0.72$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.99}$ \\
4418921632710914432 & 229.01 & -0.04 & $-2.38 \pm 0.39$ & $-2.96 \pm 0.30$ & $19.41 \pm 0.01$ & $18.94 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418732104394212864 & 229.08 & -0.13 & $-1.89 \pm 0.50$ & $-2.76 \pm 0.41$ & $19.82 \pm 0.01$ & $19.42 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418731932595515136 & 229.09 & -0.15 & $-2.18 \pm 0.71$ & $-1.30 \pm 0.64$ & $19.90 \pm 0.02$ & $19.75 \pm 0.03$ & 6 & $0.94_{-0.04}^{+0.02}$ & $1.00_{-0.96}^{-0.90}$ \\
4418732035674733312 & 229.08 & -0.14 & $-2.72 \pm 0.24$ & $-2.76 \pm 0.20$ & $18.88 \pm 0.01$ & $18.40 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418925897613485952 & 228.96 & 0.03 & $-2.64 \pm 1.72$ & $-2.56 \pm 1.70$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.88_{-0.06}^{+0.03}$ & $1.00_{-0.90}^{-0.81}$ \\
4418920155242103168 & 229.04 & -0.08 & $-3.66 \pm 0.71$ & $-3.28 \pm 0.63$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418730523846217088 & 229.13 & -0.22 & $-2.01 \pm 0.65$ & $-2.64 \pm 0.58$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.90_{-0.05}^{+0.02}$ & $1.00_{-0.92}^{-0.85}$ \\
4418732104394210176 & 229.08 & -0.14 & $-2.14 \pm 0.86$ & $-1.96 \pm 0.71$ & $nan \pm 0.04$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418919777284925312 & 229.06 & -0.12 & $-3.40 \pm 0.99$ & $-2.98 \pm 0.79$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418925790239694464 & 228.96 & 0.03 & $-2.54 \pm 0.67$ & $-1.94 \pm 0.60$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.94_{-0.03}^{+0.01}$ & $1.00_{-0.96}^{-0.91}$ \\
4418919777284907392 & 229.07 & -0.13 & $-2.34 \pm 0.88$ & $-2.44 \pm 0.74$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919846004412032 & 229.05 & -0.11 & $-1.89 \pm 0.63$ & $-2.35 \pm 0.54$ & $19.95 \pm 0.01$ & $19.61 \pm 0.01$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.99}$ \\
4418919777284923904 & 229.06 & -0.12 & $-2.02 \pm 1.23$ & $-3.91 \pm 1.11$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.96}$ \\
4418730867443614336 & 229.10 & -0.18 & $-2.86 \pm 0.75$ & $-2.56 \pm 0.71$ & $20.14 \pm 0.02$ & $19.75 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418924901181758976 & 228.98 & -0.00 & $-2.58 \pm 0.11$ & $-2.41 \pm 0.09$ & $17.34 \pm 0.00$ & $17.00 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920159537849856 & 229.04 & -0.09 & $-2.76 \pm 0.11$ & $-2.58 \pm 0.10$ & $17.79 \pm 0.00$ & $17.31 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920911156358272 & 229.03 & -0.07 & $-2.51 \pm 1.41$ & $-3.19 \pm 1.03$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418925721520200960 & 228.96 & 0.02 & $-3.96 \pm 1.00$ & $-1.53 \pm 0.80$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.93_{-0.03}^{+0.01}$ & $1.00_{-0.94}^{-0.90}$ \\
4418920911157949824 & 229.02 & -0.07 & $-2.99 \pm 1.54$ & $-3.13 \pm 1.14$ & $nan \pm 0.04$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418921190330132736 & 229.01 & -0.06 & $-2.13 \pm 1.01$ & $-2.61 \pm 1.01$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920911156358400 & 229.02 & -0.07 & $-1.68 \pm 1.27$ & $-1.36 \pm 1.01$ & $nan \pm 0.05$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920052162847488 & 229.05 & -0.11 & $-2.65 \pm 0.88$ & $-3.36 \pm 0.76$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919846004398720 & 229.05 & -0.12 & $-3.60 \pm 1.28$ & $-2.86 \pm 0.91$ & $nan \pm 0.04$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920120882353280 & 229.03 & -0.09 & $-2.58 \pm 0.21$ & $-2.32 \pm 0.19$ & $18.69 \pm 0.00$ & $18.22 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920056458766720 & 229.04 & -0.11 & $-2.93 \pm 1.33$ & $-1.92 \pm 1.55$ & $nan \pm 0.03$ & $nan \pm 0.04$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418731932595516160 & 229.07 & -0.15 & $-2.20 \pm 0.41$ & $-2.38 \pm 0.34$ & $19.49 \pm 0.01$ & $19.15 \pm 0.04$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418919846004412160 & 229.05 & -0.11 & $-3.32 \pm 0.49$ & $-2.75 \pm 0.40$ & $19.80 \pm 0.02$ & $19.36 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418919846004406016 & 229.05 & -0.11 & $-1.70 \pm 1.23$ & $-3.00 \pm 1.06$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919674207428224 & 229.06 & -0.13 & $-2.26 \pm 1.95$ & $-2.61 \pm 1.21$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418919674205691648 & 229.06 & -0.13 & $-3.87 \pm 0.81$ & $-3.31 \pm 0.67$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919674205695488 & 229.05 & -0.13 & $-2.65 \pm 0.24$ & $-2.28 \pm 0.18$ & $18.76 \pm 0.01$ & $18.28 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919674205687424 & 229.06 & -0.13 & $-2.70 \pm 1.08$ & $-1.54 \pm 1.02$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919846004410624 & 229.04 & -0.11 & $-3.99 \pm 1.38$ & $-1.38 \pm 1.26$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418731623357859584 & 229.09 & -0.18 & $-3.88 \pm 0.66$ & $-3.47 \pm 0.56$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.90_{-0.04}^{+0.02}$ & $1.00_{-0.92}^{-0.86}$ \\
4418924656367908992 & 228.98 & -0.02 & $-2.06 \pm 0.80$ & $-2.60 \pm 0.70$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418919949083630080 & 229.04 & -0.11 & $-2.70 \pm 0.22$ & $-2.53 \pm 0.20$ & $18.91 \pm 0.01$ & $18.44 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418721384155802752 & 229.14 & -0.26 & $-2.56 \pm 0.50$ & $-3.09 \pm 0.44$ & $20.08 \pm 0.01$ & $19.67 \pm 0.01$ & 6 & $0.89_{-0.04}^{+0.02}$ & $1.00_{-0.91}^{-0.85}$ \\
4418920881092357120 & 229.02 & -0.08 & $-2.93 \pm 0.23$ & $-2.52 \pm 0.20$ & $18.23 \pm 0.01$ & $17.81 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919949085305216 & 229.04 & -0.11 & $-3.75 \pm 0.62$ & $-3.10 \pm 0.54$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920945516097280 & 229.02 & -0.07 & $-2.54 \pm 0.97$ & $-2.09 \pm 0.91$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919674205685376 & 229.05 & -0.13 & $-2.56 \pm 0.93$ & $-2.10 \pm 0.81$ & $nan \pm 0.02$ & $nan \pm 0.04$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919953379416192 & 229.04 & -0.11 & $-2.83 \pm 0.30$ & $-2.33 \pm 0.26$ & $19.25 \pm 0.01$ & $18.80 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919949083637376 & 229.03 & -0.10 & $-2.83 \pm 0.85$ & $-2.13 \pm 0.71$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920120882335872 & 229.03 & -0.10 & $-1.91 \pm 0.76$ & $-2.61 \pm 0.69$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919949083633280 & 229.04 & -0.11 & $-2.54 \pm 0.42$ & $-2.07 \pm 0.38$ & $19.61 \pm 0.02$ & $19.19 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418731898235776000 & 229.06 & -0.15 & $-3.59 \pm 1.16$ & $-2.58 \pm 1.00$ & $nan \pm 0.05$ & $nan \pm 0.05$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418731692078914688 & 229.07 & -0.17 & $-2.88 \pm 0.22$ & $-2.73 \pm 0.19$ & $18.37 \pm 0.01$ & $17.85 \pm 0.02$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731902531386240 & 229.07 & -0.16 & $-2.74 \pm 0.06$ & $-2.70 \pm 0.05$ & $16.48 \pm 0.00$ & $15.81 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731966955254144 & 229.06 & -0.15 & $-1.86 \pm 1.17$ & $-3.41 \pm 0.98$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418919953379726720 & 229.03 & -0.11 & $-3.05 \pm 0.73$ & $-3.24 \pm 0.70$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919949084019840 & 229.04 & -0.12 & $-3.52 \pm 0.84$ & $-2.52 \pm 0.69$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919742925173888 & 229.04 & -0.13 & $-3.46 \pm 0.67$ & $-2.31 \pm 0.57$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920017803126528 & 229.02 & -0.10 & $-2.07 \pm 0.18$ & $-2.37 \pm 0.15$ & $18.53 \pm 0.01$ & $18.08 \pm 0.01$ & 6 & $0.85_{-0.05}^{+0.03}$ & $1.00_{-0.88}^{-0.80}$ \\
4418920945516089472 & 229.01 & -0.08 & $-2.37 \pm 0.22$ & $-2.74 \pm 0.19$ & $18.78 \pm 0.01$ & $18.34 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919949083928960 & 229.03 & -0.11 & $-2.57 \pm 1.40$ & $-3.06 \pm 1.25$ & $nan \pm 0.08$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418731898235774720 & 229.07 & -0.16 & $-3.15 \pm 0.43$ & $-3.10 \pm 0.35$ & $19.49 \pm 0.03$ & $19.05 \pm 0.00$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920881091801984 & 229.02 & -0.08 & $-2.43 \pm 1.42$ & $-1.30 \pm 1.32$ & $nan \pm 0.04$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418731902530624512 & 229.06 & -0.16 & $-2.25 \pm 1.73$ & $-3.75 \pm 1.26$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418921254753776512 & 228.99 & -0.05 & $-3.03 \pm 0.62$ & $-1.64 \pm 0.46$ & $19.89 \pm 0.02$ & $19.50 \pm 0.01$ & 6 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.94}$ \\
4418919949083634816 & 229.03 & -0.11 & $-1.76 \pm 0.97$ & $-1.19 \pm 0.75$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919742925176704 & 229.04 & -0.12 & $-2.45 \pm 0.68$ & $-3.97 \pm 0.59$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418921151674544256 & 229.00 & -0.06 & $-2.59 \pm 0.46$ & $-2.44 \pm 0.40$ & $19.52 \pm 0.04$ & $19.17 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418724923208864128 & 229.10 & -0.21 & $-2.81 \pm 0.30$ & $-2.88 \pm 0.27$ & $19.38 \pm 0.01$ & $18.93 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920945516098816 & 229.00 & -0.07 & $-2.17 \pm 0.54$ & $-2.67 \pm 0.44$ & $19.75 \pm 0.02$ & $19.47 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418921220394038272 & 228.99 & -0.05 & $-2.32 \pm 0.46$ & $-3.06 \pm 0.37$ & $19.83 \pm 0.02$ & $19.39 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919953379417344 & 229.03 & -0.11 & $-2.60 \pm 0.11$ & $-2.57 \pm 0.10$ & $17.75 \pm 0.00$ & $17.32 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920017803410688 & 229.02 & -0.10 & $-2.88 \pm 0.58$ & $-2.79 \pm 0.54$ & $20.11 \pm 0.01$ & $19.70 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731902531386112 & 229.06 & -0.16 & $-2.81 \pm 0.23$ & $-2.50 \pm 0.19$ & $18.80 \pm 0.01$ & $18.37 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920017803127040 & 229.02 & -0.10 & $-2.19 \pm 0.86$ & $-2.38 \pm 0.70$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919639845948288 & 229.04 & -0.13 & $-2.58 \pm 0.46$ & $-3.00 \pm 0.34$ & $19.56 \pm 0.01$ & $19.16 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731902531386752 & 229.06 & -0.16 & $-2.88 \pm 0.08$ & $-2.62 \pm 0.06$ & $16.92 \pm 0.00$ & $16.31 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919708565437440 & 229.03 & -0.12 & $-2.68 \pm 0.80$ & $-2.49 \pm 0.76$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418724991928344448 & 229.09 & -0.20 & $-1.78 \pm 0.55$ & $-2.39 \pm 0.48$ & $19.97 \pm 0.02$ & $19.66 \pm 0.04$ & 6 & $0.94_{-0.02}^{+0.01}$ & $1.00_{-0.95}^{-0.92}$ \\
4418921220394032512 & 228.99 & -0.05 & $-2.52 \pm 0.23$ & $-2.44 \pm 0.17$ & $18.71 \pm 0.01$ & $18.26 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920778013142144 & 229.01 & -0.09 & $-2.74 \pm 0.14$ & $-2.77 \pm 0.11$ & $17.92 \pm 0.00$ & $17.42 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418724888849127552 & 229.09 & -0.21 & $-2.29 \pm 1.12$ & $-2.86 \pm 1.00$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418919639845933568 & 229.05 & -0.14 & $-2.77 \pm 0.19$ & $-2.36 \pm 0.16$ & $18.48 \pm 0.01$ & $18.00 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919712861244416 & 229.03 & -0.13 & $-2.82 \pm 0.09$ & $-2.66 \pm 0.08$ & $17.38 \pm 0.00$ & $16.83 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731966955254016 & 229.05 & -0.15 & $-3.30 \pm 1.12$ & $-2.86 \pm 1.05$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919639845948928 & 229.04 & -0.13 & $-2.81 \pm 0.46$ & $-3.16 \pm 0.33$ & $19.59 \pm 0.01$ & $19.18 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919953379415808 & 229.03 & -0.12 & $-2.80 \pm 0.05$ & $-2.69 \pm 0.05$ & $16.52 \pm 0.00$ & $15.89 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919919019128960 & 229.03 & -0.12 & $-3.17 \pm 0.95$ & $-1.96 \pm 0.96$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920017803112832 & 229.02 & -0.11 & $-2.87 \pm 0.14$ & $-2.55 \pm 0.12$ & $18.03 \pm 0.00$ & $17.53 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919949085276544 & 229.02 & -0.11 & $-2.30 \pm 0.65$ & $-2.05 \pm 0.61$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920773717375872 & 229.01 & -0.09 & $-2.25 \pm 0.33$ & $-2.83 \pm 0.28$ & $19.37 \pm 0.01$ & $18.96 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919644141222400 & 229.04 & -0.14 & $-3.18 \pm 2.08$ & $-3.50 \pm 1.47$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919919019129216 & 229.03 & -0.12 & $-2.75 \pm 1.26$ & $-2.68 \pm 0.99$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919708565435648 & 229.03 & -0.13 & $-1.52 \pm 0.86$ & $-3.60 \pm 0.73$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418921151674532608 & 228.99 & -0.07 & $-3.15 \pm 0.55$ & $-2.57 \pm 0.48$ & $19.86 \pm 0.02$ & $19.59 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418920842438432256 & 229.00 & -0.09 & $-2.30 \pm 0.59$ & $-2.81 \pm 0.51$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418919712861243264 & 229.04 & -0.13 & $-2.76 \pm 0.04$ & $-2.64 \pm 0.04$ & $16.09 \pm 0.00$ & $15.38 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418925313498622080 & 228.94 & 0.01 & $-2.70 \pm 0.11$ & $-2.72 \pm 0.09$ & $17.75 \pm 0.00$ & $17.32 \pm 0.00$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418731966955253632 & 229.04 & -0.15 & $-2.24 \pm 1.13$ & $-3.31 \pm 0.98$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418726091439988224 & 229.05 & -0.16 & $-2.87 \pm 0.54$ & $-1.69 \pm 0.45$ & $19.75 \pm 0.01$ & $19.58 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418731971250102784 & 229.04 & -0.15 & $-2.15 \pm 1.29$ & $-2.81 \pm 1.02$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418725713482851968 & 229.08 & -0.20 & $-3.72 \pm 0.56$ & $-2.77 \pm 0.48$ & $20.03 \pm 0.02$ & $19.54 \pm 0.01$ & 6 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.94}$ \\
4418920842436859520 & 229.00 & -0.09 & $-1.70 \pm 0.67$ & $-3.04 \pm 0.61$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919639845925504 & 229.04 & -0.15 & $-2.34 \pm 0.95$ & $-2.73 \pm 0.76$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920773718952832 & 229.00 & -0.09 & $-2.82 \pm 1.56$ & $-3.29 \pm 1.43$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919708567119488 & 229.03 & -0.13 & $-1.43 \pm 1.18$ & $-2.77 \pm 0.84$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919914723871488 & 229.03 & -0.12 & $-3.71 \pm 0.94$ & $-3.46 \pm 0.77$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920842436874496 & 229.00 & -0.08 & $-2.49 \pm 1.07$ & $-3.01 \pm 0.99$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920842436863744 & 229.00 & -0.09 & $-3.13 \pm 0.24$ & $-2.39 \pm 0.21$ & $18.84 \pm 0.01$ & $18.40 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418920842438420352 & 229.00 & -0.09 & $-3.28 \pm 0.74$ & $-3.66 \pm 0.68$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913764332401792 & 229.04 & -0.15 & $-2.03 \pm 0.63$ & $-3.45 \pm 0.51$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919712860699520 & 229.03 & -0.13 & $-2.22 \pm 1.95$ & $-1.44 \pm 1.35$ & $nan \pm 0.04$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418721487235015936 & 229.12 & -0.26 & $-2.79 \pm 0.69$ & $-3.25 \pm 0.74$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.82_{-0.06}^{+0.03}$ & $1.00_{-0.85}^{-0.76}$ \\
4418919708567118464 & 229.03 & -0.13 & $-2.31 \pm 0.69$ & $-2.72 \pm 0.59$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418919639845936000 & 229.03 & -0.14 & $-2.41 \pm 0.24$ & $-2.81 \pm 0.20$ & $18.79 \pm 0.01$ & $18.34 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920842436867072 & 229.00 & -0.08 & $-2.46 \pm 0.23$ & $-2.52 \pm 0.20$ & $18.80 \pm 0.01$ & $18.42 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919983443364224 & 229.02 & -0.11 & $-2.37 \pm 0.80$ & $-3.47 \pm 0.70$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920842436859648 & 229.00 & -0.09 & $-3.09 \pm 1.26$ & $-1.80 \pm 1.13$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920743653534208 & 229.01 & -0.10 & $-1.10 \pm 0.94$ & $-3.61 \pm 0.85$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919983443369856 & 229.01 & -0.11 & $-2.78 \pm 0.38$ & $-2.76 \pm 0.33$ & $19.52 \pm 0.01$ & $19.13 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920842441834112 & 229.00 & -0.09 & $-2.83 \pm 1.10$ & $-3.81 \pm 1.03$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920842436871552 & 228.99 & -0.08 & $-2.54 \pm 0.19$ & $-2.52 \pm 0.16$ & $18.51 \pm 0.01$ & $18.07 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919914723870464 & 229.02 & -0.12 & $-2.72 \pm 0.37$ & $-2.84 \pm 0.32$ & $19.60 \pm 0.02$ & $19.17 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920739357629056 & 229.01 & -0.10 & $-2.61 \pm 0.69$ & $-1.74 \pm 0.64$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913764332387712 & 229.04 & -0.15 & $-2.26 \pm 0.81$ & $-2.90 \pm 0.69$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726091439986432 & 229.05 & -0.16 & $-1.99 \pm 1.16$ & $-3.66 \pm 1.00$ & $nan \pm 0.02$ & $nan \pm 0.04$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919987739244800 & 229.01 & -0.11 & $-2.44 \pm 0.49$ & $-3.57 \pm 0.46$ & $19.73 \pm 0.02$ & $19.37 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920846732620416 & 229.00 & -0.09 & $-2.79 \pm 0.03$ & $-2.63 \pm 0.03$ & $15.66 \pm 0.00$ & $14.94 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418924518928958336 & 228.95 & -0.02 & $-2.81 \pm 0.75$ & $-3.08 \pm 0.63$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920846732620928 & 228.99 & -0.09 & $-3.28 \pm 0.41$ & $-3.51 \pm 0.36$ & $19.66 \pm 0.02$ & $19.24 \pm 0.01$ & 6 & $0.91_{-0.03}^{+0.02}$ & $1.00_{-0.92}^{-0.87}$ \\
4418724957568602752 & 229.08 & -0.21 & $-2.61 \pm 0.81$ & $-3.63 \pm 0.72$ & $nan \pm 0.05$ & $nan \pm 0.01$ & 4 & $0.96_{-0.01}^{+0.01}$ & $1.00_{-0.97}^{-0.95}$ \\
4418920739358003456 & 229.00 & -0.10 & $-2.82 \pm 0.92$ & $-1.87 \pm 0.71$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913764330666752 & 229.03 & -0.15 & $-1.68 \pm 1.00$ & $-1.52 \pm 0.76$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920739357629184 & 229.00 & -0.10 & $-2.60 \pm 0.11$ & $-2.74 \pm 0.10$ & $17.81 \pm 0.00$ & $17.33 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920808077115392 & 229.00 & -0.09 & $-2.48 \pm 0.73$ & $-2.45 \pm 0.63$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418919914723874560 & 229.02 & -0.12 & $-2.75 \pm 0.12$ & $-2.66 \pm 0.11$ & $17.91 \pm 0.00$ & $17.40 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418721555954496128 & 229.10 & -0.25 & $-2.91 \pm 0.27$ & $-2.56 \pm 0.26$ & $19.19 \pm 0.01$ & $18.71 \pm 0.01$ & 6 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.93}$ \\
4418914043503869952 & 229.02 & -0.13 & $-1.99 \pm 0.92$ & $-2.25 \pm 0.80$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418925377922801280 & 228.93 & 0.01 & $-1.09 \pm 1.00$ & $-2.48 \pm 0.78$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.82_{-0.05}^{+0.04}$ & $1.00_{-0.86}^{-0.78}$ \\
4418921117314801920 & 228.98 & -0.06 & $-2.11 \pm 0.52$ & $-3.56 \pm 0.44$ & $19.54 \pm 0.01$ & $19.28 \pm 0.01$ & 6 & $0.93_{-0.02}^{+0.01}$ & $1.00_{-0.95}^{-0.91}$ \\
4418913833050157312 & 229.02 & -0.14 & $-3.04 \pm 0.77$ & $-2.01 \pm 0.66$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919919019677056 & 229.02 & -0.13 & $-2.46 \pm 0.53$ & $-2.21 \pm 0.44$ & $19.81 \pm 0.01$ & $19.56 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919914725512832 & 229.01 & -0.12 & $-3.49 \pm 0.96$ & $-2.39 \pm 0.82$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919983443354752 & 229.01 & -0.12 & $-2.50 \pm 0.63$ & $-2.49 \pm 0.56$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913764330665600 & 229.03 & -0.15 & $-2.21 \pm 1.27$ & $-1.21 \pm 1.04$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418913833050162176 & 229.02 & -0.13 & $-2.98 \pm 0.68$ & $-3.33 \pm 0.56$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919983443357568 & 229.01 & -0.12 & $-2.21 \pm 0.50$ & $-2.41 \pm 0.44$ & $19.77 \pm 0.01$ & $19.61 \pm 0.02$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418914039208601600 & 229.01 & -0.13 & $-2.25 \pm 1.07$ & $-3.72 \pm 1.02$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418726061376111616 & 229.04 & -0.17 & $-2.10 \pm 0.63$ & $-2.51 \pm 0.52$ & $20.15 \pm 0.02$ & $19.77 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725988360768512 & 229.05 & -0.17 & $-3.05 \pm 1.02$ & $-2.99 \pm 0.78$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920812373011200 & 228.99 & -0.09 & $-2.06 \pm 0.81$ & $-3.23 \pm 0.80$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920808077123712 & 228.99 & -0.09 & $-3.30 \pm 0.68$ & $-2.80 \pm 0.60$ & $nan \pm 0.01$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726091439988352 & 229.03 & -0.16 & $-2.40 \pm 1.06$ & $-2.54 \pm 0.89$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418724476536379008 & 229.09 & -0.25 & $-1.86 \pm 0.58$ & $-2.79 \pm 0.55$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.91_{-0.03}^{+0.02}$ & $1.00_{-0.93}^{-0.87}$ \\
4418920808077114368 & 228.99 & -0.09 & $-1.38 \pm 0.78$ & $-3.98 \pm 0.67$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.93}$ \\
4418920808078657280 & 228.99 & -0.09 & $-3.19 \pm 0.94$ & $-2.26 \pm 0.79$ & $nan \pm 0.08$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914107928101632 & 229.00 & -0.11 & $-3.28 \pm 0.48$ & $-2.95 \pm 0.41$ & $19.89 \pm 0.01$ & $19.52 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726057080247552 & 229.04 & -0.17 & $-2.89 \pm 0.98$ & $-3.44 \pm 0.82$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418914107928097920 & 229.00 & -0.12 & $-3.66 \pm 0.69$ & $-2.64 \pm 0.61$ & $nan \pm 0.01$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920739357623296 & 228.99 & -0.10 & $-2.31 \pm 0.24$ & $-2.74 \pm 0.21$ & $19.00 \pm 0.01$ & $18.54 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418921014235565696 & 228.98 & -0.08 & $-2.22 \pm 0.63$ & $-3.14 \pm 0.59$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914039213637504 & 229.01 & -0.13 & $-3.19 \pm 0.35$ & $-2.74 \pm 0.30$ & $19.49 \pm 0.01$ & $19.08 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725610403635712 & 229.05 & -0.20 & $-3.40 \pm 1.30$ & $-3.88 \pm 1.03$ & $nan \pm 0.06$ & $nan \pm 0.02$ & 4 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.93}$ \\
4418924072252304256 & 228.96 & -0.06 & $-1.46 \pm 1.44$ & $-1.83 \pm 1.16$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.97_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418925343562694016 & 228.92 & -0.00 & $-2.61 \pm 0.63$ & $-3.13 \pm 0.53$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418725679123113088 & 229.05 & -0.20 & $-3.44 \pm 0.67$ & $-2.77 \pm 0.57$ & $20.05 \pm 0.01$ & $19.67 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418914043504415104 & 229.01 & -0.13 & $-2.87 \pm 0.06$ & $-2.62 \pm 0.05$ & $16.61 \pm 0.00$ & $15.96 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914868138142208 & 228.99 & -0.11 & $-2.69 \pm 0.34$ & $-2.99 \pm 0.30$ & $19.30 \pm 0.01$ & $18.99 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418725988360766336 & 229.04 & -0.18 & $-1.94 \pm 0.61$ & $-3.03 \pm 0.49$ & $20.12 \pm 0.02$ & $19.74 \pm 0.03$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913798690406016 & 229.02 & -0.15 & $-1.93 \pm 0.72$ & $-2.68 \pm 0.61$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726057080246272 & 229.03 & -0.17 & $-2.44 \pm 1.26$ & $-3.63 \pm 1.11$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913798692088576 & 229.01 & -0.15 & $-2.91 \pm 0.79$ & $-2.80 \pm 0.68$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418726061375864320 & 229.03 & -0.17 & $-2.73 \pm 0.06$ & $-2.82 \pm 0.05$ & $16.11 \pm 0.00$ & $15.48 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418924140972103680 & 228.96 & -0.06 & $-2.36 \pm 0.63$ & $-3.02 \pm 0.54$ & $19.82 \pm 0.08$ & $19.64 \pm 0.04$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913729970917504 & 229.02 & -0.15 & $-2.07 \pm 1.01$ & $-1.51 \pm 0.88$ & $nan \pm 0.04$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914039208592640 & 229.01 & -0.13 & $-2.09 \pm 0.82$ & $-2.91 \pm 0.68$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914112223414400 & 229.00 & -0.13 & $-1.87 \pm 2.06$ & $-1.65 \pm 1.26$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920812372330240 & 228.98 & -0.10 & $-3.91 \pm 1.45$ & $-1.13 \pm 1.64$ & $nan \pm 0.04$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913729970919168 & 229.02 & -0.15 & $-2.92 \pm 0.21$ & $-2.60 \pm 0.17$ & $18.71 \pm 0.01$ & $18.25 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914936857620224 & 228.98 & -0.10 & $-2.74 \pm 0.04$ & $-2.64 \pm 0.03$ & $15.99 \pm 0.00$ & $15.29 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418726057080244480 & 229.03 & -0.18 & $-3.48 \pm 1.21$ & $-3.01 \pm 0.96$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418914932561849728 & 228.98 & -0.10 & $-1.79 \pm 0.64$ & $-2.40 \pm 0.56$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418914107928077440 & 229.00 & -0.13 & $-2.88 \pm 0.69$ & $-3.12 \pm 0.64$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418913798690410624 & 229.01 & -0.14 & $-3.12 \pm 0.88$ & $-2.74 \pm 0.75$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726057080246016 & 229.03 & -0.17 & $-2.68 \pm 0.91$ & $-3.22 \pm 0.83$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418924420144859392 & 228.93 & -0.03 & $-3.32 \pm 1.14$ & $-3.45 \pm 0.93$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.92_{-0.03}^{+0.02}$ & $1.00_{-0.94}^{-0.89}$ \\
4418914107928092160 & 228.99 & -0.12 & $-2.79 \pm 0.33$ & $-2.69 \pm 0.29$ & $19.41 \pm 0.01$ & $18.98 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914936857750656 & 228.98 & -0.10 & $-1.80 \pm 0.80$ & $-2.75 \pm 0.68$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725954001031040 & 229.02 & -0.17 & $-3.56 \pm 0.68$ & $-1.78 \pm 0.58$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914073568333824 & 229.00 & -0.13 & $-2.18 \pm 0.52$ & $-3.30 \pm 0.43$ & $19.74 \pm 0.01$ & $19.44 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418913798690398464 & 229.01 & -0.15 & $-3.16 \pm 1.09$ & $-2.52 \pm 0.92$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914863842352512 & 228.98 & -0.11 & $-2.99 \pm 0.63$ & $-3.04 \pm 0.57$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418913798692072960 & 229.01 & -0.15 & $-2.01 \pm 1.06$ & $-3.46 \pm 0.86$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418914004848839168 & 229.00 & -0.14 & $-2.54 \pm 0.90$ & $-2.22 \pm 0.83$ & $nan \pm 0.01$ & $nan \pm 0.04$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913798690402048 & 229.01 & -0.15 & $-1.93 \pm 0.86$ & $-2.45 \pm 0.67$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914004848851712 & 229.00 & -0.13 & $-2.36 \pm 0.24$ & $-2.98 \pm 0.23$ & $18.97 \pm 0.01$ & $18.51 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914829482593792 & 228.99 & -0.12 & $-2.33 \pm 0.45$ & $-3.15 \pm 0.40$ & $19.81 \pm 0.02$ & $19.36 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913626891690368 & 229.01 & -0.17 & $-2.64 \pm 0.90$ & $-2.30 \pm 0.73$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725576045414144 & 229.05 & -0.21 & $-2.17 \pm 0.60$ & $-1.58 \pm 0.48$ & $19.90 \pm 0.02$ & $19.57 \pm 0.05$ & 6 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.93}$ \\
4418725958295767296 & 229.02 & -0.17 & $-2.35 \pm 0.47$ & $-3.10 \pm 0.38$ & $19.81 \pm 0.02$ & $19.37 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418725958296689920 & 229.02 & -0.18 & $-2.17 \pm 1.23$ & $-2.85 \pm 0.99$ & $nan \pm 0.03$ & $nan \pm 0.06$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913626891693184 & 229.01 & -0.16 & $-3.13 \pm 0.56$ & $-2.87 \pm 0.47$ & $19.89 \pm 0.02$ & $19.54 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418914936857621504 & 228.97 & -0.10 & $-2.66 \pm 0.74$ & $-1.82 \pm 0.65$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914073568342016 & 228.99 & -0.13 & $-1.96 \pm 0.70$ & $-2.05 \pm 0.64$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913802986244480 & 229.00 & -0.15 & $-2.72 \pm 0.06$ & $-2.61 \pm 0.05$ & $16.50 \pm 0.00$ & $16.08 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914833778403712 & 228.98 & -0.12 & $-2.66 \pm 0.09$ & $-2.82 \pm 0.08$ & $17.34 \pm 0.00$ & $16.80 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913695611185920 & 229.00 & -0.15 & $-1.95 \pm 0.34$ & $-2.92 \pm 0.28$ & $19.36 \pm 0.02$ & $18.91 \pm 0.01$ & 6 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418914077864156288 & 228.99 & -0.13 & $-2.40 \pm 0.75$ & $-2.89 \pm 0.62$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418924312770483712 & 228.94 & -0.05 & $-3.08 \pm 0.81$ & $-2.81 \pm 0.71$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914932563349632 & 228.97 & -0.10 & $-2.57 \pm 0.52$ & $-2.87 \pm 0.46$ & $19.81 \pm 0.01$ & $19.40 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418918162377287936 & 228.95 & -0.07 & $-3.55 \pm 2.56$ & $-3.18 \pm 2.44$ & $nan \pm 0.06$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418913906065459840 & 229.00 & -0.15 & $-2.77 \pm 0.07$ & $-2.71 \pm 0.06$ & $16.83 \pm 0.00$ & $16.24 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913626891691520 & 229.01 & -0.16 & $-1.58 \pm 0.72$ & $-2.90 \pm 0.64$ & $20.11 \pm 0.02$ & $19.76 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418913901769621248 & 228.99 & -0.15 & $-2.06 \pm 0.68$ & $-1.77 \pm 0.59$ & $20.12 \pm 0.03$ & $19.73 \pm 0.02$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418924312770487680 & 228.93 & -0.05 & $-2.63 \pm 0.47$ & $-2.95 \pm 0.39$ & $19.87 \pm 0.02$ & $19.46 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418915207439762304 & 228.96 & -0.09 & $-2.11 \pm 0.91$ & $-3.54 \pm 0.79$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418913695611508864 & 229.00 & -0.16 & $-3.26 \pm 0.72$ & $-2.14 \pm 0.55$ & $20.10 \pm 0.02$ & $19.72 \pm 0.02$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913695611174400 & 229.00 & -0.16 & $-3.38 \pm 0.83$ & $-2.37 \pm 0.67$ & $19.96 \pm 0.01$ & $19.53 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725850921807360 & 229.02 & -0.19 & $-3.07 \pm 0.31$ & $-3.02 \pm 0.26$ & $19.16 \pm 0.01$ & $18.73 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914898202082816 & 228.97 & -0.11 & $-2.03 \pm 1.46$ & $-2.37 \pm 1.31$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913970489114880 & 228.98 & -0.13 & $-2.31 \pm 1.09$ & $-3.07 \pm 1.14$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418914829482592640 & 228.97 & -0.12 & $-2.40 \pm 0.27$ & $-3.14 \pm 0.24$ & $19.15 \pm 0.01$ & $18.71 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913901769619200 & 228.99 & -0.15 & $-2.92 \pm 0.14$ & $-2.58 \pm 0.12$ & $18.13 \pm 0.00$ & $17.63 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913901774186624 & 228.99 & -0.14 & $-3.32 \pm 0.68$ & $-2.96 \pm 0.57$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914829482902784 & 228.97 & -0.12 & $-3.88 \pm 1.07$ & $-3.69 \pm 0.80$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418914829482596864 & 228.97 & -0.12 & $-2.92 \pm 0.45$ & $-2.75 \pm 0.40$ & $19.77 \pm 0.03$ & $19.41 \pm 0.02$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418724373453247872 & 229.05 & -0.24 & $-2.27 \pm 0.66$ & $-2.48 \pm 0.72$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913970489100928 & 228.98 & -0.14 & $-1.85 \pm 0.73$ & $-1.99 \pm 0.67$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418918437255481856 & 228.92 & -0.05 & $-1.94 \pm 1.54$ & $-1.53 \pm 1.24$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.91_{-0.04}^{+0.02}$ & $1.00_{-0.93}^{-0.87}$ \\
4418721044854050816 & 229.08 & -0.29 & $-2.85 \pm 0.17$ & $-2.73 \pm 0.16$ & $18.43 \pm 0.01$ & $18.16 \pm 0.01$ & 6 & $0.93_{-0.05}^{+0.02}$ & $1.00_{-0.94}^{-0.88}$ \\
4418913665547290112 & 228.99 & -0.16 & $-2.75 \pm 0.12$ & $-2.68 \pm 0.09$ & $17.66 \pm 0.01$ & $17.12 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914795122855808 & 228.97 & -0.12 & $-2.58 \pm 0.87$ & $-2.82 \pm 0.83$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914730699187328 & 228.97 & -0.13 & $-2.73 \pm 0.05$ & $-2.66 \pm 0.04$ & $16.32 \pm 0.00$ & $15.73 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913901769619584 & 228.98 & -0.15 & $-2.07 \pm 0.88$ & $-2.18 \pm 0.81$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418915104360532864 & 228.95 & -0.10 & $-2.78 \pm 0.17$ & $-2.73 \pm 0.16$ & $18.28 \pm 0.00$ & $17.83 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913901769612288 & 228.98 & -0.15 & $-3.92 \pm 0.58$ & $-2.74 \pm 0.51$ & $19.89 \pm 0.01$ & $19.55 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418914898202085120 & 228.96 & -0.11 & $-2.90 \pm 1.04$ & $-3.78 \pm 0.91$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913970489106560 & 228.97 & -0.14 & $-2.65 \pm 0.18$ & $-2.51 \pm 0.17$ & $18.55 \pm 0.01$ & $18.07 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418918128017533440 & 228.94 & -0.09 & $-2.34 \pm 1.13$ & $-1.94 \pm 1.12$ & $nan \pm 0.05$ & $nan \pm 0.03$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913592533627392 & 229.00 & -0.18 & $-1.38 \pm 1.25$ & $-1.66 \pm 1.19$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913901769612544 & 228.98 & -0.15 & $-2.75 \pm 1.27$ & $-2.94 \pm 1.56$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418914795122864384 & 228.96 & -0.12 & $-2.64 \pm 0.05$ & $-2.66 \pm 0.05$ & $16.48 \pm 0.00$ & $15.95 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913661251431680 & 228.99 & -0.16 & $-2.84 \pm 0.97$ & $-2.07 \pm 0.92$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418725472964680064 & 229.01 & -0.21 & $-2.55 \pm 0.27$ & $-2.75 \pm 0.21$ & $18.86 \pm 0.00$ & $18.41 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418725198086768768 & 229.03 & -0.23 & $-3.86 \pm 1.19$ & $-1.97 \pm 0.85$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418913592531940992 & 228.99 & -0.17 & $-3.16 \pm 0.61$ & $-2.03 \pm 0.53$ & $19.90 \pm 0.02$ & $19.64 \pm 0.03$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418915001282786048 & 228.95 & -0.10 & $-3.02 \pm 1.01$ & $-2.57 \pm 0.94$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418913214574810752 & 228.99 & -0.18 & $-1.24 \pm 1.17$ & $-2.72 \pm 1.14$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418913661251426304 & 228.98 & -0.17 & $-3.25 \pm 0.81$ & $-3.32 \pm 0.71$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.97}$ \\
4418725541684162816 & 229.00 & -0.19 & $-3.23 \pm 0.50$ & $-3.07 \pm 0.44$ & $19.72 \pm 0.01$ & $19.30 \pm 0.02$ & 6 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418918128017538688 & 228.92 & -0.08 & $-1.79 \pm 0.83$ & $-2.98 \pm 0.73$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418725541684162688 & 229.00 & -0.19 & $-2.90 \pm 0.21$ & $-2.81 \pm 0.18$ & $18.64 \pm 0.01$ & $18.17 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418915001281293440 & 228.95 & -0.12 & $-2.59 \pm 0.26$ & $-2.38 \pm 0.21$ & $18.88 \pm 0.01$ & $18.43 \pm 0.00$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418914760763102080 & 228.95 & -0.13 & $-2.83 \pm 0.81$ & $-2.00 \pm 0.81$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418915001281292672 & 228.94 & -0.12 & $-2.66 \pm 0.59$ & $-2.88 \pm 0.48$ & $19.89 \pm 0.02$ & $19.37 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418914692043612800 & 228.96 & -0.14 & $-2.45 \pm 0.77$ & $-1.50 \pm 0.72$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913489457822720 & 228.98 & -0.17 & $-2.73 \pm 0.21$ & $-2.59 \pm 0.17$ & $18.68 \pm 0.00$ & $18.25 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418725163727028864 & 229.02 & -0.23 & $-1.43 \pm 1.03$ & $-2.94 \pm 0.93$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.93_{-0.04}^{+0.02}$ & $1.00_{-0.95}^{-0.89}$ \\
4418913283294292608 & 228.98 & -0.18 & $-2.49 \pm 0.29$ & $-2.78 \pm 0.23$ & $19.11 \pm 0.01$ & $18.68 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418913214574806400 & 228.99 & -0.19 & $-2.24 \pm 1.06$ & $-2.23 \pm 0.93$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.98_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913936129347840 & 228.96 & -0.15 & $-2.54 \pm 0.69$ & $-3.31 \pm 0.58$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418725438604940928 & 229.00 & -0.21 & $-1.98 \pm 0.30$ & $-2.45 \pm 0.24$ & $19.10 \pm 0.01$ & $18.72 \pm 0.02$ & 6 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418725507324419584 & 228.99 & -0.20 & $-2.90 \pm 1.17$ & $-1.52 \pm 0.97$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418725438604940544 & 229.00 & -0.21 & $-1.28 \pm 1.26$ & $-2.64 \pm 1.21$ & $nan \pm 0.03$ & $nan \pm 0.06$ & 4 & $0.95_{-0.05}^{+0.02}$ & $1.00_{-0.96}^{-0.89}$ \\
4418915035641041024 & 228.93 & -0.11 & $-2.04 \pm 0.68$ & $-2.62 \pm 0.64$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.97_{-0.03}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418725507324419072 & 228.99 & -0.21 & $-1.17 \pm 0.79$ & $-1.96 \pm 0.54$ & $20.09 \pm 0.05$ & $19.69 \pm 0.02$ & 6 & $0.96_{-0.03}^{+0.01}$ & $1.00_{-0.97}^{-0.93}$ \\
4418725507324417792 & 228.99 & -0.21 & $-2.29 \pm 1.64$ & $-3.16 \pm 1.57$ & $nan \pm 0.05$ & $nan \pm 0.01$ & 4 & $0.95_{-0.05}^{+0.01}$ & $1.00_{-0.97}^{-0.91}$ \\
4418918093657796736 & 228.91 & -0.08 & $-2.36 \pm 0.98$ & $-2.01 \pm 0.92$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.93_{-0.08}^{+0.02}$ & $1.00_{-0.95}^{-0.84}$ \\
4418913493748062464 & 228.97 & -0.18 & $-3.40 \pm 1.26$ & $-3.59 \pm 1.23$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.92_{-0.12}^{+0.03}$ & $1.00_{-0.95}^{-0.80}$ \\
4418914588964411904 & 228.93 & -0.13 & $-2.09 \pm 1.13$ & $-3.90 \pm 1.31$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.88_{-0.12}^{+0.07}$ & $1.00_{-0.95}^{-0.76}$ \\
4418914314086924288 & 228.94 & -0.15 & $-3.09 \pm 1.43$ & $-1.93 \pm 1.38$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.90_{-0.08}^{+0.06}$ & $1.00_{-0.96}^{-0.82}$ \\
4418722792905072512 & 229.01 & -0.27 & $-2.72 \pm 0.08$ & $-2.74 \pm 0.07$ & $17.50 \pm 0.01$ & $16.93 \pm 0.00$ & 6 & $0.94_{-0.03}^{+0.03}$ & $1.00_{-0.97}^{-0.90}$ \\
4418913352013765120 & 228.95 & -0.18 & $-2.12 \pm 1.21$ & $-3.30 \pm 1.22$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.84_{-0.08}^{+0.06}$ & $1.00_{-0.90}^{-0.76}$ \\
4418913317654017152 & 228.94 & -0.19 & $-2.41 \pm 0.73$ & $-2.72 \pm 0.53$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.93_{-0.04}^{+0.03}$ & $1.00_{-0.96}^{-0.88}$ \\
4418723583179058944 & 228.97 & -0.26 & $-3.12 \pm 0.46$ & $-3.00 \pm 0.37$ & $19.88 \pm 0.01$ & $19.41 \pm 0.01$ & 6 & $0.86_{-0.11}^{+0.05}$ & $1.00_{-0.91}^{-0.75}$ \\
4418911844480415232 & 228.93 & -0.20 & $-3.56 \pm 0.87$ & $-1.93 \pm 0.72$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.78_{-0.17}^{+0.08}$ & $1.00_{-0.86}^{-0.61}$ \\
4418723583179057024 & 228.96 & -0.26 & $-2.65 \pm 0.12$ & $-2.71 \pm 0.09$ & $17.84 \pm 0.00$ & $17.32 \pm 0.00$ & 6 & $0.94_{-0.07}^{+0.03}$ & $1.00_{-0.97}^{-0.87}$ \\
4418911088567188224 & 228.89 & -0.26 & $-2.97 \pm 0.71$ & $-2.82 \pm 0.60$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.70_{-0.12}^{+0.12}$ & $1.00_{-0.82}^{-0.58}$ \\
4418887272972249088 & 228.81 & -0.32 & $-2.76 \pm 0.10$ & $-3.12 \pm 0.09$ & $17.02 \pm 0.00$ & $16.59 \pm 0.00$ & 6 & $0.80_{-0.08}^{+0.08}$ & $1.00_{-0.88}^{-0.72}$ \\
4418688536245813888 & 228.57 & -0.55 & $-2.78 \pm 0.13$ & $-2.60 \pm 0.12$ & $18.19 \pm 0.01$ & $17.67 \pm 0.00$ & 6 & $0.86_{-0.07}^{+0.05}$ & $1.00_{-0.92}^{-0.79}$ \\
4418687986489979136 & 228.52 & -0.59 & $-2.73 \pm 0.15$ & $-2.76 \pm 0.13$ & $18.47 \pm 0.01$ & $17.98 \pm 0.00$ & 6 & $0.89_{-0.06}^{+0.04}$ & $1.00_{-0.94}^{-0.83}$ \\
4418312228391031296 & 228.50 & -0.65 & $-2.95 \pm 0.11$ & $-2.77 \pm 0.10$ & $17.87 \pm 0.00$ & $17.40 \pm 0.00$ & 6 & $0.88_{-0.07}^{+0.05}$ & $1.00_{-0.93}^{-0.81}$ \\
4418310274181701632 & 228.42 & -0.71 & $-2.76 \pm 0.06$ & $-2.82 \pm 0.06$ & $17.09 \pm 0.01$ & $16.49 \pm 0.00$ & 6 & $0.88_{-0.06}^{+0.05}$ & $1.00_{-0.93}^{-0.82}$ \\
4418305219004364416 & 228.48 & -0.82 & $-2.58 \pm 0.17$ & $-2.75 \pm 0.14$ & $18.49 \pm 0.01$ & $18.01 \pm 0.00$ & 6 & $0.84_{-0.09}^{+0.05}$ & $1.00_{-0.89}^{-0.75}$ \\
4418308414460040704 & 228.43 & -0.79 & $-3.45 \pm 0.39$ & $-3.24 \pm 0.30$ & $19.60 \pm 0.01$ & $19.18 \pm 0.01$ & 6 & $0.75_{-0.11}^{+0.08}$ & $1.00_{-0.83}^{-0.64}$ \\
4418299102970918144 & 228.45 & -0.87 & $-2.16 \pm 0.57$ & $-2.42 \pm 0.40$ & $19.93 \pm 0.02$ & $19.50 \pm 0.01$ & 6 & $0.72_{-0.11}^{+0.09}$ & $1.00_{-0.81}^{-0.61}$ \\
4418296079314608256 & 228.38 & -0.96 & $-2.75 \pm 0.20$ & $-2.77 \pm 0.18$ & $18.82 \pm 0.00$ & $18.36 \pm 0.01$ & 6 & $0.81_{-0.11}^{+0.07}$ & $1.00_{-0.88}^{-0.71}$ \\
4418273577981105664 & 228.08 & -1.06 & $-3.16 \pm 0.13$ & $-2.53 \pm 0.12$ & $17.83 \pm 0.00$ & $17.52 \pm 0.00$ & 6 & $0.73_{-0.11}^{+0.09}$ & $1.00_{-0.82}^{-0.61}$ \\
4418266701738642816 & 228.02 & -1.16 & $-2.47 \pm 0.45$ & $-2.65 \pm 0.41$ & $19.72 \pm 0.02$ & $19.18 \pm 0.01$ & 6 & $0.78_{-0.10}^{+0.08}$ & $1.00_{-0.87}^{-0.68}$ \\
4418265022406118784 & 227.97 & -1.20 & $-2.80 \pm 0.10$ & $-2.87 \pm 0.10$ & $17.41 \pm 0.01$ & $16.86 \pm 0.00$ & 6 & $0.79_{-0.11}^{+0.09}$ & $1.00_{-0.88}^{-0.68}$ \\
4418261930029664256 & 227.96 & -1.23 & $-2.56 \pm 0.12$ & $-2.39 \pm 0.11$ & $17.46 \pm 0.00$ & $17.13 \pm 0.01$ & 6 & $0.74_{-0.12}^{+0.09}$ & $1.00_{-0.83}^{-0.62}$ \\
4418169811571368064 & 227.83 & -1.33 & $-2.90 \pm 0.23$ & $-3.21 \pm 0.19$ & $18.82 \pm 0.01$ & $18.37 \pm 0.01$ & 6 & $0.76_{-0.11}^{+0.08}$ & $1.00_{-0.84}^{-0.66}$ \\
4418151463471047424 & 227.84 & -1.48 & $-2.88 \pm 0.09$ & $-2.88 \pm 0.08$ & $17.64 \pm 0.01$ & $17.09 \pm 0.00$ & 6 & $0.82_{-0.08}^{+0.07}$ & $1.00_{-0.88}^{-0.73}$ \\
4418168780779226496 & 227.68 & -1.35 & $-2.64 \pm 0.11$ & $-2.92 \pm 0.09$ & $17.98 \pm 0.01$ & $17.48 \pm 0.01$ & 6 & $0.82_{-0.09}^{+0.07}$ & $1.00_{-0.89}^{-0.73}$ \\
4418145416157092736 & 227.79 & -1.52 & $-2.62 \pm 0.14$ & $-2.72 \pm 0.12$ & $18.19 \pm 0.01$ & $17.76 \pm 0.01$ & 6 & $0.90_{-0.06}^{+0.04}$ & $1.00_{-0.94}^{-0.84}$ \\
4418157029748670208 & 227.74 & -1.51 & $-2.54 \pm 0.25$ & $-2.64 \pm 0.20$ & $18.98 \pm 0.00$ & $18.71 \pm 0.00$ & 6 & $0.90_{-0.06}^{+0.04}$ & $1.00_{-0.94}^{-0.84}$ \\
4418143766889632896 & 227.79 & -1.60 & $-2.81 \pm 0.06$ & $-2.90 \pm 0.05$ & $16.79 \pm 0.00$ & $16.34 \pm 0.00$ & 6 & $0.90_{-0.06}^{+0.04}$ & $1.00_{-0.94}^{-0.84}$ \\
4418161221636772992 & 227.66 & -1.45 & $-2.73 \pm 0.06$ & $-2.80 \pm 0.05$ & $17.12 \pm 0.00$ & $16.49 \pm 0.00$ & 6 & $0.96_{-0.03}^{+0.02}$ & $1.00_{-0.98}^{-0.93}$ \\
4418156892309990784 & 227.71 & -1.53 & $-2.76 \pm 0.19$ & $-2.93 \pm 0.16$ & $18.85 \pm 0.01$ & $18.39 \pm 0.01$ & 6 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418155243042270208 & 227.67 & -1.57 & $-2.67 \pm 0.44$ & $-2.73 \pm 0.37$ & $19.85 \pm 0.01$ & $19.60 \pm 0.03$ & 6 & $0.85_{-0.10}^{+0.06}$ & $1.00_{-0.91}^{-0.75}$ \\
4418130675829331328 & 227.54 & -1.66 & $-2.85 \pm 0.52$ & $-2.80 \pm 0.46$ & $19.85 \pm 0.01$ & $19.41 \pm 0.01$ & 6 & $0.71_{-0.12}^{+0.11}$ & $1.00_{-0.82}^{-0.58}$ \\
4418115660623630720 & 227.58 & -1.79 & $-2.81 \pm 0.02$ & $-2.81 \pm 0.02$ & $15.17 \pm 0.00$ & $14.18 \pm 0.01$ & 6 & $0.85_{-0.07}^{+0.07}$ & $1.00_{-0.92}^{-0.78}$ \\
4418107444350163840 & 227.30 & -1.94 & $-3.09 \pm 0.45$ & $-2.53 \pm 0.40$ & $19.30 \pm 0.02$ & $19.04 \pm 0.01$ & 6 & $0.73_{-0.10}^{+0.09}$ & $1.00_{-0.82}^{-0.63}$ \\
6339640456410258944 & 227.16 & -2.07 & $-2.49 \pm 0.24$ & $-3.14 \pm 0.20$ & $18.73 \pm 0.01$ & $18.49 \pm 0.00$ & 6 & $0.85_{-0.07}^{+0.06}$ & $1.00_{-0.91}^{-0.78}$ \\
6339645953968373376 & 227.03 & -2.11 & $-2.56 \pm 0.08$ & $-2.76 \pm 0.07$ & $17.41 \pm 0.00$ & $16.85 \pm 0.00$ & 6 & $0.81_{-0.10}^{+0.07}$ & $1.00_{-0.88}^{-0.72}$ \\
6339631114857033856 & 227.08 & -2.22 & $-2.88 \pm 0.13$ & $-3.09 \pm 0.10$ & $18.01 \pm 0.01$ & $17.49 \pm 0.01$ & 6 & $0.76_{-0.11}^{+0.09}$ & $1.00_{-0.85}^{-0.65}$ \\
6339486112465206528 & 226.37 & -2.93 & $-2.85 \pm 0.16$ & $-3.17 \pm 0.13$ & $18.26 \pm 0.01$ & $17.74 \pm 0.01$ & 6 & $0.85_{-0.07}^{+0.06}$ & $1.00_{-0.91}^{-0.78}$ \\
6339462713483344768 & 226.30 & -2.96 & $-2.68 \pm 0.38$ & $-3.12 \pm 0.32$ & $19.56 \pm 0.02$ & $19.23 \pm 0.01$ & 6 & $0.87_{-0.07}^{+0.05}$ & $1.00_{-0.92}^{-0.81}$ \\
6339015216546749952 & 225.81 & -3.60 & $-2.59 \pm 0.16$ & $-3.21 \pm 0.12$ & $18.05 \pm 0.00$ & $17.49 \pm 0.01$ & 6 & $0.73_{-0.12}^{+0.09}$ & $1.00_{-0.82}^{-0.61}$ \\
6338885783411513856 & 225.32 & -3.97 & $-2.64 \pm 0.24$ & $-3.00 \pm 0.19$ & $18.96 \pm 0.01$ & $18.46 \pm 0.01$ & 6 & $0.79_{-0.11}^{+0.07}$ & $1.00_{-0.87}^{-0.68}$ \\
6338877056038740224 & 225.14 & -4.12 & $-2.87 \pm 0.04$ & $-3.07 \pm 0.03$ & $15.52 \pm 0.00$ & $14.81 \pm 0.00$ & 6 & $0.96_{-0.03}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
6337141064617396992 & 223.70 & -5.71 & $-3.13 \pm 0.08$ & $-2.97 \pm 0.06$ & $16.99 \pm 0.00$ & $16.46 \pm 0.00$ & 6 & $0.71_{-0.20}^{+0.13}$ & $1.00_{-0.84}^{-0.52}$ \\
\bottomrule\bottomrule
\end{tabular}
\end{table*}


==> output/pal5/pal5_member_table_full.tex <==
\begin{table*}
\centering
\small
\addtolength{\tabcolsep}{-1pt}
\newcommand\capitem{\\$\phantom{+}\ast$\ }

\caption{Subset of Membership Table.
\\ This table includes a selection of candidate member stars for the GD-1
stream, based on the membership likelihoods.  For each star we include the Gaia
DR3 source ID and astrometric solution, the Pan-STARRS1 photometry, and the
membership likelihoods for the stream and background. The likelihoods are
computed using the trained model described in \autoref{ssub:trained_pal5} and we
include a quality flag ${\rm dim}(\boldsymbol{x})$, indicating the number of
features used by the model.  For most stars all features are measured. We use
dropout regularization to estimate the uncertainty in the likelihoods, and
report the 5\% and 95\% quantiles of the distribution, as well as the
dropout-disabled maximum-likelihood estimate (MLE) of the likelihood.  For
convenience we round the likelihoods to 2 decimal places, and only show the
value and uncertainty when it is non-zero.\\ \textit{The full table is
available online.}
}
\begin{tabular}{@{}r*{4}{c}*{2}{c}c*{2}{l}@{}}
\toprule
\multicolumn{5}{c}{Gaia} & \multicolumn{2}{c}{PS-1} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{Likelihood (${\rm MLE}_{5\%}^{95\%}$)}\\
\cmidrule(lr){1-5} \cmidrule(lr){6-7} \cmidrule(lr){9-11}
\texttt{source\_id} & $\alpha$ [$\mathrm{{}^{\circ}}$] & $\delta$ [$\mathrm{{}^{\circ}}$] & $\mu_{\alpha}^{*}$ [$\frac{\rm{mas}}{\rm{yr}}$] & $\mu_{\delta}$ [$\frac{\rm{mas}}{\rm{yr}}$] & g [mag] & r [mag] & ${\rm dim}(\boldsymbol{x})$ & $\mathcal{L}_{\rm stream}$ & $\mathcal{L}_{\rm background}$ \\
\midrule
4426601206034901632 & 238.96 & 5.65 & $-2.66 \pm 0.56$ & $-2.46 \pm 0.54$ & $19.47 \pm 0.01$ & $19.13 \pm 0.01$ & 6 & $0.69_{-0.12}^{+0.11}$ & $1.00_{-0.80}^{-0.57}$ \\
4426379452583612672 & 238.26 & 5.30 & $-2.87 \pm 0.09$ & $-1.97 \pm 0.08$ & $17.69 \pm 0.01$ & $17.13 \pm 0.00$ & 6 & $0.75_{-0.10}^{+0.08}$ & $1.00_{-0.83}^{-0.65}$ \\
4426348528819597440 & 237.79 & 5.06 & $-3.05 \pm 0.41$ & $-1.86 \pm 0.40$ & $19.69 \pm 0.02$ & $19.40 \pm 0.01$ & 6 & $0.77_{-0.09}^{+0.08}$ & $1.00_{-0.86}^{-0.68}$ \\
4424757462474093952 & 236.12 & 4.36 & $-2.93 \pm 0.16$ & $-2.17 \pm 0.13$ & $18.44 \pm 0.01$ & $17.98 \pm 0.00$ & 6 & $0.74_{-0.10}^{+0.10}$ & $1.00_{-0.84}^{-0.64}$ \\
4427116365888010496 & 233.13 & 2.93 & $-3.01 \pm 0.43$ & $-1.71 \pm 0.41$ & $19.67 \pm 0.01$ & $19.32 \pm 0.01$ & 6 & $0.73_{-0.15}^{+0.09}$ & $1.00_{-0.82}^{-0.58}$ \\
4421111898528957312 & 232.53 & 2.66 & $-2.65 \pm 0.34$ & $-2.41 \pm 0.25$ & $19.35 \pm 0.01$ & $19.03 \pm 0.01$ & 6 & $0.75_{-0.10}^{+0.09}$ & $1.00_{-0.84}^{-0.66}$ \\
4420968923362678912 & 232.17 & 2.21 & $-2.36 \pm 0.74$ & $-3.05 \pm 0.76$ & $nan \pm 0.05$ & $nan \pm 0.04$ & 4 & $0.80_{-0.13}^{+0.06}$ & $1.00_{-0.86}^{-0.67}$ \\
4420966312022528256 & 232.07 & 2.11 & $-2.70 \pm 0.50$ & $-2.48 \pm 0.47$ & $20.06 \pm 0.02$ & $19.68 \pm 0.01$ & 6 & $0.75_{-0.13}^{+0.08}$ & $1.00_{-0.83}^{-0.63}$ \\
4420984419604706816 & 231.95 & 2.30 & $-2.20 \pm 0.55$ & $-2.85 \pm 0.53$ & $20.08 \pm 0.02$ & $19.84 \pm 0.02$ & 6 & $0.71_{-0.11}^{+0.09}$ & $1.00_{-0.80}^{-0.59}$ \\
4420979437442608128 & 231.98 & 2.17 & $-2.61 \pm 0.38$ & $-2.89 \pm 0.33$ & $19.76 \pm 0.02$ & $19.32 \pm 0.01$ & 6 & $0.69_{-0.13}^{+0.11}$ & $1.00_{-0.80}^{-0.57}$ \\
4421172642250281728 & 231.81 & 2.30 & $-2.81 \pm 0.46$ & $-2.43 \pm 0.39$ & $20.16 \pm 0.01$ & $19.75 \pm 0.01$ & 6 & $0.75_{-0.11}^{+0.08}$ & $1.00_{-0.83}^{-0.64}$ \\
4420970057233967360 & 231.88 & 2.02 & $-2.81 \pm 0.17$ & $-2.40 \pm 0.15$ & $18.58 \pm 0.01$ & $18.09 \pm 0.01$ & 6 & $0.87_{-0.09}^{+0.05}$ & $1.00_{-0.91}^{-0.78}$ \\
4420974523999996032 & 231.81 & 2.11 & $-2.38 \pm 0.38$ & $-2.31 \pm 0.33$ & $19.69 \pm 0.02$ & $19.27 \pm 0.01$ & 6 & $0.77_{-0.11}^{+0.08}$ & $1.00_{-0.85}^{-0.66}$ \\
4420974077323374464 & 231.82 & 2.06 & $-2.59 \pm 0.22$ & $-2.57 \pm 0.19$ & $19.05 \pm 0.01$ & $18.62 \pm 0.02$ & 6 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.92}$ \\
4420974798877893504 & 231.75 & 2.09 & $-2.44 \pm 0.46$ & $-2.29 \pm 0.36$ & $19.86 \pm 0.01$ & $19.51 \pm 0.01$ & 6 & $0.78_{-0.13}^{+0.07}$ & $1.00_{-0.85}^{-0.65}$ \\
4421139175865071360 & 231.67 & 2.09 & $-2.80 \pm 0.40$ & $-2.29 \pm 0.32$ & $19.51 \pm 0.01$ & $19.33 \pm 0.01$ & 6 & $0.82_{-0.10}^{+0.06}$ & $1.00_{-0.88}^{-0.73}$ \\
4420948170080600704 & 231.63 & 1.96 & $-2.77 \pm 0.49$ & $-2.17 \pm 0.42$ & $19.98 \pm 0.02$ & $19.60 \pm 0.01$ & 6 & $0.76_{-0.10}^{+0.08}$ & $1.00_{-0.83}^{-0.66}$ \\
4421137904555364992 & 231.50 & 2.03 & $-2.62 \pm 0.36$ & $-2.32 \pm 0.29$ & $19.38 \pm 0.01$ & $18.95 \pm 0.01$ & 6 & $0.84_{-0.09}^{+0.06}$ & $1.00_{-0.90}^{-0.75}$ \\
4421137526598235520 & 231.50 & 2.02 & $-2.95 \pm 0.27$ & $-2.26 \pm 0.25$ & $19.33 \pm 0.01$ & $18.89 \pm 0.01$ & 6 & $0.74_{-0.13}^{+0.08}$ & $1.00_{-0.81}^{-0.61}$ \\
4420942432004721408 & 231.52 & 1.92 & $-2.63 \pm 0.22$ & $-2.69 \pm 0.20$ & $18.83 \pm 0.01$ & $18.37 \pm 0.00$ & 6 & $0.80_{-0.11}^{+0.07}$ & $1.00_{-0.87}^{-0.69}$ \\
4420936384690721280 & 231.62 & 1.76 & $-2.58 \pm 0.21$ & $-2.44 \pm 0.18$ & $18.71 \pm 0.01$ & $18.29 \pm 0.01$ & 6 & $0.82_{-0.09}^{+0.06}$ & $1.00_{-0.88}^{-0.73}$ \\
4421130487147097472 & 231.43 & 1.93 & $-2.89 \pm 0.19$ & $-2.74 \pm 0.16$ & $18.64 \pm 0.01$ & $18.16 \pm 0.01$ & 6 & $0.72_{-0.12}^{+0.09}$ & $1.00_{-0.81}^{-0.60}$ \\
4420934048228488320 & 231.50 & 1.67 & $-2.72 \pm 0.07$ & $-2.61 \pm 0.06$ & $16.95 \pm 0.00$ & $16.34 \pm 0.00$ & 6 & $0.88_{-0.07}^{+0.04}$ & $1.00_{-0.91}^{-0.81}$ \\
4421128077670137472 & 231.36 & 1.85 & $-2.78 \pm 0.29$ & $-2.24 \pm 0.24$ & $19.41 \pm 0.02$ & $18.94 \pm 0.01$ & 6 & $0.85_{-0.08}^{+0.05}$ & $1.00_{-0.90}^{-0.78}$ \\
4420546779620048384 & 231.50 & 1.62 & $-2.71 \pm 0.19$ & $-2.56 \pm 0.17$ & $18.57 \pm 0.01$ & $18.10 \pm 0.01$ & 6 & $0.72_{-0.13}^{+0.10}$ & $1.00_{-0.81}^{-0.59}$ \\
4421145811590429696 & 231.21 & 2.02 & $-2.78 \pm 0.02$ & $-2.50 \pm 0.02$ & $15.31 \pm 0.00$ & $14.34 \pm 0.00$ & 6 & $0.75_{-0.13}^{+0.07}$ & $1.00_{-0.83}^{-0.63}$ \\
4420752147773103616 & 231.31 & 1.80 & $-2.59 \pm 0.48$ & $-2.89 \pm 0.42$ & $20.07 \pm 0.02$ & $19.65 \pm 0.02$ & 6 & $0.78_{-0.10}^{+0.07}$ & $1.00_{-0.85}^{-0.68}$ \\
4420750739023778432 & 231.10 & 1.72 & $-2.38 \pm 0.22$ & $-2.65 \pm 0.20$ & $18.72 \pm 0.01$ & $18.28 \pm 0.01$ & 6 & $0.79_{-0.10}^{+0.07}$ & $1.00_{-0.86}^{-0.68}$ \\
4420754862192806528 & 231.04 & 1.78 & $-2.34 \pm 0.58$ & $-3.09 \pm 0.58$ & $20.07 \pm 0.01$ & $19.80 \pm 0.01$ & 6 & $0.73_{-0.13}^{+0.08}$ & $1.00_{-0.81}^{-0.60}$ \\
4420755072645928448 & 230.98 & 1.79 & $-2.56 \pm 0.06$ & $-2.85 \pm 0.06$ & $16.77 \pm 0.01$ & $16.38 \pm 0.01$ & 6 & $0.75_{-0.11}^{+0.09}$ & $1.00_{-0.84}^{-0.64}$ \\
4420553479766045824 & 231.07 & 1.56 & $-2.55 \pm 0.29$ & $-2.95 \pm 0.27$ & $19.46 \pm 0.01$ & $19.04 \pm 0.01$ & 6 & $0.82_{-0.11}^{+0.07}$ & $1.00_{-0.88}^{-0.70}$ \\
4420552418908966912 & 231.02 & 1.47 & $-2.75 \pm 0.08$ & $-2.48 \pm 0.08$ & $17.45 \pm 0.00$ & $16.91 \pm 0.00$ & 6 & $0.73_{-0.11}^{+0.09}$ & $1.00_{-0.82}^{-0.62}$ \\
4420740912138482944 & 230.97 & 1.55 & $-2.62 \pm 0.13$ & $-2.73 \pm 0.12$ & $18.16 \pm 0.00$ & $17.66 \pm 0.01$ & 6 & $0.82_{-0.11}^{+0.06}$ & $1.00_{-0.87}^{-0.71}$ \\
4420524445786697344 & 231.05 & 1.37 & $-2.67 \pm 0.09$ & $-2.54 \pm 0.08$ & $17.36 \pm 0.00$ & $16.82 \pm 0.01$ & 6 & $0.90_{-0.05}^{+0.03}$ & $1.00_{-0.93}^{-0.84}$ \\
4420721464526574976 & 230.83 & 1.56 & $-2.67 \pm 0.38$ & $-2.35 \pm 0.31$ & $19.35 \pm 0.01$ & $19.02 \pm 0.01$ & 6 & $0.85_{-0.07}^{+0.05}$ & $1.00_{-0.89}^{-0.78}$ \\
4420528568955338112 & 230.90 & 1.42 & $-2.76 \pm 0.19$ & $-2.34 \pm 0.18$ & $18.87 \pm 0.00$ & $18.39 \pm 0.00$ & 6 & $0.72_{-0.13}^{+0.08}$ & $1.00_{-0.81}^{-0.60}$ \\
4420734662961249280 & 230.75 & 1.63 & $-2.64 \pm 0.08$ & $-2.56 \pm 0.07$ & $17.28 \pm 0.00$ & $16.69 \pm 0.00$ & 6 & $0.77_{-0.12}^{+0.08}$ & $1.00_{-0.85}^{-0.64}$ \\
4420512522957298176 & 230.86 & 1.13 & $-2.80 \pm 0.19$ & $-2.47 \pm 0.18$ & $18.75 \pm 0.01$ & $18.23 \pm 0.00$ & 6 & $0.78_{-0.13}^{+0.08}$ & $1.00_{-0.86}^{-0.66}$ \\
4420708888861661440 & 230.63 & 1.35 & $-2.50 \pm 0.14$ & $-2.21 \pm 0.12$ & $18.27 \pm 0.00$ & $17.86 \pm 0.00$ & 6 & $0.74_{-0.12}^{+0.08}$ & $1.00_{-0.82}^{-0.62}$ \\
4420517681213474304 & 230.68 & 1.22 & $-2.68 \pm 0.07$ & $-2.53 \pm 0.06$ & $17.05 \pm 0.00$ & $16.53 \pm 0.00$ & 6 & $0.84_{-0.09}^{+0.05}$ & $1.00_{-0.89}^{-0.75}$ \\
4420711259683622400 & 230.49 & 1.38 & $-2.79 \pm 0.14$ & $-2.55 \pm 0.12$ & $18.22 \pm 0.00$ & $17.71 \pm 0.00$ & 6 & $0.95_{-0.04}^{+0.02}$ & $1.00_{-0.97}^{-0.90}$ \\
4420615396014658432 & 230.44 & 1.23 & $-2.46 \pm 0.35$ & $-2.74 \pm 0.31$ & $19.52 \pm 0.01$ & $19.08 \pm 0.01$ & 6 & $0.88_{-0.08}^{+0.05}$ & $1.00_{-0.92}^{-0.79}$ \\
4420608700160449280 & 230.46 & 1.08 & $-2.78 \pm 0.09$ & $-2.63 \pm 0.08$ & $17.50 \pm 0.01$ & $16.95 \pm 0.00$ & 6 & $0.85_{-0.07}^{+0.05}$ & $1.00_{-0.91}^{-0.78}$ \\
4420608562721387776 & 230.44 & 1.06 & $-2.42 \pm 0.18$ & $-2.61 \pm 0.15$ & $18.57 \pm 0.01$ & $18.10 \pm 0.01$ & 6 & $0.75_{-0.12}^{+0.09}$ & $1.00_{-0.84}^{-0.62}$ \\
4420607768151633408 & 230.21 & 1.13 & $-2.92 \pm 0.16$ & $-2.61 \pm 0.16$ & $18.20 \pm 0.01$ & $17.69 \pm 0.00$ & 6 & $0.69_{-0.11}^{+0.11}$ & $1.00_{-0.80}^{-0.59}$ \\
4420577192280259840 & 230.19 & 0.92 & $-2.78 \pm 0.03$ & $-2.65 \pm 0.03$ & $15.66 \pm 0.00$ & $14.85 \pm 0.00$ & 6 & $0.81_{-0.10}^{+0.08}$ & $1.00_{-0.89}^{-0.71}$ \\
4420385323205469568 & 230.15 & 0.73 & $-2.76 \pm 0.22$ & $-2.42 \pm 0.20$ & $18.98 \pm 0.00$ & $18.52 \pm 0.01$ & 6 & $0.73_{-0.12}^{+0.09}$ & $1.00_{-0.82}^{-0.61}$ \\
4420579460023004800 & 230.01 & 0.92 & $-2.58 \pm 0.08$ & $-2.72 \pm 0.07$ & $17.25 \pm 0.01$ & $16.79 \pm 0.00$ & 6 & $0.96_{-0.03}^{+0.02}$ & $1.00_{-0.98}^{-0.94}$ \\
4420577948194795648 & 230.04 & 0.87 & $-2.97 \pm 0.41$ & $-2.40 \pm 0.33$ & $19.56 \pm 0.01$ & $19.12 \pm 0.01$ & 6 & $0.73_{-0.12}^{+0.10}$ & $1.00_{-0.83}^{-0.61}$ \\
4420376527112384128 & 229.98 & 0.58 & $-2.57 \pm 0.23$ & $-2.67 \pm 0.18$ & $19.01 \pm 0.00$ & $18.74 \pm 0.01$ & 6 & $0.83_{-0.08}^{+0.06}$ & $1.00_{-0.89}^{-0.75}$ \\
4420565677471968384 & 229.87 & 0.65 & $-2.81 \pm 0.38$ & $-2.33 \pm 0.31$ & $19.53 \pm 0.01$ & $19.21 \pm 0.01$ & 6 & $0.78_{-0.10}^{+0.08}$ & $1.00_{-0.87}^{-0.68}$ \\
4419063504070321664 & 229.86 & 0.60 & $-2.68 \pm 0.26$ & $-2.67 \pm 0.22$ & $19.21 \pm 0.01$ & $18.74 \pm 0.00$ & 6 & $0.91_{-0.06}^{+0.04}$ & $1.00_{-0.95}^{-0.85}$ \\
4419064053826136064 & 229.77 & 0.60 & $-2.71 \pm 0.39$ & $-2.26 \pm 0.32$ & $19.61 \pm 0.02$ & $19.35 \pm 0.01$ & 6 & $0.79_{-0.11}^{+0.09}$ & $1.00_{-0.87}^{-0.68}$ \\
4419078145614843776 & 229.61 & 0.64 & $-2.87 \pm 0.30$ & $-2.51 \pm 0.26$ & $19.41 \pm 0.01$ & $18.81 \pm 0.00$ & 6 & $0.73_{-0.15}^{+0.10}$ & $1.00_{-0.83}^{-0.58}$ \\
4419055055870634368 & 229.65 & 0.45 & $-2.70 \pm 0.04$ & $-2.69 \pm 0.03$ & $15.89 \pm 0.00$ & $15.17 \pm 0.00$ & 6 & $0.83_{-0.09}^{+0.06}$ & $1.00_{-0.90}^{-0.74}$ \\
4419058487549267584 & 229.56 & 0.49 & $-2.29 \pm 0.52$ & $-2.98 \pm 0.52$ & $19.84 \pm 0.01$ & $19.42 \pm 0.01$ & 6 & $0.81_{-0.10}^{+0.08}$ & $1.00_{-0.89}^{-0.71}$ \\
4419059797514551168 & 229.52 & 0.55 & $-2.77 \pm 0.07$ & $-2.62 \pm 0.07$ & $17.10 \pm 0.00$ & $16.54 \pm 0.00$ & 6 & $0.76_{-0.10}^{+0.08}$ & $1.00_{-0.84}^{-0.66}$ \\
4419028250978701952 & 229.51 & 0.30 & $-2.76 \pm 0.29$ & $-2.46 \pm 0.29$ & $19.17 \pm 0.01$ & $18.72 \pm 0.02$ & 6 & $0.79_{-0.10}^{+0.09}$ & $1.00_{-0.88}^{-0.68}$ \\
4419027804302099712 & 229.48 & 0.27 & $-2.75 \pm 0.53$ & $-2.45 \pm 0.54$ & $19.98 \pm 0.01$ & $19.66 \pm 0.02$ & 6 & $0.77_{-0.10}^{+0.08}$ & $1.00_{-0.85}^{-0.67}$ \\
4419025300337195264 & 229.39 & 0.17 & $-2.75 \pm 0.10$ & $-2.59 \pm 0.08$ & $17.44 \pm 0.00$ & $16.88 \pm 0.00$ & 6 & $0.87_{-0.07}^{+0.05}$ & $1.00_{-0.92}^{-0.80}$ \\
4419023234457620352 & 229.24 & 0.20 & $-2.69 \pm 0.14$ & $-2.41 \pm 0.11$ & $18.20 \pm 0.01$ & $17.74 \pm 0.00$ & 6 & $0.83_{-0.08}^{+0.08}$ & $1.00_{-0.91}^{-0.75}$ \\
4418926855391616000 & 229.07 & 0.06 & $-2.60 \pm 0.30$ & $-2.81 \pm 0.24$ & $19.37 \pm 0.02$ & $18.94 \pm 0.01$ & 6 & $0.95_{-0.07}^{+0.04}$ & $1.00_{-0.99}^{-0.88}$ \\
4418926477434478080 & 229.07 & 0.04 & $-1.65 \pm 0.57$ & $-2.68 \pm 0.42$ & $20.12 \pm 0.02$ & $19.71 \pm 0.01$ & 6 & $0.61_{-0.26}^{+0.20}$ & $1.00_{-0.82}^{-0.35}$ \\
4418926374355250432 & 229.07 & 0.03 & $-2.50 \pm 0.67$ & $-2.50 \pm 0.54$ & $19.94 \pm 0.02$ & $19.63 \pm 0.01$ & 6 & $0.93_{-0.14}^{+0.04}$ & $1.00_{-0.97}^{-0.79}$ \\
4418928165356912000 & 229.02 & 0.09 & $-2.72 \pm 0.04$ & $-2.66 \pm 0.03$ & $16.11 \pm 0.00$ & $15.51 \pm 0.00$ & 6 & $0.88_{-0.16}^{+0.07}$ & $1.00_{-0.95}^{-0.72}$ \\
4418923007100469760 & 229.08 & -0.02 & $-2.65 \pm 0.11$ & $-2.62 \pm 0.09$ & $17.77 \pm 0.00$ & $17.30 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920361400550912 & 229.12 & -0.07 & $-2.69 \pm 0.96$ & $-2.85 \pm 0.75$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.94_{-0.09}^{+0.03}$ & $1.00_{-0.97}^{-0.85}$ \\
4418926339995504512 & 229.05 & 0.03 & $-1.12 \pm 0.89$ & $-2.68 \pm 0.76$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.78_{-0.19}^{+0.08}$ & $1.00_{-0.87}^{-0.60}$ \\
4418732207473429632 & 229.14 & -0.12 & $-1.57 \pm 0.89$ & $-1.38 \pm 0.75$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.79_{-0.14}^{+0.08}$ & $1.00_{-0.87}^{-0.65}$ \\
4418920636278474880 & 229.10 & -0.06 & $-2.70 \pm 0.11$ & $-2.71 \pm 0.09$ & $17.78 \pm 0.01$ & $17.26 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418921529631708416 & 229.07 & -0.03 & $-1.62 \pm 0.56$ & $-2.43 \pm 0.43$ & $19.90 \pm 0.04$ & $19.45 \pm 0.01$ & 6 & $0.92_{-0.06}^{+0.03}$ & $1.00_{-0.95}^{-0.86}$ \\
4418920331336673024 & 229.11 & -0.08 & $-3.45 \pm 0.84$ & $-2.19 \pm 0.72$ & $nan \pm 0.04$ & $nan \pm 0.01$ & 4 & $0.94_{-0.04}^{+0.02}$ & $1.00_{-0.96}^{-0.89}$ \\
4418926236916260736 & 229.05 & 0.01 & $-2.86 \pm 1.01$ & $-2.64 \pm 0.84$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.94_{-0.05}^{+0.02}$ & $1.00_{-0.96}^{-0.89}$ \\
4418921529631707136 & 229.07 & -0.03 & $-2.17 \pm 0.45$ & $-2.17 \pm 0.38$ & $19.66 \pm 0.04$ & $19.35 \pm 0.01$ & 6 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418921735790148864 & 229.06 & -0.02 & $-2.43 \pm 0.47$ & $-2.68 \pm 0.39$ & $19.81 \pm 0.02$ & $19.35 \pm 0.01$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418921426552475392 & 229.07 & -0.04 & $-3.38 \pm 1.51$ & $-1.03 \pm 1.36$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418926511794191232 & 229.03 & 0.02 & $-2.54 \pm 0.64$ & $-1.73 \pm 0.50$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.92_{-0.04}^{+0.03}$ & $1.00_{-0.95}^{-0.88}$ \\
4418921529631697152 & 229.06 & -0.04 & $-1.49 \pm 1.16$ & $-2.08 \pm 0.95$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.93_{-0.04}^{+0.02}$ & $1.00_{-0.95}^{-0.89}$ \\
4418732551070815360 & 229.11 & -0.11 & $-3.37 \pm 0.68$ & $-2.29 \pm 0.60$ & $20.07 \pm 0.01$ & $19.71 \pm 0.01$ & 6 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.91}$ \\
4418921426552478336 & 229.06 & -0.04 & $-1.30 \pm 0.86$ & $-3.04 \pm 0.75$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.92_{-0.04}^{+0.03}$ & $1.00_{-0.95}^{-0.88}$ \\
4418730764364400512 & 229.15 & -0.18 & $-2.65 \pm 0.92$ & $-1.57 \pm 0.77$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.74_{-0.10}^{+0.07}$ & $1.00_{-0.80}^{-0.64}$ \\
4418921495271963136 & 229.06 & -0.03 & $-2.82 \pm 0.17$ & $-2.74 \pm 0.15$ & $18.37 \pm 0.01$ & $17.93 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418732177408528512 & 229.13 & -0.14 & $-3.25 \pm 1.11$ & $-3.53 \pm 0.93$ & $nan \pm 0.04$ & $nan \pm 0.05$ & 4 & $0.83_{-0.08}^{+0.05}$ & $1.00_{-0.89}^{-0.76}$ \\
4418927649960836352 & 228.98 & 0.07 & $-2.38 \pm 0.27$ & $-2.28 \pm 0.24$ & $19.28 \pm 0.02$ & $18.82 \pm 0.01$ & 6 & $0.86_{-0.07}^{+0.05}$ & $1.00_{-0.90}^{-0.79}$ \\
4418920189601805824 & 229.09 & -0.10 & $-2.40 \pm 1.02$ & $-1.54 \pm 0.91$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.92}$ \\
4418920189601804544 & 229.09 & -0.11 & $-2.07 \pm 0.65$ & $-2.78 \pm 0.53$ & $20.11 \pm 0.02$ & $19.76 \pm 0.02$ & 6 & $0.98_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418920567558981760 & 229.07 & -0.07 & $-1.67 \pm 0.74$ & $-2.71 \pm 0.71$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.96_{-0.02}^{+0.02}$ & $1.00_{-0.97}^{-0.93}$ \\
4418920189601820928 & 229.08 & -0.10 & $-3.06 \pm 0.61$ & $-1.06 \pm 0.51$ & $20.14 \pm 0.02$ & $19.77 \pm 0.02$ & 6 & $0.76_{-0.10}^{+0.09}$ & $1.00_{-0.86}^{-0.66}$ \\
4418920258323013504 & 229.08 & -0.10 & $-2.06 \pm 1.01$ & $-3.20 \pm 0.84$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418920498839492736 & 229.07 & -0.08 & $-3.44 \pm 0.68$ & $-1.42 \pm 0.65$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418921392192734592 & 229.05 & -0.05 & $-2.86 \pm 0.35$ & $-2.55 \pm 0.30$ & $19.21 \pm 0.01$ & $18.83 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418731799452216064 & 229.11 & -0.15 & $-2.82 \pm 1.94$ & $-1.68 \pm 1.24$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.91_{-0.05}^{+0.03}$ & $1.00_{-0.94}^{-0.86}$ \\
4418921392194337152 & 229.05 & -0.05 & $-2.21 \pm 0.55$ & $-2.45 \pm 0.52$ & $19.87 \pm 0.02$ & $19.54 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418921701430402560 & 229.03 & -0.03 & $-2.77 \pm 0.57$ & $-1.92 \pm 0.51$ & $19.92 \pm 0.01$ & $19.55 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418921323473240192 & 229.05 & -0.06 & $-3.50 \pm 0.69$ & $-1.44 \pm 0.65$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418920567558985472 & 229.06 & -0.07 & $-1.84 \pm 0.43$ & $-2.82 \pm 0.38$ & $19.72 \pm 0.01$ & $19.30 \pm 0.01$ & 6 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418920189601803008 & 229.08 & -0.11 & $-3.16 \pm 0.84$ & $-2.37 \pm 0.62$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418925858959184128 & 228.98 & 0.04 & $-2.87 \pm 0.10$ & $-2.70 \pm 0.08$ & $17.63 \pm 0.00$ & $17.11 \pm 0.00$ & 6 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418921396488436352 & 229.04 & -0.04 & $-2.69 \pm 0.06$ & $-2.68 \pm 0.05$ & $16.52 \pm 0.00$ & $15.97 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418732138753953920 & 229.09 & -0.12 & $-2.76 \pm 0.67$ & $-2.36 \pm 0.53$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.98}$ \\
4418926138132347008 & 228.97 & 0.06 & $-2.66 \pm 0.05$ & $-2.74 \pm 0.04$ & $16.24 \pm 0.00$ & $15.56 \pm 0.00$ & 6 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418920258321297792 & 229.07 & -0.10 & $-3.02 \pm 0.66$ & $-2.09 \pm 0.60$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418732070034473856 & 229.09 & -0.13 & $-1.68 \pm 1.73$ & $-2.74 \pm 1.11$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.92}$ \\
4418919811644676480 & 229.08 & -0.11 & $-2.50 \pm 0.76$ & $-2.44 \pm 0.61$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418731829516302848 & 229.10 & -0.14 & $-2.73 \pm 0.11$ & $-2.54 \pm 0.09$ & $17.42 \pm 0.01$ & $17.05 \pm 0.04$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418732143049556096 & 229.09 & -0.13 & $-2.74 \pm 0.16$ & $-2.56 \pm 0.13$ & $18.12 \pm 0.00$ & $17.63 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418921598351163008 & 229.03 & -0.05 & $-2.43 \pm 0.35$ & $-2.04 \pm 0.32$ & $19.39 \pm 0.02$ & $18.98 \pm 0.01$ & 6 & $0.95_{-0.03}^{+0.02}$ & $1.00_{-0.97}^{-0.92}$ \\
4418925068685178368 & 228.98 & 0.02 & $-2.88 \pm 0.36$ & $-2.39 \pm 0.30$ & $19.47 \pm 0.01$ & $19.07 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418919880364162048 & 229.07 & -0.10 & $-1.54 \pm 0.82$ & $-2.52 \pm 0.73$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418921289115106048 & 229.04 & -0.07 & $-2.85 \pm 0.80$ & $-1.24 \pm 0.77$ & $nan \pm 0.07$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920155242104064 & 229.05 & -0.08 & $-1.28 \pm 0.64$ & $-3.15 \pm 0.62$ & $20.10 \pm 0.02$ & $19.72 \pm 0.01$ & 6 & $0.90_{-0.06}^{+0.03}$ & $1.00_{-0.93}^{-0.85}$ \\
4418921667070659840 & 229.02 & -0.03 & $-3.10 \pm 0.87$ & $-3.47 \pm 0.81$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418921289115105792 & 229.04 & -0.07 & $-2.04 \pm 0.58$ & $-2.63 \pm 0.53$ & $19.99 \pm 0.02$ & $19.69 \pm 0.01$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920533199234048 & 229.05 & -0.08 & $-2.36 \pm 0.76$ & $-2.86 \pm 0.66$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.99}$ \\
4418919880365871232 & 229.07 & -0.11 & $-3.82 \pm 1.62$ & $-2.67 \pm 1.13$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418920086522610048 & 229.05 & -0.09 & $-2.76 \pm 0.87$ & $-2.90 \pm 0.68$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.99}$ \\
4418919777284924416 & 229.07 & -0.12 & $-3.26 \pm 0.80$ & $-2.86 \pm 0.57$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418732104394214272 & 229.07 & -0.12 & $-2.95 \pm 0.22$ & $-2.62 \pm 0.17$ & $18.44 \pm 0.01$ & $17.96 \pm 0.00$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418920086522602880 & 229.06 & -0.10 & $-2.09 \pm 0.82$ & $-1.80 \pm 0.72$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418732039970339968 & 229.09 & -0.15 & $-2.67 \pm 0.04$ & $-2.66 \pm 0.03$ & $15.88 \pm 0.00$ & $15.11 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418921357832971264 & 229.03 & -0.06 & $-2.76 \pm 0.81$ & $-2.11 \pm 0.72$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418921632710914432 & 229.01 & -0.04 & $-2.38 \pm 0.39$ & $-2.96 \pm 0.30$ & $19.41 \pm 0.01$ & $18.94 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418732104394212864 & 229.08 & -0.13 & $-1.89 \pm 0.50$ & $-2.76 \pm 0.41$ & $19.82 \pm 0.01$ & $19.42 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418731932595515136 & 229.09 & -0.15 & $-2.18 \pm 0.71$ & $-1.30 \pm 0.64$ & $19.90 \pm 0.02$ & $19.75 \pm 0.03$ & 6 & $0.94_{-0.04}^{+0.01}$ & $1.00_{-0.95}^{-0.90}$ \\
4418732035674733312 & 229.08 & -0.14 & $-2.72 \pm 0.24$ & $-2.76 \pm 0.20$ & $18.88 \pm 0.01$ & $18.40 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418925897613485952 & 228.96 & 0.03 & $-2.64 \pm 1.72$ & $-2.56 \pm 1.70$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.88_{-0.07}^{+0.03}$ & $1.00_{-0.91}^{-0.81}$ \\
4418920155242103168 & 229.04 & -0.08 & $-3.66 \pm 0.71$ & $-3.28 \pm 0.63$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418730523846217088 & 229.13 & -0.22 & $-2.01 \pm 0.65$ & $-2.64 \pm 0.58$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.90_{-0.06}^{+0.02}$ & $1.00_{-0.92}^{-0.84}$ \\
4418732104394210176 & 229.08 & -0.14 & $-2.14 \pm 0.86$ & $-1.96 \pm 0.71$ & $nan \pm 0.04$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919777284925312 & 229.06 & -0.12 & $-3.40 \pm 0.99$ & $-2.98 \pm 0.79$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418925790239694464 & 228.96 & 0.03 & $-2.54 \pm 0.67$ & $-1.94 \pm 0.60$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.94_{-0.03}^{+0.01}$ & $1.00_{-0.95}^{-0.91}$ \\
4418919777284907392 & 229.07 & -0.13 & $-2.34 \pm 0.88$ & $-2.44 \pm 0.74$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919846004412032 & 229.05 & -0.11 & $-1.89 \pm 0.63$ & $-2.35 \pm 0.54$ & $19.95 \pm 0.01$ & $19.61 \pm 0.01$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919777284923904 & 229.06 & -0.12 & $-2.02 \pm 1.23$ & $-3.91 \pm 1.11$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418730867443614336 & 229.10 & -0.18 & $-2.86 \pm 0.75$ & $-2.56 \pm 0.71$ & $20.14 \pm 0.02$ & $19.75 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418924901181758976 & 228.98 & -0.00 & $-2.58 \pm 0.11$ & $-2.41 \pm 0.09$ & $17.34 \pm 0.00$ & $17.00 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920159537849856 & 229.04 & -0.09 & $-2.76 \pm 0.11$ & $-2.58 \pm 0.10$ & $17.79 \pm 0.00$ & $17.31 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920911156358272 & 229.03 & -0.07 & $-2.51 \pm 1.41$ & $-3.19 \pm 1.03$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418925721520200960 & 228.96 & 0.02 & $-3.96 \pm 1.00$ & $-1.53 \pm 0.80$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.93_{-0.03}^{+0.02}$ & $1.00_{-0.95}^{-0.90}$ \\
4418920911157949824 & 229.02 & -0.07 & $-2.99 \pm 1.54$ & $-3.13 \pm 1.14$ & $nan \pm 0.04$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418921190330132736 & 229.01 & -0.06 & $-2.13 \pm 1.01$ & $-2.61 \pm 1.01$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920911156358400 & 229.02 & -0.07 & $-1.68 \pm 1.27$ & $-1.36 \pm 1.01$ & $nan \pm 0.05$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920052162847488 & 229.05 & -0.11 & $-2.65 \pm 0.88$ & $-3.36 \pm 0.76$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919846004398720 & 229.05 & -0.12 & $-3.60 \pm 1.28$ & $-2.86 \pm 0.91$ & $nan \pm 0.04$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920120882353280 & 229.03 & -0.09 & $-2.58 \pm 0.21$ & $-2.32 \pm 0.19$ & $18.69 \pm 0.00$ & $18.22 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920056458766720 & 229.04 & -0.11 & $-2.93 \pm 1.33$ & $-1.92 \pm 1.55$ & $nan \pm 0.03$ & $nan \pm 0.04$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418731932595516160 & 229.07 & -0.15 & $-2.20 \pm 0.41$ & $-2.38 \pm 0.34$ & $19.49 \pm 0.01$ & $19.15 \pm 0.04$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418919846004412160 & 229.05 & -0.11 & $-3.32 \pm 0.49$ & $-2.75 \pm 0.40$ & $19.80 \pm 0.02$ & $19.36 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418919846004406016 & 229.05 & -0.11 & $-1.70 \pm 1.23$ & $-3.00 \pm 1.06$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919674207428224 & 229.06 & -0.13 & $-2.26 \pm 1.95$ & $-2.61 \pm 1.21$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418919674205691648 & 229.06 & -0.13 & $-3.87 \pm 0.81$ & $-3.31 \pm 0.67$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919674205695488 & 229.05 & -0.13 & $-2.65 \pm 0.24$ & $-2.28 \pm 0.18$ & $18.76 \pm 0.01$ & $18.28 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919674205687424 & 229.06 & -0.13 & $-2.70 \pm 1.08$ & $-1.54 \pm 1.02$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919846004410624 & 229.04 & -0.11 & $-3.99 \pm 1.38$ & $-1.38 \pm 1.26$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418731623357859584 & 229.09 & -0.18 & $-3.88 \pm 0.66$ & $-3.47 \pm 0.56$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.90_{-0.04}^{+0.02}$ & $1.00_{-0.92}^{-0.86}$ \\
4418924656367908992 & 228.98 & -0.02 & $-2.06 \pm 0.80$ & $-2.60 \pm 0.70$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418919949083630080 & 229.04 & -0.11 & $-2.70 \pm 0.22$ & $-2.53 \pm 0.20$ & $18.91 \pm 0.01$ & $18.44 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418721384155802752 & 229.14 & -0.26 & $-2.56 \pm 0.50$ & $-3.09 \pm 0.44$ & $20.08 \pm 0.01$ & $19.67 \pm 0.01$ & 6 & $0.89_{-0.04}^{+0.02}$ & $1.00_{-0.91}^{-0.85}$ \\
4418920881092357120 & 229.02 & -0.08 & $-2.93 \pm 0.23$ & $-2.52 \pm 0.20$ & $18.23 \pm 0.01$ & $17.81 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919949085305216 & 229.04 & -0.11 & $-3.75 \pm 0.62$ & $-3.10 \pm 0.54$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920945516097280 & 229.02 & -0.07 & $-2.54 \pm 0.97$ & $-2.09 \pm 0.91$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.99}$ \\
4418919674205685376 & 229.05 & -0.13 & $-2.56 \pm 0.93$ & $-2.10 \pm 0.81$ & $nan \pm 0.02$ & $nan \pm 0.04$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919953379416192 & 229.04 & -0.11 & $-2.83 \pm 0.30$ & $-2.33 \pm 0.26$ & $19.25 \pm 0.01$ & $18.80 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919949083637376 & 229.03 & -0.10 & $-2.83 \pm 0.85$ & $-2.13 \pm 0.71$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920120882335872 & 229.03 & -0.10 & $-1.91 \pm 0.76$ & $-2.61 \pm 0.69$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919949083633280 & 229.04 & -0.11 & $-2.54 \pm 0.42$ & $-2.07 \pm 0.38$ & $19.61 \pm 0.02$ & $19.19 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418731898235776000 & 229.06 & -0.15 & $-3.59 \pm 1.16$ & $-2.58 \pm 1.00$ & $nan \pm 0.05$ & $nan \pm 0.05$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418731692078914688 & 229.07 & -0.17 & $-2.88 \pm 0.22$ & $-2.73 \pm 0.19$ & $18.37 \pm 0.01$ & $17.85 \pm 0.02$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731902531386240 & 229.07 & -0.16 & $-2.74 \pm 0.06$ & $-2.70 \pm 0.05$ & $16.48 \pm 0.00$ & $15.81 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731966955254144 & 229.06 & -0.15 & $-1.86 \pm 1.17$ & $-3.41 \pm 0.98$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919953379726720 & 229.03 & -0.11 & $-3.05 \pm 0.73$ & $-3.24 \pm 0.70$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919949084019840 & 229.04 & -0.12 & $-3.52 \pm 0.84$ & $-2.52 \pm 0.69$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919742925173888 & 229.04 & -0.13 & $-3.46 \pm 0.67$ & $-2.31 \pm 0.57$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920017803126528 & 229.02 & -0.10 & $-2.07 \pm 0.18$ & $-2.37 \pm 0.15$ & $18.53 \pm 0.01$ & $18.08 \pm 0.01$ & 6 & $0.85_{-0.05}^{+0.03}$ & $1.00_{-0.88}^{-0.80}$ \\
4418920945516089472 & 229.01 & -0.08 & $-2.37 \pm 0.22$ & $-2.74 \pm 0.19$ & $18.78 \pm 0.01$ & $18.34 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919949083928960 & 229.03 & -0.11 & $-2.57 \pm 1.40$ & $-3.06 \pm 1.25$ & $nan \pm 0.08$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418731898235774720 & 229.07 & -0.16 & $-3.15 \pm 0.43$ & $-3.10 \pm 0.35$ & $19.49 \pm 0.03$ & $19.05 \pm 0.00$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920881091801984 & 229.02 & -0.08 & $-2.43 \pm 1.42$ & $-1.30 \pm 1.32$ & $nan \pm 0.04$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418731902530624512 & 229.06 & -0.16 & $-2.25 \pm 1.73$ & $-3.75 \pm 1.26$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418921254753776512 & 228.99 & -0.05 & $-3.03 \pm 0.62$ & $-1.64 \pm 0.46$ & $19.89 \pm 0.02$ & $19.50 \pm 0.01$ & 6 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.94}$ \\
4418919949083634816 & 229.03 & -0.11 & $-1.76 \pm 0.97$ & $-1.19 \pm 0.75$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418919742925176704 & 229.04 & -0.12 & $-2.45 \pm 0.68$ & $-3.97 \pm 0.59$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.97}$ \\
4418921151674544256 & 229.00 & -0.06 & $-2.59 \pm 0.46$ & $-2.44 \pm 0.40$ & $19.52 \pm 0.04$ & $19.17 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418724923208864128 & 229.10 & -0.21 & $-2.81 \pm 0.30$ & $-2.88 \pm 0.27$ & $19.38 \pm 0.01$ & $18.93 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920945516098816 & 229.00 & -0.07 & $-2.17 \pm 0.54$ & $-2.67 \pm 0.44$ & $19.75 \pm 0.02$ & $19.47 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418921220394038272 & 228.99 & -0.05 & $-2.32 \pm 0.46$ & $-3.06 \pm 0.37$ & $19.83 \pm 0.02$ & $19.39 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919953379417344 & 229.03 & -0.11 & $-2.60 \pm 0.11$ & $-2.57 \pm 0.10$ & $17.75 \pm 0.00$ & $17.32 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920017803410688 & 229.02 & -0.10 & $-2.88 \pm 0.58$ & $-2.79 \pm 0.54$ & $20.11 \pm 0.01$ & $19.70 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731902531386112 & 229.06 & -0.16 & $-2.81 \pm 0.23$ & $-2.50 \pm 0.19$ & $18.80 \pm 0.01$ & $18.37 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920017803127040 & 229.02 & -0.10 & $-2.19 \pm 0.86$ & $-2.38 \pm 0.70$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919639845948288 & 229.04 & -0.13 & $-2.58 \pm 0.46$ & $-3.00 \pm 0.34$ & $19.56 \pm 0.01$ & $19.16 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731902531386752 & 229.06 & -0.16 & $-2.88 \pm 0.08$ & $-2.62 \pm 0.06$ & $16.92 \pm 0.00$ & $16.31 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919708565437440 & 229.03 & -0.12 & $-2.68 \pm 0.80$ & $-2.49 \pm 0.76$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418724991928344448 & 229.09 & -0.20 & $-1.78 \pm 0.55$ & $-2.39 \pm 0.48$ & $19.97 \pm 0.02$ & $19.66 \pm 0.04$ & 6 & $0.94_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.93}$ \\
4418921220394032512 & 228.99 & -0.05 & $-2.52 \pm 0.23$ & $-2.44 \pm 0.17$ & $18.71 \pm 0.01$ & $18.26 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920778013142144 & 229.01 & -0.09 & $-2.74 \pm 0.14$ & $-2.77 \pm 0.11$ & $17.92 \pm 0.00$ & $17.42 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418724888849127552 & 229.09 & -0.21 & $-2.29 \pm 1.12$ & $-2.86 \pm 1.00$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.96_{-0.01}^{+0.01}$ & $1.00_{-0.97}^{-0.95}$ \\
4418919639845933568 & 229.05 & -0.14 & $-2.77 \pm 0.19$ & $-2.36 \pm 0.16$ & $18.48 \pm 0.01$ & $18.00 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919712861244416 & 229.03 & -0.13 & $-2.82 \pm 0.09$ & $-2.66 \pm 0.08$ & $17.38 \pm 0.00$ & $16.83 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418731966955254016 & 229.05 & -0.15 & $-3.30 \pm 1.12$ & $-2.86 \pm 1.05$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919639845948928 & 229.04 & -0.13 & $-2.81 \pm 0.46$ & $-3.16 \pm 0.33$ & $19.59 \pm 0.01$ & $19.18 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919953379415808 & 229.03 & -0.12 & $-2.80 \pm 0.05$ & $-2.69 \pm 0.05$ & $16.52 \pm 0.00$ & $15.89 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919919019128960 & 229.03 & -0.12 & $-3.17 \pm 0.95$ & $-1.96 \pm 0.96$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920017803112832 & 229.02 & -0.11 & $-2.87 \pm 0.14$ & $-2.55 \pm 0.12$ & $18.03 \pm 0.00$ & $17.53 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919949085276544 & 229.02 & -0.11 & $-2.30 \pm 0.65$ & $-2.05 \pm 0.61$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920773717375872 & 229.01 & -0.09 & $-2.25 \pm 0.33$ & $-2.83 \pm 0.28$ & $19.37 \pm 0.01$ & $18.96 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919644141222400 & 229.04 & -0.14 & $-3.18 \pm 2.08$ & $-3.50 \pm 1.47$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919919019129216 & 229.03 & -0.12 & $-2.75 \pm 1.26$ & $-2.68 \pm 0.99$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919708565435648 & 229.03 & -0.13 & $-1.52 \pm 0.86$ & $-3.60 \pm 0.73$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418921151674532608 & 228.99 & -0.07 & $-3.15 \pm 0.55$ & $-2.57 \pm 0.48$ & $19.86 \pm 0.02$ & $19.59 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418920842438432256 & 229.00 & -0.09 & $-2.30 \pm 0.59$ & $-2.81 \pm 0.51$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418919712861243264 & 229.04 & -0.13 & $-2.76 \pm 0.04$ & $-2.64 \pm 0.04$ & $16.09 \pm 0.00$ & $15.38 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418925313498622080 & 228.94 & 0.01 & $-2.70 \pm 0.11$ & $-2.72 \pm 0.09$ & $17.75 \pm 0.00$ & $17.32 \pm 0.00$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418731966955253632 & 229.04 & -0.15 & $-2.24 \pm 1.13$ & $-3.31 \pm 0.98$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418726091439988224 & 229.05 & -0.16 & $-2.87 \pm 0.54$ & $-1.69 \pm 0.45$ & $19.75 \pm 0.01$ & $19.58 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418731971250102784 & 229.04 & -0.15 & $-2.15 \pm 1.29$ & $-2.81 \pm 1.02$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418725713482851968 & 229.08 & -0.20 & $-3.72 \pm 0.56$ & $-2.77 \pm 0.48$ & $20.03 \pm 0.02$ & $19.54 \pm 0.01$ & 6 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.94}$ \\
4418920842436859520 & 229.00 & -0.09 & $-1.70 \pm 0.67$ & $-3.04 \pm 0.61$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418919639845925504 & 229.04 & -0.15 & $-2.34 \pm 0.95$ & $-2.73 \pm 0.76$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920773718952832 & 229.00 & -0.09 & $-2.82 \pm 1.56$ & $-3.29 \pm 1.43$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919708567119488 & 229.03 & -0.13 & $-1.43 \pm 1.18$ & $-2.77 \pm 0.84$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418919914723871488 & 229.03 & -0.12 & $-3.71 \pm 0.94$ & $-3.46 \pm 0.77$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920842436874496 & 229.00 & -0.08 & $-2.49 \pm 1.07$ & $-3.01 \pm 0.99$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920842436863744 & 229.00 & -0.09 & $-3.13 \pm 0.24$ & $-2.39 \pm 0.21$ & $18.84 \pm 0.01$ & $18.40 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418920842438420352 & 229.00 & -0.09 & $-3.28 \pm 0.74$ & $-3.66 \pm 0.68$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.97}$ \\
4418913764332401792 & 229.04 & -0.15 & $-2.03 \pm 0.63$ & $-3.45 \pm 0.51$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919712860699520 & 229.03 & -0.13 & $-2.22 \pm 1.95$ & $-1.44 \pm 1.35$ & $nan \pm 0.04$ & $nan \pm 0.03$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418721487235015936 & 229.12 & -0.26 & $-2.79 \pm 0.69$ & $-3.25 \pm 0.74$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.82_{-0.05}^{+0.03}$ & $1.00_{-0.85}^{-0.77}$ \\
4418919708567118464 & 229.03 & -0.13 & $-2.31 \pm 0.69$ & $-2.72 \pm 0.59$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418919639845936000 & 229.03 & -0.14 & $-2.41 \pm 0.24$ & $-2.81 \pm 0.20$ & $18.79 \pm 0.01$ & $18.34 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920842436867072 & 229.00 & -0.08 & $-2.46 \pm 0.23$ & $-2.52 \pm 0.20$ & $18.80 \pm 0.01$ & $18.42 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919983443364224 & 229.02 & -0.11 & $-2.37 \pm 0.80$ & $-3.47 \pm 0.70$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920842436859648 & 229.00 & -0.09 & $-3.09 \pm 1.26$ & $-1.80 \pm 1.13$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920743653534208 & 229.01 & -0.10 & $-1.10 \pm 0.94$ & $-3.61 \pm 0.85$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919983443369856 & 229.01 & -0.11 & $-2.78 \pm 0.38$ & $-2.76 \pm 0.33$ & $19.52 \pm 0.01$ & $19.13 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920842441834112 & 229.00 & -0.09 & $-2.83 \pm 1.10$ & $-3.81 \pm 1.03$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418920842436871552 & 228.99 & -0.08 & $-2.54 \pm 0.19$ & $-2.52 \pm 0.16$ & $18.51 \pm 0.01$ & $18.07 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919914723870464 & 229.02 & -0.12 & $-2.72 \pm 0.37$ & $-2.84 \pm 0.32$ & $19.60 \pm 0.02$ & $19.17 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920739357629056 & 229.01 & -0.10 & $-2.61 \pm 0.69$ & $-1.74 \pm 0.64$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913764332387712 & 229.04 & -0.15 & $-2.26 \pm 0.81$ & $-2.90 \pm 0.69$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418726091439986432 & 229.05 & -0.16 & $-1.99 \pm 1.16$ & $-3.66 \pm 1.00$ & $nan \pm 0.02$ & $nan \pm 0.04$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418919987739244800 & 229.01 & -0.11 & $-2.44 \pm 0.49$ & $-3.57 \pm 0.46$ & $19.73 \pm 0.02$ & $19.37 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920846732620416 & 229.00 & -0.09 & $-2.79 \pm 0.03$ & $-2.63 \pm 0.03$ & $15.66 \pm 0.00$ & $14.94 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418924518928958336 & 228.95 & -0.02 & $-2.81 \pm 0.75$ & $-3.08 \pm 0.63$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920846732620928 & 228.99 & -0.09 & $-3.28 \pm 0.41$ & $-3.51 \pm 0.36$ & $19.66 \pm 0.02$ & $19.24 \pm 0.01$ & 6 & $0.91_{-0.03}^{+0.02}$ & $1.00_{-0.93}^{-0.88}$ \\
4418724957568602752 & 229.08 & -0.21 & $-2.61 \pm 0.81$ & $-3.63 \pm 0.72$ & $nan \pm 0.05$ & $nan \pm 0.01$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418920739358003456 & 229.00 & -0.10 & $-2.82 \pm 0.92$ & $-1.87 \pm 0.71$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913764330666752 & 229.03 & -0.15 & $-1.68 \pm 1.00$ & $-1.52 \pm 0.76$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920739357629184 & 229.00 & -0.10 & $-2.60 \pm 0.11$ & $-2.74 \pm 0.10$ & $17.81 \pm 0.00$ & $17.33 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418920808077115392 & 229.00 & -0.09 & $-2.48 \pm 0.73$ & $-2.45 \pm 0.63$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418919914723874560 & 229.02 & -0.12 & $-2.75 \pm 0.12$ & $-2.66 \pm 0.11$ & $17.91 \pm 0.00$ & $17.40 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418721555954496128 & 229.10 & -0.25 & $-2.91 \pm 0.27$ & $-2.56 \pm 0.26$ & $19.19 \pm 0.01$ & $18.71 \pm 0.01$ & 6 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.94}$ \\
4418914043503869952 & 229.02 & -0.13 & $-1.99 \pm 0.92$ & $-2.25 \pm 0.80$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418925377922801280 & 228.93 & 0.01 & $-1.09 \pm 1.00$ & $-2.48 \pm 0.78$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.82_{-0.05}^{+0.03}$ & $1.00_{-0.86}^{-0.77}$ \\
4418921117314801920 & 228.98 & -0.06 & $-2.11 \pm 0.52$ & $-3.56 \pm 0.44$ & $19.54 \pm 0.01$ & $19.28 \pm 0.01$ & 6 & $0.93_{-0.02}^{+0.01}$ & $1.00_{-0.95}^{-0.91}$ \\
4418913833050157312 & 229.02 & -0.14 & $-3.04 \pm 0.77$ & $-2.01 \pm 0.66$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919919019677056 & 229.02 & -0.13 & $-2.46 \pm 0.53$ & $-2.21 \pm 0.44$ & $19.81 \pm 0.01$ & $19.56 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418919914725512832 & 229.01 & -0.12 & $-3.49 \pm 0.96$ & $-2.39 \pm 0.82$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919983443354752 & 229.01 & -0.12 & $-2.50 \pm 0.63$ & $-2.49 \pm 0.56$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913764330665600 & 229.03 & -0.15 & $-2.21 \pm 1.27$ & $-1.21 \pm 1.04$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418913833050162176 & 229.02 & -0.13 & $-2.98 \pm 0.68$ & $-3.33 \pm 0.56$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418919983443357568 & 229.01 & -0.12 & $-2.21 \pm 0.50$ & $-2.41 \pm 0.44$ & $19.77 \pm 0.01$ & $19.61 \pm 0.02$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418914039208601600 & 229.01 & -0.13 & $-2.25 \pm 1.07$ & $-3.72 \pm 1.02$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418726061376111616 & 229.04 & -0.17 & $-2.10 \pm 0.63$ & $-2.51 \pm 0.52$ & $20.15 \pm 0.02$ & $19.77 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725988360768512 & 229.05 & -0.17 & $-3.05 \pm 1.02$ & $-2.99 \pm 0.78$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418920812373011200 & 228.99 & -0.09 & $-2.06 \pm 0.81$ & $-3.23 \pm 0.80$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920808077123712 & 228.99 & -0.09 & $-3.30 \pm 0.68$ & $-2.80 \pm 0.60$ & $nan \pm 0.01$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726091439988352 & 229.03 & -0.16 & $-2.40 \pm 1.06$ & $-2.54 \pm 0.89$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418724476536379008 & 229.09 & -0.25 & $-1.86 \pm 0.58$ & $-2.79 \pm 0.55$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.91_{-0.03}^{+0.02}$ & $1.00_{-0.93}^{-0.87}$ \\
4418920808077114368 & 228.99 & -0.09 & $-1.38 \pm 0.78$ & $-3.98 \pm 0.67$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.93}$ \\
4418920808078657280 & 228.99 & -0.09 & $-3.19 \pm 0.94$ & $-2.26 \pm 0.79$ & $nan \pm 0.08$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914107928101632 & 229.00 & -0.11 & $-3.28 \pm 0.48$ & $-2.95 \pm 0.41$ & $19.89 \pm 0.01$ & $19.52 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726057080247552 & 229.04 & -0.17 & $-2.89 \pm 0.98$ & $-3.44 \pm 0.82$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418914107928097920 & 229.00 & -0.12 & $-3.66 \pm 0.69$ & $-2.64 \pm 0.61$ & $nan \pm 0.01$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418920739357623296 & 228.99 & -0.10 & $-2.31 \pm 0.24$ & $-2.74 \pm 0.21$ & $19.00 \pm 0.01$ & $18.54 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418921014235565696 & 228.98 & -0.08 & $-2.22 \pm 0.63$ & $-3.14 \pm 0.59$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914039213637504 & 229.01 & -0.13 & $-3.19 \pm 0.35$ & $-2.74 \pm 0.30$ & $19.49 \pm 0.01$ & $19.08 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725610403635712 & 229.05 & -0.20 & $-3.40 \pm 1.30$ & $-3.88 \pm 1.03$ & $nan \pm 0.06$ & $nan \pm 0.02$ & 4 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.93}$ \\
4418924072252304256 & 228.96 & -0.06 & $-1.46 \pm 1.44$ & $-1.83 \pm 1.16$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.97_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.96}$ \\
4418925343562694016 & 228.92 & -0.00 & $-2.61 \pm 0.63$ & $-3.13 \pm 0.53$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418725679123113088 & 229.05 & -0.20 & $-3.44 \pm 0.67$ & $-2.77 \pm 0.57$ & $20.05 \pm 0.01$ & $19.67 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418914043504415104 & 229.01 & -0.13 & $-2.87 \pm 0.06$ & $-2.62 \pm 0.05$ & $16.61 \pm 0.00$ & $15.96 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914868138142208 & 228.99 & -0.11 & $-2.69 \pm 0.34$ & $-2.99 \pm 0.30$ & $19.30 \pm 0.01$ & $18.99 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418725988360766336 & 229.04 & -0.18 & $-1.94 \pm 0.61$ & $-3.03 \pm 0.49$ & $20.12 \pm 0.02$ & $19.74 \pm 0.03$ & 6 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913798690406016 & 229.02 & -0.15 & $-1.93 \pm 0.72$ & $-2.68 \pm 0.61$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726057080246272 & 229.03 & -0.17 & $-2.44 \pm 1.26$ & $-3.63 \pm 1.11$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913798692088576 & 229.01 & -0.15 & $-2.91 \pm 0.79$ & $-2.80 \pm 0.68$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418726061375864320 & 229.03 & -0.17 & $-2.73 \pm 0.06$ & $-2.82 \pm 0.05$ & $16.11 \pm 0.00$ & $15.48 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418924140972103680 & 228.96 & -0.06 & $-2.36 \pm 0.63$ & $-3.02 \pm 0.54$ & $19.82 \pm 0.08$ & $19.64 \pm 0.04$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913729970917504 & 229.02 & -0.15 & $-2.07 \pm 1.01$ & $-1.51 \pm 0.88$ & $nan \pm 0.04$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914039208592640 & 229.01 & -0.13 & $-2.09 \pm 0.82$ & $-2.91 \pm 0.68$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914112223414400 & 229.00 & -0.13 & $-1.87 \pm 2.06$ & $-1.65 \pm 1.26$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418920812372330240 & 228.98 & -0.10 & $-3.91 \pm 1.45$ & $-1.13 \pm 1.64$ & $nan \pm 0.04$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913729970919168 & 229.02 & -0.15 & $-2.92 \pm 0.21$ & $-2.60 \pm 0.17$ & $18.71 \pm 0.01$ & $18.25 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914936857620224 & 228.98 & -0.10 & $-2.74 \pm 0.04$ & $-2.64 \pm 0.03$ & $15.99 \pm 0.00$ & $15.29 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418726057080244480 & 229.03 & -0.18 & $-3.48 \pm 1.21$ & $-3.01 \pm 0.96$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418914932561849728 & 228.98 & -0.10 & $-1.79 \pm 0.64$ & $-2.40 \pm 0.56$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418914107928077440 & 229.00 & -0.13 & $-2.88 \pm 0.69$ & $-3.12 \pm 0.64$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418913798690410624 & 229.01 & -0.14 & $-3.12 \pm 0.88$ & $-2.74 \pm 0.75$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418726057080246016 & 229.03 & -0.17 & $-2.68 \pm 0.91$ & $-3.22 \pm 0.83$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418924420144859392 & 228.93 & -0.03 & $-3.32 \pm 1.14$ & $-3.45 \pm 0.93$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.92_{-0.03}^{+0.02}$ & $1.00_{-0.94}^{-0.89}$ \\
4418914107928092160 & 228.99 & -0.12 & $-2.79 \pm 0.33$ & $-2.69 \pm 0.29$ & $19.41 \pm 0.01$ & $18.98 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914936857750656 & 228.98 & -0.10 & $-1.80 \pm 0.80$ & $-2.75 \pm 0.68$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725954001031040 & 229.02 & -0.17 & $-3.56 \pm 0.68$ & $-1.78 \pm 0.58$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914073568333824 & 229.00 & -0.13 & $-2.18 \pm 0.52$ & $-3.30 \pm 0.43$ & $19.74 \pm 0.01$ & $19.44 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418913798690398464 & 229.01 & -0.15 & $-3.16 \pm 1.09$ & $-2.52 \pm 0.92$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914863842352512 & 228.98 & -0.11 & $-2.99 \pm 0.63$ & $-3.04 \pm 0.57$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418913798692072960 & 229.01 & -0.15 & $-2.01 \pm 1.06$ & $-3.46 \pm 0.86$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.98}$ \\
4418914004848839168 & 229.00 & -0.14 & $-2.54 \pm 0.90$ & $-2.22 \pm 0.83$ & $nan \pm 0.01$ & $nan \pm 0.04$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913798690402048 & 229.01 & -0.15 & $-1.93 \pm 0.86$ & $-2.45 \pm 0.67$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914004848851712 & 229.00 & -0.13 & $-2.36 \pm 0.24$ & $-2.98 \pm 0.23$ & $18.97 \pm 0.01$ & $18.51 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914829482593792 & 228.99 & -0.12 & $-2.33 \pm 0.45$ & $-3.15 \pm 0.40$ & $19.81 \pm 0.02$ & $19.36 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913626891690368 & 229.01 & -0.17 & $-2.64 \pm 0.90$ & $-2.30 \pm 0.73$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725576045414144 & 229.05 & -0.21 & $-2.17 \pm 0.60$ & $-1.58 \pm 0.48$ & $19.90 \pm 0.02$ & $19.57 \pm 0.05$ & 6 & $0.95_{-0.02}^{+0.01}$ & $1.00_{-0.96}^{-0.93}$ \\
4418725958295767296 & 229.02 & -0.17 & $-2.35 \pm 0.47$ & $-3.10 \pm 0.38$ & $19.81 \pm 0.02$ & $19.37 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418725958296689920 & 229.02 & -0.18 & $-2.17 \pm 1.23$ & $-2.85 \pm 0.99$ & $nan \pm 0.03$ & $nan \pm 0.06$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913626891693184 & 229.01 & -0.16 & $-3.13 \pm 0.56$ & $-2.87 \pm 0.47$ & $19.89 \pm 0.02$ & $19.54 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418914936857621504 & 228.97 & -0.10 & $-2.66 \pm 0.74$ & $-1.82 \pm 0.65$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914073568342016 & 228.99 & -0.13 & $-1.96 \pm 0.70$ & $-2.05 \pm 0.64$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913802986244480 & 229.00 & -0.15 & $-2.72 \pm 0.06$ & $-2.61 \pm 0.05$ & $16.50 \pm 0.00$ & $16.08 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914833778403712 & 228.98 & -0.12 & $-2.66 \pm 0.09$ & $-2.82 \pm 0.08$ & $17.34 \pm 0.00$ & $16.80 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913695611185920 & 229.00 & -0.15 & $-1.95 \pm 0.34$ & $-2.92 \pm 0.28$ & $19.36 \pm 0.02$ & $18.91 \pm 0.01$ & 6 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418914077864156288 & 228.99 & -0.13 & $-2.40 \pm 0.75$ & $-2.89 \pm 0.62$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418924312770483712 & 228.94 & -0.05 & $-3.08 \pm 0.81$ & $-2.81 \pm 0.71$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914932563349632 & 228.97 & -0.10 & $-2.57 \pm 0.52$ & $-2.87 \pm 0.46$ & $19.81 \pm 0.01$ & $19.40 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418918162377287936 & 228.95 & -0.07 & $-3.55 \pm 2.56$ & $-3.18 \pm 2.44$ & $nan \pm 0.06$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418913906065459840 & 229.00 & -0.15 & $-2.77 \pm 0.07$ & $-2.71 \pm 0.06$ & $16.83 \pm 0.00$ & $16.24 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913626891691520 & 229.01 & -0.16 & $-1.58 \pm 0.72$ & $-2.90 \pm 0.64$ & $20.11 \pm 0.02$ & $19.76 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418913901769621248 & 228.99 & -0.15 & $-2.06 \pm 0.68$ & $-1.77 \pm 0.59$ & $20.12 \pm 0.03$ & $19.73 \pm 0.02$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418924312770487680 & 228.93 & -0.05 & $-2.63 \pm 0.47$ & $-2.95 \pm 0.39$ & $19.87 \pm 0.02$ & $19.46 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418915207439762304 & 228.96 & -0.09 & $-2.11 \pm 0.91$ & $-3.54 \pm 0.79$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913695611508864 & 229.00 & -0.16 & $-3.26 \pm 0.72$ & $-2.14 \pm 0.55$ & $20.10 \pm 0.02$ & $19.72 \pm 0.02$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418913695611174400 & 229.00 & -0.16 & $-3.38 \pm 0.83$ & $-2.37 \pm 0.67$ & $19.96 \pm 0.01$ & $19.53 \pm 0.01$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418725850921807360 & 229.02 & -0.19 & $-3.07 \pm 0.31$ & $-3.02 \pm 0.26$ & $19.16 \pm 0.01$ & $18.73 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914898202082816 & 228.97 & -0.11 & $-2.03 \pm 1.46$ & $-2.37 \pm 1.31$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913970489114880 & 228.98 & -0.13 & $-2.31 \pm 1.09$ & $-3.07 \pm 1.14$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.99}$ \\
4418914829482592640 & 228.97 & -0.12 & $-2.40 \pm 0.27$ & $-3.14 \pm 0.24$ & $19.15 \pm 0.01$ & $18.71 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913901769619200 & 228.99 & -0.15 & $-2.92 \pm 0.14$ & $-2.58 \pm 0.12$ & $18.13 \pm 0.00$ & $17.63 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913901774186624 & 228.99 & -0.14 & $-3.32 \pm 0.68$ & $-2.96 \pm 0.57$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914829482902784 & 228.97 & -0.12 & $-3.88 \pm 1.07$ & $-3.69 \pm 0.80$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418914829482596864 & 228.97 & -0.12 & $-2.92 \pm 0.45$ & $-2.75 \pm 0.40$ & $19.77 \pm 0.03$ & $19.41 \pm 0.02$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418724373453247872 & 229.05 & -0.24 & $-2.27 \pm 0.66$ & $-2.48 \pm 0.72$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418913970489100928 & 228.98 & -0.14 & $-1.85 \pm 0.73$ & $-1.99 \pm 0.67$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418918437255481856 & 228.92 & -0.05 & $-1.94 \pm 1.54$ & $-1.53 \pm 1.24$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.91_{-0.04}^{+0.02}$ & $1.00_{-0.93}^{-0.87}$ \\
4418721044854050816 & 229.08 & -0.29 & $-2.85 \pm 0.17$ & $-2.73 \pm 0.16$ & $18.43 \pm 0.01$ & $18.16 \pm 0.01$ & 6 & $0.93_{-0.04}^{+0.01}$ & $1.00_{-0.94}^{-0.88}$ \\
4418913665547290112 & 228.99 & -0.16 & $-2.75 \pm 0.12$ & $-2.68 \pm 0.09$ & $17.66 \pm 0.01$ & $17.12 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418914795122855808 & 228.97 & -0.12 & $-2.58 \pm 0.87$ & $-2.82 \pm 0.83$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418914730699187328 & 228.97 & -0.13 & $-2.73 \pm 0.05$ & $-2.66 \pm 0.04$ & $16.32 \pm 0.00$ & $15.73 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913901769619584 & 228.98 & -0.15 & $-2.07 \pm 0.88$ & $-2.18 \pm 0.81$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418915104360532864 & 228.95 & -0.10 & $-2.78 \pm 0.17$ & $-2.73 \pm 0.16$ & $18.28 \pm 0.00$ & $17.83 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913901769612288 & 228.98 & -0.15 & $-3.92 \pm 0.58$ & $-2.74 \pm 0.51$ & $19.89 \pm 0.01$ & $19.55 \pm 0.01$ & 6 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.98}^{-0.97}$ \\
4418914898202085120 & 228.96 & -0.11 & $-2.90 \pm 1.04$ & $-3.78 \pm 0.91$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913970489106560 & 228.97 & -0.14 & $-2.65 \pm 0.18$ & $-2.51 \pm 0.17$ & $18.55 \pm 0.01$ & $18.07 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418918128017533440 & 228.94 & -0.09 & $-2.34 \pm 1.13$ & $-1.94 \pm 1.12$ & $nan \pm 0.05$ & $nan \pm 0.03$ & 4 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913592533627392 & 229.00 & -0.18 & $-1.38 \pm 1.25$ & $-1.66 \pm 1.19$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418913901769612544 & 228.98 & -0.15 & $-2.75 \pm 1.27$ & $-2.94 \pm 1.56$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.97}$ \\
4418914795122864384 & 228.96 & -0.12 & $-2.64 \pm 0.05$ & $-2.66 \pm 0.05$ & $16.48 \pm 0.00$ & $15.95 \pm 0.00$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418913661251431680 & 228.99 & -0.16 & $-2.84 \pm 0.97$ & $-2.07 \pm 0.92$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418725472964680064 & 229.01 & -0.21 & $-2.55 \pm 0.27$ & $-2.75 \pm 0.21$ & $18.86 \pm 0.00$ & $18.41 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418725198086768768 & 229.03 & -0.23 & $-3.86 \pm 1.19$ & $-1.97 \pm 0.85$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418913592531940992 & 228.99 & -0.17 & $-3.16 \pm 0.61$ & $-2.03 \pm 0.53$ & $19.90 \pm 0.02$ & $19.64 \pm 0.03$ & 6 & $0.99$ & $1.00_{-0.99}^{-0.99}$ \\
4418915001282786048 & 228.95 & -0.10 & $-3.02 \pm 1.01$ & $-2.57 \pm 0.94$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.99}^{-0.97}$ \\
4418913214574810752 & 228.99 & -0.18 & $-1.24 \pm 1.17$ & $-2.72 \pm 1.14$ & $nan \pm 0.03$ & $nan \pm 0.03$ & 4 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418913661251426304 & 228.98 & -0.17 & $-3.25 \pm 0.81$ & $-3.32 \pm 0.71$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.97}$ \\
4418725541684162816 & 229.00 & -0.19 & $-3.23 \pm 0.50$ & $-3.07 \pm 0.44$ & $19.72 \pm 0.01$ & $19.30 \pm 0.02$ & 6 & $0.97_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418918128017538688 & 228.92 & -0.08 & $-1.79 \pm 0.83$ & $-2.98 \pm 0.73$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.96_{-0.02}^{+0.01}$ & $1.00_{-0.97}^{-0.94}$ \\
4418725541684162688 & 229.00 & -0.19 & $-2.90 \pm 0.21$ & $-2.81 \pm 0.18$ & $18.64 \pm 0.01$ & $18.17 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418915001281293440 & 228.95 & -0.12 & $-2.59 \pm 0.26$ & $-2.38 \pm 0.21$ & $18.88 \pm 0.01$ & $18.43 \pm 0.00$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418914760763102080 & 228.95 & -0.13 & $-2.83 \pm 0.81$ & $-2.00 \pm 0.81$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418915001281292672 & 228.94 & -0.12 & $-2.66 \pm 0.59$ & $-2.88 \pm 0.48$ & $19.89 \pm 0.02$ & $19.37 \pm 0.01$ & 6 & $0.99$ & $1.00_{-1.00}^{-0.99}$ \\
4418914692043612800 & 228.96 & -0.14 & $-2.45 \pm 0.77$ & $-1.50 \pm 0.72$ & $nan \pm 0.01$ & $nan \pm 0.02$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913489457822720 & 228.98 & -0.17 & $-2.73 \pm 0.21$ & $-2.59 \pm 0.17$ & $18.68 \pm 0.00$ & $18.25 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-1.00}$ \\
4418725163727028864 & 229.02 & -0.23 & $-1.43 \pm 1.03$ & $-2.94 \pm 0.93$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.93_{-0.03}^{+0.02}$ & $1.00_{-0.95}^{-0.89}$ \\
4418913283294292608 & 228.98 & -0.18 & $-2.49 \pm 0.29$ & $-2.78 \pm 0.23$ & $19.11 \pm 0.01$ & $18.68 \pm 0.01$ & 6 & $1.00$ & $1.00_{-1.00}^{-0.99}$ \\
4418913214574806400 & 228.99 & -0.19 & $-2.24 \pm 1.06$ & $-2.23 \pm 0.93$ & $nan \pm 0.02$ & $nan \pm 0.03$ & 4 & $0.98_{-0.01}^{+0.01}$ & $1.00_{-0.98}^{-0.96}$ \\
4418913936129347840 & 228.96 & -0.15 & $-2.54 \pm 0.69$ & $-3.31 \pm 0.58$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.99_{-0.01}^{+0.00}$ & $1.00_{-0.99}^{-0.98}$ \\
4418725438604940928 & 229.00 & -0.21 & $-1.98 \pm 0.30$ & $-2.45 \pm 0.24$ & $19.10 \pm 0.01$ & $18.72 \pm 0.02$ & 6 & $0.97_{-0.02}^{+0.01}$ & $1.00_{-0.98}^{-0.95}$ \\
4418725507324419584 & 228.99 & -0.20 & $-2.90 \pm 1.17$ & $-1.52 \pm 0.97$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.97_{-0.03}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418725438604940544 & 229.00 & -0.21 & $-1.28 \pm 1.26$ & $-2.64 \pm 1.21$ & $nan \pm 0.03$ & $nan \pm 0.06$ & 4 & $0.95_{-0.06}^{+0.02}$ & $1.00_{-0.96}^{-0.88}$ \\
4418915035641041024 & 228.93 & -0.11 & $-2.04 \pm 0.68$ & $-2.62 \pm 0.64$ & $nan \pm 0.01$ & $nan \pm 0.01$ & 4 & $0.97_{-0.03}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418725507324419072 & 228.99 & -0.21 & $-1.17 \pm 0.79$ & $-1.96 \pm 0.54$ & $20.09 \pm 0.05$ & $19.69 \pm 0.02$ & 6 & $0.96_{-0.04}^{+0.01}$ & $1.00_{-0.97}^{-0.92}$ \\
4418725507324417792 & 228.99 & -0.21 & $-2.29 \pm 1.64$ & $-3.16 \pm 1.57$ & $nan \pm 0.05$ & $nan \pm 0.01$ & 4 & $0.95_{-0.05}^{+0.01}$ & $1.00_{-0.97}^{-0.90}$ \\
4418918093657796736 & 228.91 & -0.08 & $-2.36 \pm 0.98$ & $-2.01 \pm 0.92$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.93_{-0.08}^{+0.02}$ & $1.00_{-0.95}^{-0.84}$ \\
4418913493748062464 & 228.97 & -0.18 & $-3.40 \pm 1.26$ & $-3.59 \pm 1.23$ & $nan \pm 0.02$ & $nan \pm 0.01$ & 4 & $0.92_{-0.10}^{+0.03}$ & $1.00_{-0.96}^{-0.82}$ \\
4418914588964411904 & 228.93 & -0.13 & $-2.09 \pm 1.13$ & $-3.90 \pm 1.31$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.88_{-0.11}^{+0.07}$ & $1.00_{-0.95}^{-0.77}$ \\
4418914314086924288 & 228.94 & -0.15 & $-3.09 \pm 1.43$ & $-1.93 \pm 1.38$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.90_{-0.08}^{+0.06}$ & $1.00_{-0.96}^{-0.82}$ \\
4418722792905072512 & 229.01 & -0.27 & $-2.72 \pm 0.08$ & $-2.74 \pm 0.07$ & $17.50 \pm 0.01$ & $16.93 \pm 0.00$ & 6 & $0.94_{-0.05}^{+0.03}$ & $1.00_{-0.97}^{-0.89}$ \\
4418913352013765120 & 228.95 & -0.18 & $-2.12 \pm 1.21$ & $-3.30 \pm 1.22$ & $nan \pm 0.03$ & $nan \pm 0.02$ & 4 & $0.84_{-0.10}^{+0.06}$ & $1.00_{-0.90}^{-0.74}$ \\
4418913317654017152 & 228.94 & -0.19 & $-2.41 \pm 0.73$ & $-2.72 \pm 0.53$ & $nan \pm 0.02$ & $nan \pm 0.02$ & 4 & $0.93_{-0.05}^{+0.03}$ & $1.00_{-0.96}^{-0.88}$ \\
4418723583179058944 & 228.97 & -0.26 & $-3.12 \pm 0.46$ & $-3.00 \pm 0.37$ & $19.88 \pm 0.01$ & $19.41 \pm 0.01$ & 6 & $0.86_{-0.11}^{+0.06}$ & $1.00_{-0.92}^{-0.76}$ \\
4418911844480415232 & 228.93 & -0.20 & $-3.56 \pm 0.87$ & $-1.93 \pm 0.72$ & $nan \pm 0.04$ & $nan \pm 0.02$ & 4 & $0.78_{-0.19}^{+0.09}$ & $1.00_{-0.87}^{-0.59}$ \\
4418723583179057024 & 228.96 & -0.26 & $-2.65 \pm 0.12$ & $-2.71 \pm 0.09$ & $17.84 \pm 0.00$ & $17.32 \pm 0.00$ & 6 & $0.94_{-0.08}^{+0.03}$ & $1.00_{-0.96}^{-0.85}$ \\
4418911088567188224 & 228.89 & -0.26 & $-2.97 \pm 0.71$ & $-2.82 \pm 0.60$ & $nan \pm 0.03$ & $nan \pm 0.01$ & 4 & $0.70_{-0.11}^{+0.14}$ & $1.00_{-0.84}^{-0.59}$ \\
4418887272972249088 & 228.81 & -0.32 & $-2.76 \pm 0.10$ & $-3.12 \pm 0.09$ & $17.02 \pm 0.00$ & $16.59 \pm 0.00$ & 6 & $0.80_{-0.10}^{+0.07}$ & $1.00_{-0.87}^{-0.70}$ \\
4418688536245813888 & 228.57 & -0.55 & $-2.78 \pm 0.13$ & $-2.60 \pm 0.12$ & $18.19 \pm 0.01$ & $17.67 \pm 0.00$ & 6 & $0.86_{-0.08}^{+0.05}$ & $1.00_{-0.92}^{-0.79}$ \\
4418687986489979136 & 228.52 & -0.59 & $-2.73 \pm 0.15$ & $-2.76 \pm 0.13$ & $18.47 \pm 0.01$ & $17.98 \pm 0.00$ & 6 & $0.89_{-0.07}^{+0.04}$ & $1.00_{-0.94}^{-0.83}$ \\
4418312228391031296 & 228.50 & -0.65 & $-2.95 \pm 0.11$ & $-2.77 \pm 0.10$ & $17.87 \pm 0.00$ & $17.40 \pm 0.00$ & 6 & $0.88_{-0.07}^{+0.05}$ & $1.00_{-0.93}^{-0.81}$ \\
4418310274181701632 & 228.42 & -0.71 & $-2.76 \pm 0.06$ & $-2.82 \pm 0.06$ & $17.09 \pm 0.01$ & $16.49 \pm 0.00$ & 6 & $0.88_{-0.07}^{+0.05}$ & $1.00_{-0.93}^{-0.81}$ \\
4418305219004364416 & 228.48 & -0.82 & $-2.58 \pm 0.17$ & $-2.75 \pm 0.14$ & $18.49 \pm 0.01$ & $18.01 \pm 0.00$ & 6 & $0.84_{-0.07}^{+0.06}$ & $1.00_{-0.90}^{-0.77}$ \\
4418308414460040704 & 228.43 & -0.79 & $-3.45 \pm 0.39$ & $-3.24 \pm 0.30$ & $19.60 \pm 0.01$ & $19.18 \pm 0.01$ & 6 & $0.75_{-0.11}^{+0.09}$ & $1.00_{-0.84}^{-0.64}$ \\
4418299102970918144 & 228.45 & -0.87 & $-2.16 \pm 0.57$ & $-2.42 \pm 0.40$ & $19.93 \pm 0.02$ & $19.50 \pm 0.01$ & 6 & $0.72_{-0.13}^{+0.09}$ & $1.00_{-0.81}^{-0.58}$ \\
4418296079314608256 & 228.38 & -0.96 & $-2.75 \pm 0.20$ & $-2.77 \pm 0.18$ & $18.82 \pm 0.00$ & $18.36 \pm 0.01$ & 6 & $0.81_{-0.08}^{+0.06}$ & $1.00_{-0.87}^{-0.73}$ \\
4418273577981105664 & 228.08 & -1.06 & $-3.16 \pm 0.13$ & $-2.53 \pm 0.12$ & $17.83 \pm 0.00$ & $17.52 \pm 0.00$ & 6 & $0.73_{-0.12}^{+0.09}$ & $1.00_{-0.82}^{-0.61}$ \\
4418266701738642816 & 228.02 & -1.16 & $-2.47 \pm 0.45$ & $-2.65 \pm 0.41$ & $19.72 \pm 0.02$ & $19.18 \pm 0.01$ & 6 & $0.78_{-0.12}^{+0.07}$ & $1.00_{-0.85}^{-0.67}$ \\
4418265022406118784 & 227.97 & -1.20 & $-2.80 \pm 0.10$ & $-2.87 \pm 0.10$ & $17.41 \pm 0.01$ & $16.86 \pm 0.00$ & 6 & $0.79_{-0.10}^{+0.08}$ & $1.00_{-0.87}^{-0.69}$ \\
4418261930029664256 & 227.96 & -1.23 & $-2.56 \pm 0.12$ & $-2.39 \pm 0.11$ & $17.46 \pm 0.00$ & $17.13 \pm 0.01$ & 6 & $0.74_{-0.12}^{+0.09}$ & $1.00_{-0.83}^{-0.62}$ \\
4418169811571368064 & 227.83 & -1.33 & $-2.90 \pm 0.23$ & $-3.21 \pm 0.19$ & $18.82 \pm 0.01$ & $18.37 \pm 0.01$ & 6 & $0.76_{-0.11}^{+0.09}$ & $1.00_{-0.85}^{-0.65}$ \\
4418151463471047424 & 227.84 & -1.48 & $-2.88 \pm 0.09$ & $-2.88 \pm 0.08$ & $17.64 \pm 0.01$ & $17.09 \pm 0.00$ & 6 & $0.82_{-0.09}^{+0.06}$ & $1.00_{-0.88}^{-0.73}$ \\
4418168780779226496 & 227.68 & -1.35 & $-2.64 \pm 0.11$ & $-2.92 \pm 0.09$ & $17.98 \pm 0.01$ & $17.48 \pm 0.01$ & 6 & $0.82_{-0.09}^{+0.06}$ & $1.00_{-0.88}^{-0.73}$ \\
4418145416157092736 & 227.79 & -1.52 & $-2.62 \pm 0.14$ & $-2.72 \pm 0.12$ & $18.19 \pm 0.01$ & $17.76 \pm 0.01$ & 6 & $0.90_{-0.06}^{+0.04}$ & $1.00_{-0.94}^{-0.84}$ \\
4418157029748670208 & 227.74 & -1.51 & $-2.54 \pm 0.25$ & $-2.64 \pm 0.20$ & $18.98 \pm 0.00$ & $18.71 \pm 0.00$ & 6 & $0.90_{-0.06}^{+0.04}$ & $1.00_{-0.94}^{-0.84}$ \\
4418143766889632896 & 227.79 & -1.60 & $-2.81 \pm 0.06$ & $-2.90 \pm 0.05$ & $16.79 \pm 0.00$ & $16.34 \pm 0.00$ & 6 & $0.90_{-0.06}^{+0.04}$ & $1.00_{-0.94}^{-0.84}$ \\
4418161221636772992 & 227.66 & -1.45 & $-2.73 \pm 0.06$ & $-2.80 \pm 0.05$ & $17.12 \pm 0.00$ & $16.49 \pm 0.00$ & 6 & $0.96_{-0.03}^{+0.02}$ & $1.00_{-0.98}^{-0.93}$ \\
4418156892309990784 & 227.71 & -1.53 & $-2.76 \pm 0.19$ & $-2.93 \pm 0.16$ & $18.85 \pm 0.01$ & $18.39 \pm 0.01$ & 6 & $0.97_{-0.03}^{+0.01}$ & $1.00_{-0.98}^{-0.94}$ \\
4418155243042270208 & 227.67 & -1.57 & $-2.67 \pm 0.44$ & $-2.73 \pm 0.37$ & $19.85 \pm 0.01$ & $19.60 \pm 0.03$ & 6 & $0.85_{-0.10}^{+0.05}$ & $1.00_{-0.91}^{-0.75}$ \\
4418130675829331328 & 227.54 & -1.66 & $-2.85 \pm 0.52$ & $-2.80 \pm 0.46$ & $19.85 \pm 0.01$ & $19.41 \pm 0.01$ & 6 & $0.71_{-0.08}^{+0.11}$ & $1.00_{-0.82}^{-0.62}$ \\
4418115660623630720 & 227.58 & -1.79 & $-2.81 \pm 0.02$ & $-2.81 \pm 0.02$ & $15.17 \pm 0.00$ & $14.18 \pm 0.01$ & 6 & $0.85_{-0.08}^{+0.06}$ & $1.00_{-0.91}^{-0.77}$ \\
4418107444350163840 & 227.30 & -1.94 & $-3.09 \pm 0.45$ & $-2.53 \pm 0.40$ & $19.30 \pm 0.02$ & $19.04 \pm 0.01$ & 6 & $0.73_{-0.11}^{+0.10}$ & $1.00_{-0.83}^{-0.62}$ \\
6339640456410258944 & 227.16 & -2.07 & $-2.49 \pm 0.24$ & $-3.14 \pm 0.20$ & $18.73 \pm 0.01$ & $18.49 \pm 0.00$ & 6 & $0.85_{-0.07}^{+0.05}$ & $1.00_{-0.90}^{-0.78}$ \\
6339645953968373376 & 227.03 & -2.11 & $-2.56 \pm 0.08$ & $-2.76 \pm 0.07$ & $17.41 \pm 0.00$ & $16.85 \pm 0.00$ & 6 & $0.81_{-0.10}^{+0.06}$ & $1.00_{-0.87}^{-0.71}$ \\
6339631114857033856 & 227.08 & -2.22 & $-2.88 \pm 0.13$ & $-3.09 \pm 0.10$ & $18.01 \pm 0.01$ & $17.49 \pm 0.01$ & 6 & $0.76_{-0.11}^{+0.09}$ & $1.00_{-0.85}^{-0.65}$ \\
6339486112465206528 & 226.37 & -2.93 & $-2.85 \pm 0.16$ & $-3.17 \pm 0.13$ & $18.26 \pm 0.01$ & $17.74 \pm 0.01$ & 6 & $0.85_{-0.08}^{+0.06}$ & $1.00_{-0.91}^{-0.78}$ \\
6339462713483344768 & 226.30 & -2.96 & $-2.68 \pm 0.38$ & $-3.12 \pm 0.32$ & $19.56 \pm 0.02$ & $19.23 \pm 0.01$ & 6 & $0.87_{-0.07}^{+0.05}$ & $1.00_{-0.92}^{-0.80}$ \\
6339015216546749952 & 225.81 & -3.60 & $-2.59 \pm 0.16$ & $-3.21 \pm 0.12$ & $18.05 \pm 0.00$ & $17.49 \pm 0.01$ & 6 & $0.73_{-0.13}^{+0.09}$ & $1.00_{-0.83}^{-0.60}$ \\
6338885783411513856 & 225.32 & -3.97 & $-2.64 \pm 0.24$ & $-3.00 \pm 0.19$ & $18.96 \pm 0.01$ & $18.46 \pm 0.01$ & 6 & $0.79_{-0.09}^{+0.09}$ & $1.00_{-0.88}^{-0.70}$ \\
6338877056038740224 & 225.14 & -4.12 & $-2.87 \pm 0.04$ & $-3.07 \pm 0.03$ & $15.52 \pm 0.00$ & $14.81 \pm 0.00$ & 6 & $0.96_{-0.03}^{+0.02}$ & $1.00_{-0.98}^{-0.93}$ \\
6337141064617396992 & 223.70 & -5.71 & $-3.13 \pm 0.08$ & $-2.97 \pm 0.06$ & $16.99 \pm 0.00$ & $16.46 \pm 0.00$ & 6 & $0.71_{-0.20}^{+0.12}$ & $1.00_{-0.84}^{-0.52}$ \\
\bottomrule\bottomrule
\end{tabular}
\end{table*}


==> showyourwork-metadata.tex <==

        \OnGithubActionsfalse
        \def\syw@url{https://nstarman@github.com/nstarman/stellar_stream_density_ml_paper}
    \def\syw@slug{nstarman/stellar_stream_density_ml_paper}
    \def\syw@sha{6f109ac1b9d772ee87481a953ef0cebd0702c573}
    \def\syw@runid{}

        \AddStamptrue
        \newcommand{\syw@stampX}{0.5}
    \newcommand{\syw@stampY}{0.5}
    \newcommand{\syw@stampSize}{0.75}
    \newcommand{\syw@stampAngle}{-20.0}
    \newcommand{\syw@stampText}{nstarman@{\faGithub}/nstarman/stellar{\_}stream{\_}de...}
    \newcommand{\syw@stampVersion}{0.4.2}

        \addvalue{fig:PGM_script}{src/scripts/pgm.py}
        \addvalue{fig:mock_data_photometric_background_selection_script}{src/scripts/mock/plot/photometric_background_selection.py}
        \addvalue{fig:mock_data_photometric_background_selection_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:mock_data_result_script}{src/scripts/mock/plot/results.py}
        \addvalue{fig:mock_data_result_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:gd1-data_selection_script}{src/scripts/gd1/plot/data_selection.py}
        \addvalue{fig:gd1-data_selection_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:gd1-photometric_background_selection_script}{src/scripts/gd1/plot/photometric_background_selection.py}
        \addvalue{fig:gd1-photometric_background_selection_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:gd1-results-full_script}{src/scripts/gd1/plot/results_full.py}
        \addvalue{fig:gd1-results-full_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:gd1-results-panels_script}{src/scripts/gd1/plot/results_panels.py}
        \addvalue{fig:gd1-results-panels_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:gd1-heatmap_script}{src/scripts/gd1/plot/smooth_likelihood.py}
        \addvalue{fig:gd1-heatmap_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:pal5-data_selection_script}{src/scripts/pal5/plot/data_selection.py}
        \addvalue{fig:pal5-data_selection_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:pal5-photometric_background_selection_script}{src/scripts/pal5/plot/photometric_background_selection.py}
        \addvalue{fig:pal5-photometric_background_selection_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:pal5-results-full_script}{src/scripts/pal5/plot/results_full.py}
        \addvalue{fig:pal5-results-full_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:pal5-results-panels_script}{src/scripts/pal5/plot/results_panels.py}
        \addvalue{fig:pal5-results-panels_cache}{https://sandbox.zenodo.org/record/1220409}
        \addvalue{fig:pal5-heatmap_script}{src/scripts/pal5/plot/smooth_likelihood.py}
        \addvalue{fig:pal5-heatmap_cache}{https://sandbox.zenodo.org/record/1220409}
    
        \addvalue{output/mock/nstream_variable.txt_rule}{Snakefile\#L62}
        \addvalue{output/mock/nbackground_variable.txt_rule}{Snakefile\#L74}
        \addvalue{output/mock/isochrone_age_variable.txt_rule}{Snakefile\#L86}
        \addvalue{output/mock/isochrone_feh_variable.txt_rule}{Snakefile\#L98}
        \addvalue{output/gd1/ndata_variable.txt_rule}{Snakefile\#L255}
        \addvalue{output/gd1/control_points.tex_rule}{Snakefile\#L555}
        \addvalue{output/gd1/member_table_select.tex_rule}{Snakefile\#L469}
        \addvalue{output/gd1/nstream/nstream_variable.txt_rule}{Snakefile\#L504}
        \addvalue{output/gd1/nstream/minimum_membership_probability.txt_rule}{Snakefile\#L494}
        \addvalue{output/gd1/nstream/posterior_percentile.txt_rule}{Snakefile\#L484}
        \addvalue{output/gd1/nspur/nspur_variable.txt_rule}{Snakefile\#L538}
        \addvalue{output/pal5/ndata_variable.txt_rule}{Snakefile\#L603}
        \addvalue{output/pal5/control_points.tex_rule}{Snakefile\#L794}
        \addvalue{output/pal5/member_table_select.tex_rule}{Snakefile\#L776}
        


==> showyourwork.tex <==
% Imports
\RequirePackage{mathtools} % equation tags
\RequirePackage{xcolor} % custom colors
\RequirePackage{hyperref} % url links
\RequirePackage{suffix} % allows definition of starred commmands
\RequirePackage{fontawesome5} % FontAwesome symbols
\RequirePackage{letltxmacro} % command redefinitions
\RequirePackage{xstring} % string manipulation
\RequirePackage{catchfile} % read file into macro
\RequirePackage{totcount} % count total number of errors
\RequirePackage[notref, notcite]{showkeys} % get label refs
\RequirePackage{xspace} % better spacing after icons
\RequirePackage{graphicx} % includegraphics
\RequirePackage{stackengine} % stacking figure links
\RequirePackage{tikz} % stamp
\RequirePackage{etoolbox} % ifcsmacro
\RequirePackage{eso-pic} % AddToShipoutPictureBG
\usetikzlibrary{calc}
\usetikzlibrary{math}
\usetikzlibrary{decorations.text}

% Is this running on GitHub Actions?
\newif\ifOnGithubActions

% Should we add a showyourwork stamp?
\newif\ifAddStamp

% Key-value pairs used to assemble the hyperlinks for figures
% See https://tex.stackexchange.com/a/48931
\def\addvalue#1#2{\expandafter\gdef\csname syw@data@\detokenize{#1}\endcsname{#2}}
\def\usevalue#1{%
  \ifcsname syw@data@#1\endcsname%
    \csname syw@data@#1\expandafter\endcsname%
  \else%
    KEYNOTFOUND%
  \fi%
}

% Import metadata
\IfFileExists{./showyourwork-metadata.tex}{
  \input{showyourwork-metadata.tex}
}{
  \OnGithubActionsfalse
  \AddStampfalse
  \def\syw@url{https://github.com/showyourwork/showyourwork-example}
  \def\syw@sha{dev}
  \def\syw@runid{0}
}

% Log figure script commands (a no-op in the build step)
\newcommand\script[1]{}

% Showyourwork logo
\newcommand{\showyourwork}{%
  \smash{\raisebox{-1.4ex}{\includegraphics[width=7.3em]{showyourwork-logo.pdf}}}\xspace%
}

% Define custom colors
\definecolor{sywRed}{rgb}{0.80,0.14,0.19}
\definecolor{sywStampRed}{rgb}{0.80,0.45,0.45}
\definecolor{sywStampLightRed}{rgb}{0.90,0.74,0.74}
\definecolor{sywOrange}{rgb}{1.0,0.65,0.0}
\definecolor{sywYellow}{rgb}{1.0,0.88,0.30}
\definecolor{sywBlue}{rgb}{0.12,0.47,0.71}
\definecolor{sywGreen}{rgb}{0.13,0.53,0.23}

% Generate the stamp on the first page
\ifAddStamp
  % No-op offsets. Override these for, e.g.,
  % specific documentclasses that require a
  % different default stamp position.
  \newcommand{\syw@stampXOffset}{0.00}
  \newcommand{\syw@stampYOffset}{0.00}

  % Define the stamp
  \newcommand{\syw@stamp}{%
    \pgfmathsetmacro{\sr}{0.50}%
    \pgfmathsetmacro{\tr}{1.33*\sr}%
    \pgfmathsetmacro{\vr}{0.15}%
    \pgfmathsetmacro{\sd}{2*\sr}%
    \pgfmathsetmacro{\sx}{\syw@stampX + \syw@stampXOffset}%
    \pgfmathsetmacro{\sy}{\syw@stampY + \syw@stampYOffset}%
    \pgfmathsetmacro{\tx}{\tr*sin(\syw@stampAngle)}%
    \pgfmathsetmacro{\ty}{-\tr*cos(\syw@stampAngle)}%
    \pgfmathsetmacro{\vx}{\vr*sin(\syw@stampAngle)}%
    \pgfmathsetmacro{\vy}{-\vr*cos(\syw@stampAngle)}%
    \pgfmathsetmacro{\invsz}{1/\syw@stampSize}%
    \scalebox{\syw@stampSize}{%
      \href{\syw@url/tree/\syw@sha/}{%
        \begin{tikzpicture}[remember picture,overlay]
          \node (STAMP) at ($\invsz*(current page.north east) - \invsz*(\sx in, \sy in)$)
            [rotate=\syw@stampAngle]
            {\includegraphics[width=\sd in]{showyourwork-stamp.pdf}};
          \node (VERSION) at ($(STAMP.center) - (\vx in, \vy in)$)
            [rotate=\syw@stampAngle,font=\fontsize{5}{7}\selectfont\ttfamily\bfseries,color=sywStampLightRed]
            {\syw@stampVersion};
          \draw[draw=none,
            postaction={decorate},
            decoration={text along path,
              text={|\ttfamily\normalsize\bfseries|\syw@stampText},
              text align=center,
              text color=sywStampRed
            }]
            ($(STAMP.center) - (\tx in, \ty in)$)
            arc
            [start angle={\syw@stampAngle+90},
            end angle={\syw@stampAngle+450},
            radius=\tr in];
        \end{tikzpicture}%
      }%
    }%
  }
  % Render it as a background image on current page
  \AddToShipoutPictureBG*{
    \makeatletter%
    \syw@stamp%
    \makeatother%
  }
\fi

% Custom margin icon
\newcommand\marginicon[1]{
  \renewcommand\showkeyslabelformat[1]{#1}%
}

% User-facing commands
\newcommand\GitHubURL{\syw@url}
\newcommand\GitHubSHA{\syw@sha}
\newcommand\GitHubIcon{\faGithub\xspace}

% Figure script icon
\newcommand\syw@Script[1]{%
  \raisebox{0pt}[6pt][0pt]{%
    \href{\syw@url/blob/\syw@sha/\usevalue{#1}}{%
      \color{sywBlue}\faGithub%
    }%
  }%
}

% Figure dataset icon
\newcommand\syw@DatasetOne[1]{%
  \raisebox{0pt}[6pt][6pt]{%
    \href{\usevalue{#1}}{%
      \color{sywBlue}\faDatabase%
    }%
  }%
}

% Figure dataset icon
\newcommand\syw@DatasetTwo[1]{%
  \raisebox{0pt}[6pt][6pt]{%
    \href{\usevalue{#1}}{%
      \color{sywBlue}\faDatabase%
    }%
  }%
}

% Figure dataset icon
\newcommand\syw@DatasetThree[1]{%
  \raisebox{0pt}[6pt][6pt]{%
    \href{\usevalue{#1}}{%
      \color{sywBlue}\faDatabase%
    }%
  }%
}

% Figure cache icon
\newcommand\syw@Cache[1]{%
  \raisebox{0pt}[6pt][6pt]{%
    \IfSubStr*{\usevalue{#1}}{sandbox}{%
      \href{\usevalue{#1}}{%
        \color{sywRed}\faRecycle%
      }%
    }{%
      \href{\usevalue{#1}}{%
        \color{sywBlue}\faRecycle%
      }%
    }%
  }%
}

% Variable script icon: links to a line in the Snakefile
\newcommand\syw@Variable[1]{%
  \raisebox{0pt}[6pt][0pt]{%
    \href{\syw@url/blob/\syw@sha/\usevalue{#1}}{%
      \color{sywBlue}\faGithub%
    }%
  }%
}

% Hack `showkeys' to show margin links for figures and variables
% See https://tex.stackexchange.com/a/580553
\renewcommand\showkeyslabelformat[1]{%
  \normalfont%
  \setstackgap{S}{0pt}
  \Shortstack[c]{
    \IfEq*{\usevalue{#1_cache}}{KEYNOTFOUND}{}{\syw@Cache{#1_cache}}
    \IfEq*{\usevalue{#1_datasetThree}}{KEYNOTFOUND}{}{\syw@DatasetThree{#1_datasetThree}}
    \IfEq*{\usevalue{#1_datasetTwo}}{KEYNOTFOUND}{}{\syw@DatasetTwo{#1_datasetTwo}}
    \IfEq*{\usevalue{#1_datasetOne}}{KEYNOTFOUND}{}{\syw@DatasetOne{#1_datasetOne}}
    \IfEq*{\usevalue{#1_script}}{KEYNOTFOUND}{}{\syw@Script{#1_script}}
  }
  % Link to the line in the Snakefile that generates a given variable
  % in the texfile
  \IfEq*{\usevalue{#1_rule}}{KEYNOTFOUND}{}{\syw@Variable{#1_rule}}
}

% Set the graphics path for all figures
\graphicspath{{./}{./figures/}}

% Alias of \input for syw-controlled files
\newcommand\variable[1]{%
  \input{#1}\label{#1}\unskip%
}


==> xstring.tex <==
% !TeX encoding = ISO-8859-1
% Ce fichier contient le code de l'extension "xstring"
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
\def\xstringname               {xstring}                             %
\def\xstringversion              {1.83}                              %
%                                                                    %
\def\xstringdate              {2019/02/06}                           %
%                                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
% Author     : Christian Tellechea                                   %
% Status     : Maintained                                            %
% Maintainer : Christian Tellechea                                   %
% Email      : unbonpetit@netc.fr                                    %
% Package URL: https://www.ctan.org/pkg/xstring                      %
% Bug tracker: https://framagit.org/unbonpetit/xstring/issues        %
% Repository : https://framagit.org/unbonpetit/xstring/tree/master   %
% Copyright  : Christian Tellechea 2008-2019                         %
% Licence    : Released under the LaTeX Project Public License v1.3c %
%              or later, see http://www.latex-project.org/lppl.txt   %
% Files      : 1) xstring.tex                                        %
%              2) xstring.sty                                        %
%              3) xstring-fr.tex                                     %
%              4) xstring-fr.pdf                                     %
%              5) xstring-en.tex                                     %
%              6) xstring-en.pdf                                     %
%              7) README                                             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifdefined\usepackage\else
	\immediate\write-1 {Package: xstring \xstringdate\space v\xstringversion\space String manipulations (CT)}%
\fi
\newcount\integerpart
\newcount\decimalpart% compteurs utilis?s par xstring

\edef\restorexstringcatcode{\catcode\number`\_ =\number\catcode`\_\relax}
\catcode`\_=11

\long\def\xs_execfirst#1#2{#1}
\long\def\xs_execsecond#1#2{#2}
\long\def\xs_gobarg#1{}
\expandafter\def\expandafter\xs_gobspace\space{}
\def\xs_deftok#1#2{\let#1= #2\relax}\xs_deftok\xs_sptoken{ }
\long\def\xs_ifnxttok#1#2#3{\xs_deftok\xs_toksmatch{#1}\def\__truecode{#2}\def\__falsecode{#3}\xs_ifnxttok_a}
\def\xs_ifnxttok_a{\futurelet\__futurtok\xs_ifnxttok_b}
\def\xs_ifnxttok_b{%
	\xs_ifx{\__futurtok\xs_sptoken}
	{\afterassignment\xs_ifnxttok_a\let\__futurtok= }
	{\xs_ifx{\__futurtok\xs_toksmatch}\__truecode\__falsecode}%
}
\def\xs_ifstar#1{\xs_ifnxttok*{\xs_execfirst{#1}}}
\long\def\xs_testopt#1#2{\xs_ifnxttok[{#1}{#1[{#2}]}}
\long\def\xs_exparg#1#2{\expandafter\xs_exparg_a\expandafter{#2}{#1}}%
\long\def\xs_exparg_a#1#2{#2{#1}}
\long\def\xs_exptwoargs#1#2#3{\xs_exparg{\xs_exparg{#1}{#2}}{#3}}
\long\def\xs_eearg#1#2{\xs_exparg{\xs_exparg{#1}}{#2}}
\long\def\xs_edefaddtomacro#1#2{\edef#1{\unexpanded\expandafter{#1}#2}}
\long\def\xs_addtomacro#1#2{\xs_exparg{\def#1}{#1#2}}
\long\def\xs_eaddtomacro#1#2{\xs_exparg{\xs_addtomacro#1}{#2}}
\long\def\xs_eeaddtomacro#1#2{\xs_exparg{\xs_eaddtomacro#1}{#2}}
\long\def\xs_endgroup_eaddtomacro#1#2{\xs_exparg{\endgroup\xs_addtomacro#1}{#2}}
\long\def\xs_beforespace#1 #2\_nil{#1}
\long\def\xs_afterspace#1 #2\_nil{#2}
\long\def\xs_gobtonil#1\_nil{}
\long\def\xs_gobtobrace#1#{}
\long\def\xs_ifx#1{\ifx#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\def\xs_ifnum#1{\ifnum#1\expandafter\xs_execfirst\else\expandafter\xs_execsecond\fi}
\long\def\xs_ifempty#1{\expandafter\xs_ifx\expandafter{\expandafter\relax\detokenize{#1}\relax}}

\def\xs_toks_toverb{% lit 1 argument et le transforme en verb
\begingroup
\def\do##1{\catcode`##112 }%
\dospecials
\obeyspaces
\xs_read_verb
}

\def\setverbdelim#1{% d?finit quel est le d?limiteur de verb
\xs_exparg\xs_ifempty{\xs_gobarg#1}%
{}
{\errmessage{Package xstring Warning: verb delimiter "\detokenize{#1}" is not a single token}}%
\def\xs_read_verb##1#1##2#1{\endgroup\xs_assign_verb{##2}}% on appelle l'ex?cution de fin
}

% Assigne l'argument entre d?limiteur verb dans la sc #1
\def\verbtocs#1{%
\def\xs_assign_verb##1{\def#1{##1}}%
\xs_toks_toverb
}

\begingroup
\catcode0 3 \gdef\xs_twozeroschars{^^00}%
\catcode0 7 \xdef\xs_twozeroschars{\xs_twozeroschars^^00}%
\endgroup

\edef\xs_reserved_A{\long\def\noexpand\xs_assigntokenizeresult##1\xs_twozeroschars}
\xs_reserved_A#2{\endgroup\xs_exparg{\def#2}{\xs_gobarg#1}}

\def\tokenize#1#2{%
	\begingroup
	\xs_def\xs_reserved_A{#2}% on d?veloppe en accord avec \fullexpandarg ou \noexpandarg
	\everyeof\expandafter{\xs_twozeroschars#1}%
	\endlinechar-1
	\expandafter\xs_assigntokenizeresult\scantokens\expandafter{\expandafter\relax\xs_reserved_A}% on fait l'assignation
}%

\long\def\xs_assign_xstringresult#1#2{\xs_ifempty{#2}{#1}{\def#2{#1}}}

\def\xs_ldef{\long\def}
\def\xs_ledef{\long\edef}

\def\normalexpandarg{%
\let\xs_def\xs_ldef% on d?finit \xs_call avec \def
\def\xs_expand##1{\unexpanded\expandafter{##1}}%
}
\let\noexpandarg\normalexpandarg% synonyme

\def\expandarg{%
\let\xs_def\xs_ldef% on d?finit \xs_call avec \def
\def\xs_expand##1{\unexpanded\expandafter\expandafter\expandafter{##1}}%
}

\def\fullexpandarg{%
\let\xs_def\xs_ledef% on d?finit\xs_call avec \edef
\def\xs_expand##1{##1}% et on neutralise \xs_expand
}

\def\saveexpandmode{\let\xs_saved_def\xs_defarg\let\xs_saved_expand\xs_expand}
\def\restoreexpandmode{\let\xs_defarg\xs_saved_def\let\xs_expand\xs_saved_expand}

% Macro interne renvoyant #2 si son argument commence par une accolade ouvrante "{"
% et #3 sinon (Ulrich Diez sur comp.text.tex)
\long\def\xs_ifbeginwithbrace#1{%
	\csname xs_exec%
	\expandafter\xs_gobarg\string{%
		\expandafter\xs_gobarg\expandafter{\expandafter{\string#1}%
			\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_execfirst
			\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\xs_gobarg
			\expandafter\expandafter\expandafter\xs_gobarg
			\expandafter\expandafter\expandafter{\expandafter\string\expandafter}\string}%
		\expandafter\xs_gobarg\string}%
	\xs_execsecond{first}{second}%
	\endcsname
}

% Cette macro interne prend la 1ere unit? syntaxique de #1 et assigne le r?sultat ? #2
\long\def\xs_returnfirstsyntaxunit#1#2{%
	\let\xs_toks\relax
	\xs_ifempty{#1}
	{\let#2\empty
	}
	{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
		{\def#2{ }}
		{\xs_ifbeginwithbrace{#1}
			{\def\xs_groupfound{\xs_exparg{\def#2}{\expandafter{#2}}\xs_gobtonil}% on met #2 dans des accolades et on finit
				\let\xs_toks\bgroup
				\afterassignment\xs_groupfound
				\def#2%
			}
			{\long\def\xs_assignfirstarg##1##2\_nil{\def#2{##1}}%
				\xs_assignfirstarg
			}%
			#1\_nil
		}%
	}%
}

\long\def\xs_removefirstsyntaxunit#1#2{%
	\xs_ifempty{#1}
	{\let#2\empty
	}
	{\xs_eearg\xs_ifempty{\expandafter\xs_beforespace\detokenize{#1} \_nil}% #1 commence par un espace ?
		{\xs_exparg\xs_ifbeginwithbrace{\xs_gobspace#1}
			{\xs_exparg{\def#2}{\xs_gobtobrace#1}}%
			{\xs_exparg{\def#2}{\xs_afterspace#1\_nil}}%
		}%
		{\xs_exparg{\def#2}{\xs_gobarg#1}}%
	}%
}

% Cette macro interne est utilis?e dans les macros ?toil?es pour :
% 1) d?velopper l'argument selon qu'on a choisit \fullexpandarg
%    ou \normalexpandarg, et ceci ? l'aide de la macro \xs_def
% 2) Ensuite, on d?tokenize ce d?veloppement de fa?on n'avoir plus que
%    des catcodes de 10 pour les espaces et 12 pour le reste.
\long\def\xs_expand_and_detokenize#1#2{%
	\long\def#1{#2}%
	\expandafter\edef\expandafter#1\expandafter{\xs_expand#1}% on d?veloppe #2 selon le mode de d?veloppement
	\long\edef#1{\detokenize\expandafter{#1}}% puis on d?tokenize et on assigne ? #1
}

\long\def\xs_expand_and_assign#1#2{\xs_def#1{#2}}% on d?veloppe #2 selon \fullexpandarg ou \normalexpandarg

\def\xs_arglist{0########1########2########3########4########5########6########7########8########9}

% \xs_assign_args{3} met dans la sc \xs_myarg les tokens "####1####2####3"
\def\xs_assign_args#1{\def\xs_assign_args_i0##1#1##2\_nil{\def\xs_myarg{##1#1}}\expandafter\xs_assign_args_i\xs_arglist\_nil}

% \xs_assign_opt_args{3} met dans la sc \xs_myarg les tokens "[####1]####2####3####4"
\def\xs_assign_opt_args#1{\xs_exparg\xs_assign_opt_args_i{\number\numexpr#1+1}}
\def\xs_assign_opt_args_i#1{\def\xs_assign_opt_args_ii0##11##2#1##3\_nil{\def\xs_myarg{[##11]##2#1}}\expandafter\xs_assign_opt_args_ii\xs_arglist\_nil}

% \xs_assign_one_arg{3} met dans la sc \xs_myarg les tokens "####3"
\def\xs_assign_one_arg#1{\xs_exparg\xs_assign_one_arg_i{\number\numexpr#1-1}{#1}}
\def\xs_assign_one_arg_i#1#2{\def\xs_assign_one_arg_ii##1#1##2#2##3\_nil{\def\xs_myarg{##2#2}}\expandafter\xs_assign_one_arg_ii\xs_arglist\_nil}

% #1 : num?ro du 1er argument; #2 : nombre de lignes; #3 argument optionnel; #4 : dernier num?ro de l'argument devant ?tre d?tokenis? si ?toile
\def\xs_buildlines#1#2#3#4{%
\let\xs_newlines\empty
\let\xs_newargs\empty
\def\xs_buildlines_i##1{%
\xs_exparg\xs_assign_one_arg{\number\numexpr##1+#1-1}%
\edef\xs_reserved_B{\noexpand\xs_expand\csname xs_arg_\romannumeral\numexpr##1\endcsname}%
\xs_ifnum{##1=1 }% si c'est le premier argument
{\xs_ifempty{#3}%
	{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
		\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
	}% et s'il y a un argument optionnel alors, on met des crochets
	{\xs_eaddtomacro\xs_newargs{\expandafter[\xs_reserved_B]}%
		\def\xs_reserved_B{xs_def}% ne pas d?tok?niser l'argument optionnel grace au \xs_def
	}%
}
{\xs_eaddtomacro\xs_newargs{\expandafter{\xs_reserved_B}}%
	\edef\xs_reserved_B{\ifnum##1>#4 xs_def\else xs_assign\fi}%
}%
\edef\xs_newlines{\unexpanded\expandafter{\xs_newlines}\expandafter\noexpand\csname\xs_reserved_B\endcsname\expandafter\noexpand\csname xs_arg_\romannumeral\numexpr##1\endcsname{\xs_myarg}}%
\xs_ifnum{##1<#2 }
{\xs_exparg\xs_buildlines_i{\number\numexpr##1+1}}
{}%
}%
\xs_buildlines_i1%
}

\def\xs_newmacro{%
	\xs_ifstar
	{\let\xs_reserved_D\empty\xs_newmacro_}
	{\let\xs_reserved_D\relax\xs_newmacro_0}%
}

% #1 : dernier num?ro de l'argument devant ?tre d?tokenis?
% #2 : nom de la macro publique
% #3 : argument optionnel (vide si pas d'arg optionnel)
% #4 : nombre d'arguments obligatoires
% #5 : utilisation de testopt (1 si oui, 0 si non)
% #6 : code de la macro
\def\xs_newmacro_#1#2#3#4#5{%
	\edef\xs_reserved_A{xs_\expandafter\xs_gobarg\string#2}%
	\edef\xs_reserved_C{\expandafter\noexpand\csname\xs_reserved_A _\ifx\empty#3\empty _\fi\endcsname}%
	\edef\xs_reserved_B{%
		\long
		\ifx\empty\xs_reserved_D
			\def\noexpand#2{\noexpand\xs_ifstar
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_detokenize\expandafter\noexpand\xs_reserved_C}%
				{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
			}%
		\else
			\def\noexpand#2{\let\noexpand\xs_assign\noexpand\xs_expand_and_assign\expandafter\noexpand\xs_reserved_C}%
		\fi
		\ifx\empty#3\empty
		\else
			\def\expandafter\noexpand\xs_reserved_C{%
				\noexpand\xs_testopt{\expandafter\noexpand\csname\xs_reserved_A __\endcsname}{\ifx\xs_def\xs_ledef#3\else\unexpanded{#3}\fi}}%
		\fi
	}%
	% Que fait \xs_reserved_B ? Il d?finit :
	% si #3 est vide : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM__}{\let\xs_assign\xs_expand_and_assign\xs_NOM__}}
	% si #3 existe   : \NOM{\xs_ifstar{\let\xs_assign\xs_expand_and_detokenize\xs_NOM_}{\let\xs_assign\xs_expand_and_assign\xs_NOM_}}
	%                  \xs_NOM_{\xs_testopt{\xs_NOM__}{#3}}}
	\xs_reserved_B
	\ifx\empty#3\empty
		\xs_buildlines1{#4}{#3}{#1}%
		\xs_assign_args{#4}%
	\else
		\xs_exparg{\xs_buildlines1}{\number\numexpr#4+1}{#3}{#1}%
		\xs_assign_opt_args{#4}%
	\fi
	\edef\xs_reserved_B{\def\expandafter\noexpand\csname\xs_reserved_A __\endcsname\xs_myarg}%
	\edef\xs_reserved_C{\unexpanded\expandafter{\xs_newlines}\edef\noexpand\xs_call}%
	\edef\xs_reserved_D{\noexpand\noexpand\expandafter\noexpand\csname\xs_reserved_A\endcsname\unexpanded\expandafter{\xs_newargs}}%
	\ifnum#5=1 \edef\xs_reserved_D{\noexpand\noexpand\noexpand\xs_testopt{\unexpanded\expandafter{\xs_reserved_D}}{}}\fi
	\xs_edefaddtomacro\xs_reserved_C{{\unexpanded\expandafter{\xs_reserved_D}}\noexpand\xs_call}%
	\xs_edefaddtomacro\xs_reserved_B{{\unexpanded\expandafter{\xs_reserved_C}}}%
	% Que fait \xs_reserved_B ? Il d?finit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def\xs_NOM__[##2]##3##4##5{%
	%          \xs_def\xs_arg_i{##2}\xs_assign\xs_arg_ii{##3}\xs_assign\xs_arg_iii{##4}\xs_asign\xs_arg_iv{##5}%
	% si #5=0: \edef\xs_call{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}%
	% si #5=1: \edef\xs_call{\noexpand\xs_testopt{\noexpand\xs_NOM[\xs_expand\xs_arg_i]{\xs_expand\xs_arg_i}{\xs_expand\xs_arg_ii}{\xs_expand\xs_arg_iii}{\xs_expand\xs_arg_iv}}{}}%
	%          \xs_call}
	\long\xs_reserved_B
	\edef\xs_reserved_B{%
		\def\expandafter\noexpand\csname\xs_reserved_A\endcsname
		\xs_myarg\ifnum#5=1 [\unexpanded{##}\number\numexpr\ifx\empty#3\empty#4+1\else#4+2\fi]\fi
	}%
	% Que fait \xs_reserved_B ? Il d?finit par exemple pour 3 arguments obligatoires et 1 facultatif :
	%    \def \xs_NOM[##2]##3##4##5[##6]{#6}
	\long\xs_reserved_B
}

% macro g?n?rique qui lit \xs_reserved_C us par us
% 3 sous-routines sont appel?es ? des moments cl? :
% \xs_atendofgroup      (un groupe se finit, appel r?cursif)
% \xs_atbegingroup      (un groupe vient d'?tre ouvert)
% \xs_atnextsyntaxunit  (la future US n'est pas un groupe)
\def\xs_read_reserved_C{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\xs_atendofgroup
			\xs_read_reserved_C
		}%
	}
	{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exploregroups
		\xs_ifx{\bgroup\xs_toks}
		{\advance\integerpart1
			\begingroup
			\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
			\xs_calc_grouIP
			\def\xs_nestlevel{1}%
			\integerpart0
			\xs_atbegingroup
		}
		{\advance\decimalpart1
			\xs_atnextsyntaxunit
		}%
		\xs_read_reserved_C
	}%
}

% macro g?n?rique qui lit \xs_reserved_D en proc?dant ? des tests avec \IfBeginWith
% 1 sous-routine est appel?e :
% \xs_atoccurfound      (une occurrence a ?t? trouv?e)
\def\xs_read_reserved_D{%
	\xs_exparg\xs_ifempty{\xs_reserved_D}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_C}{{\unexpanded\expandafter{\xs_reserved_C}}}%
			}%
			\__temp
			\xs_read_reserved_D
		}%
	}%
	{\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_D\xs_reserved_E
		{\advance\decimalpart1
			\let\xs_reserved_D\xs_reserved_A
			\xs_atoccurfound
		}%
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_A
			\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
			\xs_exploregroups
			\xs_ifx{\bgroup\xs_toks}
			{\advance\integerpart1
				\begingroup
				\expandafter\def\expandafter\xs_reserved_D\xs_reserved_A
				\xs_calc_grouIP
				\let\xs_reserved_C\empty
				\def\xs_nestlevel{1}%
				\integerpart0
			}
			{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
			}%
		}%
		\xs_read_reserved_D
	}%
}

\xs_newmacro\StrRemoveBraces{}{1}{1}{%
	\def\xs_reserved_C{#1}%
	\let\xs_reserved_B\empty
	\def\xs_nestlevel{0}%
	\xs_StrRemoveBraces_i
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#2}%
}

\def\xs_StrRemoveBraces_i{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\xs_ifnum{\xs_nestlevel=0 }
		{}
		{\xs_endgroup_eaddtomacro\xs_reserved_B\xs_reserved_B
			\xs_StrRemoveBraces_i
		}%
	}
	{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_ifx{\bgroup\xs_toks}
		{\xs_ifx{\xs_exploregroups\relax}% on explore les groupes ?
			{\begingroup
				\expandafter\def\expandafter\xs_reserved_C\xs_reserved_A
				\def\xs_nestlevel{1}%
				\let\xs_reserved_B\empty
			}
			{\expandafter\xs_addtomacro\expandafter\xs_reserved_B\xs_reserved_A
			}%
		}
		{\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
		}%
		\xs_StrRemoveBraces_i
	}%
}

% \xs_cutafteroccur coupe l'argument #1 apr?s la #3?me occurrence de #2
% \xs_reserved_C : contient ce qui se trouve avant cette occurrence
% \xs_reserved_D : contient ce qui se trouve avant cette occurrence y compris cette occurrence
% \xs_reserved_E : contient ce qui se trouve apr?s l'occurrence
% si l'occurrence n'existe pas ou qu'un des arguments est vide, toutes les chaines renvoy?es sont vides
\long\def\xs_cutafteroccur#1#2#3{%
	\xs_ifnum{#3<1 }
	{\let\xs_reserved_C\empty\let\xs_reserved_E\empty\gdef\groupID{}}
	{\xs_cutafteroccur_i{#1}{#2}{#3}}%
}

\long\def\xs_cutafteroccur_i#1#2#3{%
	\def\xs_reserved_D{#1}\let\xs_reserved_C\empty\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
		{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
			}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% mange l'appel r?cursif \xs_read_reserved_D dans \xs_read_reserved_D
		}
		{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
		}%
	}%
	\xs_read_reserved_D
	\xs_ifnum{\decimalpart=\numexpr(#3)\relax}% occurrence trouv?e ?
	{\let\xs_reserved_E\xs_reserved_D
		\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
	}
	{\let\xs_reserved_C\empty
		\let\xs_reserved_E\empty
		\gdef\groupID{}%
	}%
}

\xs_newmacro*3\IfSubStr{1}{2}{0}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_ifempty{\xs_reserved_D}\xs_execsecond\xs_execfirst
}

\xs_newmacro*2\IfBeginWith{}{2}{0}{%
	\xs_ifempty{#2}%
	{\xs_execsecond}
	{\xs_IfBeginWith_i{#1}{#2}}%
}

\long\def\xs_IfBeginWith_i#1#2{%
	\xs_ifempty{#2}%
	{\xs_execfirst% #2 est vide, tous les tests sont pass?s avec succ?s : on renvoie #3
	}
	{\xs_ifempty{#1}%
		{\xs_execsecond% #1 est vide, c'est que #2 est + long que #1 : on renvoie #4
		}
		{\xs_returnfirstsyntaxunit{#2}\xs_reserved_B
			\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
			\xs_ifx{\xs_reserved_A\xs_reserved_B}% il y a ?galit?...
			{\xs_removefirstsyntaxunit{#2}\xs_reserved_B
				\xs_removefirstsyntaxunit{#1}\xs_reserved_A% on enl?ve les 1ere unit?s syntaxiques
				\xs_exptwoargs\xs_IfBeginWith_i\xs_reserved_A\xs_reserved_B
			}
			{\xs_execsecond
			}%
		}%
	}%
}

\xs_newmacro*2\IfEndWith{}{2}{0}{%
	\xs_ifempty{#2}%
	{\xs_execsecond
	}
	{\xs_StrCount{#1}{#2}[\xs_reserved_A]%
		\xs_ifnum{\xs_reserved_A=0 }
		{\xs_execsecond}
		{\xs_exparg\xs_ifempty{\xs_reserved_C}}%
	}%
}

\xs_newmacro*4\IfSubStrBefore{1,1}{3}{0}{\xs_IfSubStrBefore_i[#1]{#2}{#3}{#4}}

\def\xs_IfSubStrBefore_i[#1,#2]#3#4#5{%
	\def\xs_reserved_C{#3}%
	\xs_ifx{\xs_exploregroups\relax}% si on explore les groupes
	{\let\xs_reserved_B\empty
		\def\xs_nestlevel{0}%
		\xs_StrRemoveBraces_i% on retire les accolades
		\let\xs_reserved_C\xs_reserved_B
	}
	{}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#5}{#2}%
	\xs_exparg\xs_cutafteroccur\xs_reserved_C{#4}{#1}%
	\gdef\groupID{}%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	\xs_execsecond
	\xs_execfirst
}

\xs_newmacro*4\IfSubStrBehind{1,1}{3}{0}{\xs_IfSubStrBehind_i[#1]{#2}{#3}{#4}}
\long\def\xs_IfSubStrBehind_i[#1,#2]#3#4#5{\xs_IfSubStrBefore_i[#2,#1]{#3}{#5}{#4}}

\long\def\xs_formatnumber#1#2{%
	\xs_ifempty{#1}%
	{\def#2{0X}% si vide, renvoie 0X
	}
	{\xs_returnfirstsyntaxunit{#1}\xs_reserved_A
		\def\xs_reserved_B{+}%
		\xs_ifx{\xs_reserved_A\xs_reserved_B}
		{\xs_removefirstsyntaxunit{#1}\xs_reserved_C
			\xs_exparg\xs_ifempty{\xs_reserved_C}%
			{\def#2{+0X}}
			{\xs_exparg{\def#2}{\expandafter+\expandafter0\xs_reserved_C}}%
		}
		{\def\xs_reserved_B{-}%
			\xs_ifx{\xs_reserved_A\xs_reserved_B}
			{\xs_removefirstsyntaxunit{#1}\xs_reserved_A
				\xs_exparg\xs_ifempty{\xs_reserved_A}%
				{\def#2{-0X}}%
				{\xs_exparg{\def#2}{\expandafter-\expandafter0\xs_reserved_A}}%
			}
			{\def#2{0#1}%
			}%
		}%
	}%
}

\xs_newmacro\IfInteger{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\let\xs_after_intpart\afterinteger
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
	{\xs_ifnum{\decimalpart=0 }
		{\xs_execfirst% partie d?cimale constitu?e de 0 --> seul cas o? on renvoie vrai
		}
		{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
			\xs_execsecond
		}%
	}
	{\expandafter\xs_defafterinteger\xs_after_intpart\relax\_nil
		\xs_execsecond
	}%
}

\xs_newmacro\IfDecimal{}{1}{0}{%
	\xs_formatnumber{#1}\xs_reserved_A
	\decimalpart0
	\afterassignment\xs_defafterinteger\integerpart\xs_reserved_A\relax\_nil
	\expandafter\xs_testdot\afterinteger\_nil
	\xs_ifx{\empty\afterdecimal}
}

\begingroup\catcode`\@ 11
\long\gdef\xs_defafterinteger#1\relax\_nil{\def\@xs@afterinteger{#1}\let\afterinteger\@xs@afterinteger}
\long\gdef\xs_defafterdecimal#1\_nil{\def\@xs@afterdecimal{#1}\let\afterdecimal\@xs@afterinteger}
\endgroup

\def\xs_testdot{%
\let\xs_decsep\empty
\xs_ifnxttok.
{\def\xs_decsep{.}\xs_readdecimalpart}%
{\xs_testcomma}%
}

\def\xs_testcomma{%
	\xs_ifnxttok,
	{\def\xs_dessep{,}\xs_readdecimalpart}%
		{\xs_defafterdecimal}%
}

\long\def\xs_readdecimalpart#1#2\_nil{%
	\xs_ifempty{#2}
	{\def\xs_reserved_A{0X}}
	{\def\xs_reserved_A{0#2}}%
	\afterassignment\xs_defafterinteger\decimalpart\xs_reserved_A\relax\_nil
	\expandafter\xs_defafterdecimal\afterinteger\_nil
}

% test d'?galit? sur des chaines (et des chaines contenant des nombres)
\long\def\xs_IfStrEqFalse_i#1#2{\let\xs_reserved_A\xs_execsecond}
\long\def\xs_IfStrEqFalse_ii#1#2{% renvoie vrai si les 2 arg sont d?cimaux et s'ils sont ?gaux, faux sinon
	\xs_IfDecimal{#1}%
	{\xs_IfDecimal{#2}%
		{\ifdim#1pt=#2pt
				\let\xs_reserved_A\xs_execfirst
			\else
				\let\xs_reserved_A\xs_execsecond
			\fi% les 2 sont d?cimaux : on fait le test
		}%
		{\let\xs_reserved_A\xs_execsecond}% un seul est d?cimal
	}%
	{\let\xs_reserved_A\xs_execsecond}% #1 n'est pas d?cimal
}

\long\def\xs_TestEqual#1#2{% teste si les 2 arguments sont ?gaux
	\def\xs_reserved_A{#1}\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
	{\let\xs_reserved_A\xs_execfirst}% ?galit? parfaite des 2 chaines
	{\xs_reserved_D{#1}{#2}}%
	\xs_reserved_A
}

\xs_newmacro*2\IfStrEq{}{2}{0}{% teste si les deux chaines sont ?gales
	\let\xs_reserved_D\xs_IfStrEqFalse_i
	\xs_TestEqual{#1}{#2}%
}

\xs_newmacro*2\IfEq{}{2}{0}{% teste si les 2 arguments (chaine ou nombre) sont ?gaux
	\let\xs_reserved_D\xs_IfStrEqFalse_ii
	\xs_TestEqual{#1}{#2}%
}

\def\IfStrEqCase{%
	\xs_ifstar
	{\xs_IfStringCase{\IfStrEq*}}%
	{\xs_IfStringCase\IfStrEq}%
}

\def\IfEqCase{%
	\xs_ifstar
	{\xs_IfStringCase{\IfEq*}}%
	{\xs_IfStringCase\IfEq}%
}

\long\def\xs_IfStringCase#1#2#3{% #1=macro avec ou sans ?toile  #2=argument ? tester  #3=liste des {<cas>}{code>}
	\long\def\xs_testcase##1##2##3\_nil{% lit les 2 premieres unit?s syntaxiques dans ##1 et ##2. Les autres dans ##3
		#1{#2}{##1}% compare
			{\xs_testopt{\xs_IfStringCase_ii{##2}}{}}% le test est positif, on ex?cute le code correspondant et on mange l'argument optionnel ## BUGfix dans 1.82
			{\xs_ifempty{##3}%
				{\xs_testopt{\xs_IfStringCase_i}{}}% s'il n'y a plus de cas, on ex?cute le code <autres cas> ## BUGfix dans 1.82
				{\xs_testcase##3\_nil}% sinon, on recommence avec ce qui reste
			}%
	}%
	\xs_testcase#3\_nil
}

\long\def\xs_IfStringCase_i[#1]{#1}
\long\def\xs_IfStringCase_ii#1[#2]{#1}

% Renvoie ce qui est ? gauche de l'occurence n?#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBefore{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#4}%
}

% Renvoie ce qui est ? droite de l'occurence n?#1 de la sous chaine #3 dans la chaine #2
\xs_newmacro*3\StrBehind{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_E}{#4}%
}

% Renvoie ce qui est strictement compris entre les occurrences n?#1 et n?#2
% des chaines #4 et #5 dans la chaine #3
\xs_newmacro*4\StrBetween{1,1}{3}{1}{\xs_StrBetween_i[#1]{#2}{#3}{#4}[#5]}
\long\def\xs_StrBetween_i[#1,#2]#3#4#5[#6]{%
	\begingroup
	\noexploregroups
	\xs_cutafteroccur{#3}{#5}{#2}%
	\xs_exparg\xs_cutafteroccur{\xs_reserved_C}{#4}{#1}%
	\expandafter
	\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_E}{#6}%
	\gdef\groupID{}%
}

\def\exploregroups{\let\xs_exploregroups\relax}
\def\noexploregroups{\def\xs_exploregroups{\let\xs_toks\relax}}
\def\saveexploremode{\let\xs_saveexploremode\xs_exploregroups}
\def\restoreexploremode{\let\xs_exploregroups\xs_saveexploremode}

% Remplace les #1 premi?res occurences de la chaine #3
% par la chaine #4 dans la chaine #2
\xs_newmacro\StrSubstitute{0}{3}{1}{%
	\def\xs_reserved_D{#2}\let\xs_reserved_C\empty\def\xs_reserved_E{#3}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{#1<1 }
		{\def\xs_reserved_A{#4}}
		{\xs_ifnum{\decimalpart>#1 }
			{\def\xs_reserved_A{#3}}
			{\def\xs_reserved_A{#4}}%
		}%
		\xs_eaddtomacro\xs_reserved_C{\xs_reserved_A}%
	}%
	\xs_ifempty{#3}%
	{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#5}%
	}
	{\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#5}%
	}%
}

% Supprime les #1 premi?res occurrences de #3 dans #2
\xs_newmacro\StrDel{0}{2}{1}{\xs_StrSubstitute[#1]{#2}{#3}{}[#4]}

\def\xs_exitallgroups{\ifnum\xs_nestlevel>0 \endgroup\expandafter\xs_exitallgroups\fi}

% Compte combien d'unit?s syntaxiques contient la chaine #1 ?
\xs_newmacro\StrLen{}{1}{1}{%
	\def\xs_reserved_C{#1}\decimalpart0 \def\xs_nestlevel{0}\gdef\groupID{0}%
	\let\xs_atbegingroup\relax
	\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
	\let\xs_atnextsyntaxunit\relax
	\xs_read_reserved_C
	\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#2}%
}

% Macro interne fermant autant de groupes que n?cessaire pour trouver une unit? syntaxique derri?re
\def\xs_continuetonext{%
	\xs_exparg\xs_ifempty{\xs_reserved_C}%
	{\ifnum\xs_nestlevel>0
			\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}% on concat?ne
			\expandafter\xs_continuetonext% on recommence
		\fi}
	{}%
}%

\def\xs_calc_grouIP{%
	\begingroup\def\xs_reserved_A{0}%
	\xs_ifx{\xs_reserved_A\groupID}% si on arrive du groupe de niveau 0
	{\endgroup\xdef\groupID{\number\integerpart}}% on met simplement le niveau
	{\endgroup\xs_eearg{\gdef\groupID}{\expandafter\groupID\expandafter,\number\integerpart}}%
}

% Cette macro coupe la chaine #1 apr?s l'unit? syntaxique n?#2
\def\StrSplit{%
	\xs_ifstar
	{\let\xs_reserved_E\xs_continuetonext\StrSplit_i}%
	{\let\xs_reserved_E\relax\StrSplit_i}%
}

\xs_newmacro\StrSplit_i{}{2}{0}{\xs_StrSplit_ii{#2}{#1}\xs_StrSplit_iii}

% Cette macro interne coupe la chaine #2 apr?s l'unit? syntaxique n?#1
% Le d?but est assign? dans \xs_reserved_B et la fin dans \xs_reserved_C
\long\def\xs_StrSplit_ii#1#2{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#2}\def\xs_reserved_D{#1}\gdef\groupID{}%
	\ifnum#1>0
		\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{%
			\edef\__temp{%
				\endgroup
				\noexpand\decimalpart=\number\decimalpart\relax
				\unexpanded{\xs_addtomacro\xs_reserved_B}{{\unexpanded\expandafter{\xs_reserved_B}}}%
			}%
			\__temp
		}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{%
			\xs_eaddtomacro\xs_reserved_B{\xs_reserved_A}%
			\xs_ifnum{\decimalpart=\xs_reserved_D\relax}
			{\ifx\xs_reserved_C\empty\xs_reserved_E\fi
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_B}}\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}}%
				\expandafter\xs_exitallgroups\__temp
				\xs_gobarg% mange l'appel r?cursif \xs_read_reserved_C dans \xs_read_reserved_C
			}
			{}%
		}%
		\xs_read_reserved_C
	\fi
}

\def\xs_StrSplit_iii#1#2{\let#1\xs_reserved_B\let#2\xs_reserved_C}

% StrCut[n]{<texte>}{<motif>}\macroA\macroB
% \macroA re?oit ce qui se trouve avant la n ?me occurrence <motif> dans <texte>
% \macroB re?oit ce qui est apr?s cette n ?me occurrence
\xs_newmacro*3\StrCut{1}{2}{0}{%
	\xs_ifempty{#3}%
	{\gdef\groupID{}\let\xs_reserved_C\empty\let\xs_reserved_E\empty
	}
	{\xs_ifnum{#1<1 }
		{\xs_StrCut_ii{#2}{#3}1}
		{\xs_StrCut_ii{#2}{#3}{#1}}%
	}%
	\xs_StrCut_iii
}

\long\def\xs_StrCut_ii#1#2#3{%
	\let\xs_reserved_C\empty\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}%
	\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
	\def\xs_atoccurfound{%
		\xs_ifnum{\decimalpart=\numexpr(#3)\relax}
		{\edef\__temp{%
				\def\noexpand\xs_reserved_C{\unexpanded\expandafter{\xs_reserved_C}}%
				\def\noexpand\xs_reserved_D{\unexpanded\expandafter{\xs_reserved_D}}%
				\noexpand\decimalpart=\number\decimalpart\relax
			}%
			\expandafter\xs_exitallgroups\__temp
			\xs_gobarg% stoppe la r?cursivit? dans \xs_read_reserved_D
		}
		{\xs_eaddtomacro\xs_reserved_C{\xs_reserved_E}%
		}%
	}%
	\xs_read_reserved_D
	\let\xs_reserved_E\xs_reserved_D
	\xs_exparg{\def\xs_reserved_D}{\xs_reserved_C#2}%
}

\long\def\xs_StrCut_iii#1#2{\let#1\xs_reserved_C\let#2\xs_reserved_E}

% De la chaine #1, renvoie ce qui se trouve entre les positions
%  #2 et #3, unit?s syntaxiques aux positions compris !
\xs_newmacro\StrMid{}{3}{1}{%
	\begingroup
	\noexploregroups
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#3}{#1}%
	\edef\xs_reserved_C{\number\numexpr#2-1}%
	\let\xs_reserved_E\relax
	\xs_exptwoargs\xs_StrSplit_ii\xs_reserved_C\xs_reserved_B
	\expandafter\endgroup
	\expandafter\xs_assign_xstringresult\expandafter{\xs_reserved_C}{#4}%
	\gdef\groupID{}%
}

% supprime #2 unit?s syntaxiques ? gauche dans la chaine #1
\xs_newmacro\StrGobbleLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

% extrait de #1 la chaine ? gauche de longueur #2
\xs_newmacro\StrLeft{}{2}{1}{%
	\let\xs_reserved_E\relax
	\xs_StrSplit_ii{#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% supprime #2 unit?s syntaxiques ? droite dans la chaine #1
\xs_newmacro\StrGobbleRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% renvoie #2 unit?s syntaxiques ? la droite de la chaine #1
\xs_newmacro\StrRight{}{2}{1}{%
	\xs_StrLen{#1}[\xs_reserved_D]%
	\let\xs_reserved_E\relax
	\xs_exparg\xs_StrSplit_ii{\number\numexpr\xs_reserved_D-#2}{#1}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_C}{#3}%
}

\xs_newmacro\StrChar{}{2}{1}{%
	\let\xs_reserved_B\empty\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
	\ifnum#2>0
		\def\groupID{0}\def\xs_nestlevel{0}\integerpart0 \decimalpart0
		\let\xs_atbegingroup\relax
		\def\xs_atendofgroup{\expandafter\endgroup\expandafter\decimalpart\number\decimalpart\relax}%
		\def\xs_atnextsyntaxunit{%
			\ifnum\decimalpart=\xs_reserved_D% la n i?me US est atteinte ?
				\edef\__temp{\def\noexpand\xs_reserved_B{\unexpanded\expandafter{\xs_reserved_A}}}% on capture l'US en cours qui est celle cherch?e
				\expandafter\xs_exitallgroups\__temp
				\expandafter\xs_gobarg% stoppe la r?cursivit? dans \xs_read_reserved_C
			\fi
		}%
		\xs_read_reserved_C
	\fi
	\xs_exparg\xs_ifempty{\xs_reserved_B}%
	{\gdef\groupID{}}
	{}%
	\xs_exparg\xs_assign_xstringresult{\xs_reserved_B}{#3}%
}

% Combien de fois compte t-on #2 dans #1 ?
\xs_newmacro\StrCount{}{2}{1}{%
	\def\xs_reserved_D{#1}\def\xs_reserved_E{#2}\let\xs_reserved_C\empty
	\xs_ifempty{#2}%
	{\xs_assign_xstringresult{0}{#3}%
	}
	{\decimalpart0 \integerpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atoccurfound{\let\xs_reserved_C\empty\xs_read_reserved_D}%
		\xs_read_reserved_D
		\xs_exparg\xs_assign_xstringresult{\number\decimalpart}{#3}%
	}%
}

% renvoie la position de l'occurrence #1 de la sous chaine #3 dans la chaine #2
\xs_newmacro\StrPosition{1}{2}{1}{%
	\xs_cutafteroccur{#2}{#3}{#1}%
	\let\xs_reserved_E\groupID
	\xs_ifx{\xs_reserved_C\xs_reserved_D}
	{\xs_assign_xstringresult{0}{#4}%
		\let\xs_reserved_E\empty
	}
	{\xs_exparg\xs_StrLen{\xs_reserved_C}[\xs_reserved_C]%
		\xs_exparg\xs_assign_xstringresult{\number\numexpr\xs_reserved_C+1}{#4}%
	}%
	\global\let\groupID\xs_reserved_E
}

\def\comparestrict{\def\xs_comparecoeff{1}}
\def\comparenormal{\def\xs_comparecoeff{0}}
\def\savecomparemode{\let\xs_saved_comparecoeff\xs_comparecoeff}
\def\restorecomparemode{\let\xs_comparecoeff\xs_saved_comparecoeff}

% Compare les deux arguments #1 et #2
% Renvoie 0 s'ils sont ?gaux et renvoie la
% position de la premiere unit? syntaxiques diff?rente sinon
\xs_newmacro*2\StrCompare{}{2}{1}{%
	\def\xs_reserved_A{#1}%
	\def\xs_reserved_B{#2}%
	\xs_ifx{\xs_reserved_B\xs_reserved_A}
	{\xs_assign_xstringresult{0}{#3}}
	{\xs_StrCompare_i{#1}{#2}{#3}}%
}

\long\def\xs_StrCompare_i#1#2#3{%
\def\xs_StrCompare_iii##1{%
\let\xs_reserved_A\empty
\xs_exparg\xs_ifempty{\xs_reserved_C}%
{\edef\xs_reserved_A{*\xs_comparecoeff}}%
{\xs_exparg\xs_ifempty{\xs_reserved_D}%
	{\edef\xs_reserved_A{*\xs_comparecoeff}}
	{}%
}%
\def\xs_next{\xs_exparg\xs_assign_xstringresult{\number\numexpr##1\xs_reserved_A\relax}{#3}}%
}%
\def\xs_StrCompare_ii##1{% ##1 est la position
\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_A
\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_D}\xs_reserved_B
\xs_ifx{\xs_reserved_B\xs_reserved_A}
{\xs_exparg\xs_ifempty{\xs_reserved_A}%
	{\xs_StrCompare_iii{##1}% les 2 unit?s syntaxiques sont ?gales, on renvoie la position
	}
	{\def\xs_next{\xs_exparg\xs_StrCompare_ii{\number\numexpr##1+1}}% les 2 unit?s syntaxiques sont ?gales et non vides, on recommence
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
		\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_D}\xs_reserved_D
	}%
}% les 2 unit?s syntaxiques sont diff?rentes : on renvoie la position
{\xs_StrCompare_iii{##1}%
}%
\xs_next
}%
\def\xs_reserved_C{#1}\def\xs_reserved_D{#2}%
\xs_StrCompare_ii1%
}

\xs_newmacro\StrFindGroup{}{2}{1}{%
	\def\xs_reserved_A{#2}\def\xs_reserved_B{0}%
	\xs_ifx{\xs_reserved_A\xs_reserved_B}
	{\xs_assign_xstringresult{{#1}}{#3}}
	{\xs_StrFindGroup_i{#1}{#2}[#3]}%
}

\long\def\xs_StrFindGroup_i#1#2[#3]{%
	\def\xs_StrFindGroup_ii{%
		\xs_exparg\xs_ifempty{\xs_reserved_C}%
		{\xs_assign_xstringresult{}{#3}% s'il ne reste plus rien, on renvoie vide
		}
		{\xs_exparg\xs_returnfirstsyntaxunit{\xs_reserved_C}\xs_reserved_D
			\xs_ifx{\bgroup\xs_toks}% si la 1?re unit? syntaxique est un groupe explicite
			{\advance\decimalpart1 % on augmente le compteur
				\xs_ifnum{\decimalpart=\xs_reserved_A\relax}% on est au groupe cherch? lors de la profondeur courante ?
				{\xs_ifx{\empty\xs_reserved_B}% on est ? la profondeur maximale ?
					{\xs_exparg\xs_assign_xstringresult{\xs_reserved_D}{#3}}% on renvoie ce groupe
					{\xs_exparg{\expandafter\xs_StrFindGroup_i\xs_reserved_D}{\xs_reserved_B}[#3]}% on recommence avec ce groupe et les profondeurs de recherche restantes
				}
				{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
					\xs_StrFindGroup_ii
				}%
			}
			{\xs_exparg\xs_removefirstsyntaxunit{\xs_reserved_C}\xs_reserved_C
				\xs_StrFindGroup_ii
			}%
		}%
	}%
	\xs_extractgroupnumber{#2}\xs_reserved_A\xs_reserved_B
	\decimalpart0
	\xs_ifnum{\xs_reserved_A>0 }
	{\def\xs_reserved_C{#1}}
	{\let\xs_reserved_C\empty}%
	\xs_StrFindGroup_ii
}

\def\xs_extractgroupnumber#1#2#3{%
	\def\xs_extractgroupnumber_i##1,##2\_nil{\def#2{##1}\def#3{##2}}%
	\xs_extractgroupnumber_i#1,\_nil
	\ifx\empty#3\else\xs_extractgroupnumber_i#1\_nil\fi
}

\def\expandingroups{\let\xs_expandingroups\exploregroups}

\def\noexpandingroups{\let\xs_expandingroups\noexploregroups}

\def\StrExpand{\xs_testopt{\xs_StrExpand}{1}}
\long\def\xs_StrExpand[#1]#2#3{%
	\begingroup
	\xs_expandingroups
	\xs_ifnum{#1>0 }
	{\integerpart#1 \decimalpart0 \gdef\groupID{0}\def\xs_nestlevel{0}%
		\def\xs_atendofgroup{\xs_endgroup_eaddtomacro\xs_reserved_B{\expandafter{\xs_reserved_B}}}%
		\def\xs_atbegingroup{\let\xs_reserved_B\empty}%
		\def\xs_atnextsyntaxunit{\xs_eeaddtomacro\xs_reserved_B{\xs_reserved_A}}%
		\def\xs_reserved_C{#2}%
		\xs_StrExpand_i{#1}% Appel de la macro r?cursive
	}
	{\def\xs_reserved_B{#2}%
	}
	\expandafter
	\endgroup
	\expandafter\def\expandafter#3\expandafter{\xs_reserved_B}%
	\gdef\groupID{}%
}

\long\def\xs_StrExpand_i#1{%
	\xs_ifnum{#1>0 }
	{\let\xs_reserved_B\empty
		\xs_read_reserved_C
		\let\xs_reserved_C\xs_reserved_B
		\def\xs_reserved_A{\xs_exparg\xs_StrExpand_i{\number\numexpr#1-1}}%
	}
	{\let\xs_reserved_A\relax
	}%
	\xs_reserved_A
}

\def\scancs{\xs_testopt{\xs_scancs}{1}}
\long\def\xs_scancs[#1]#2#3{%
	\xs_StrExpand[#1]{#3}{#2}%
	\edef#2{\detokenize\expandafter{#2}}%
}

\restorexstringcatcode

\setverbdelim{|}%
\fullexpandarg\saveexpandmode
\comparenormal\savecomparemode
\noexploregroups\saveexploremode
\expandingroups

\endinput

H I S T O R I Q U E
------------------------------------------------------------------------------
v1.0    4/7/2008 : - Package achev?.
7/7/2008 : - Package publi? sur CTAN.
------------------------------------------------------------------------------
v1.1    15/8/2008
- Le package ne n?cessite plus LaTeX et est d?sormais utilisable sous
Plain eTeX.
- Ajout des macros \IfInteger et \IfDecimal.
Pour cette derni?re, la partie enti?re et la partie d?cimale sont
r?cup?rables dans les compteurs \integerpart et \decimalpart. Ce
qu'il reste apr?s qu'un caract?re non attendu soit rencontr? est
dispo dans \xs_remainafterdecimal
- Correction d'un bug dans \tokenize :
suppression de l'expansion avec \normalexpandarg pour ?viter le bug
avec les lettres accentu?es dans l'exemple : \tokenize\aa{??}
- Am?lioration du code de la plupart des macros.
- ?criture d'une routine \xs_newmacro d?finissant les  macros.
- Suppression de tous les compteurs grace ? \numexpr.
- Nouvelles fonctionnalit?s internes dans :
\IfSubStr
ajout des chaines se trouvant avant et apr?s l'occurrence test?e
dans les sc \xs_behind_IfSubStr et \xs_before_IfSubStr
\StrCount
a) ajout de ce qui se trouve apr?s la derni?re occurrence dans la
sc \xs_StrCount_afterlastocccur
b) la macro ne d?pend plus d'aucune autre
------------------------------------------------------------------------------
v1.2    23/8/2008
- Am?lioration du code de \StrMid \StrGobbleLeft, \StrLeft,
\StrGobbleRight et \StrRight ? l'aide de la nouvelle macro
\xs_StrSplit_i
- Nouveau test \IfStrEq qui compare 2 chaines
- Nouveau test \IfEq qui compare 2 chaines (ou 2 nombres si les 2 chaines
contiennent un nombre)
- Correction d'un bug dans \xs_formatnumber. La macro n'envisageait pas le
cas o? son argument ?tait vide ce qui faiasait planter
\IfDecimal{}{V}{F} et \IfInteger{}{V}{F}
------------------------------------------------------------------------------
v1.3    21/9/2008
- Am?lioration du code, mise en place de r?cursivit?s terminales dans
toutes les macros r?cursives, simplification de \xs_TestEqual en
utilisant \ifx
- Nouvelles macros \IfStrEqCase et \IfEqCase
Teste si une cha?ne est ?gale ? plusieurs chaines donn?es et
ex?cute un code sp?cifique
- Cr?ation de la macro publique \StrSplit
Coupe la chaine en 2 ? une position donn?e
- Nouvelle macro \StrCompare
Compare 2 cha?nes et renvoie la position du 1er caract?re diff?rent.
Renvoie 0 si elles sont ?gales.
------------------------------------------------------------------------------
v1.3a   29/9/2008
- Correction d'un bug : \expandafter#1
dans les macros \IfSubStrBefore et \StrBetween qui buggue si #1 est un
nombre > 9 !
- R? ?criture de \xs_returnfirstsyntaxunit et \xs_gobarg qui
deviennent purement d?veloppables.
- R? ?criture de \StrLen
- Nouvelle macro interne \xs_cutafteroccur
Coupe la chaine apr?s la ni?me occurrence d'une sous chaine.
- Code am?lior? de \StrMid, \StrLeft, \StrGobbleLeft, \StrRight,
\StrGobbleRight grace ? \xs_cutafteroccur
------------------------------------------------------------------------------
v1.4   4/11/2008
- xstring traite ses arguments par unit? syntaxique, et donc toutes les
macros internes ont ?t? r?-?crites ? cette fin.
- Le manuel a ?t? r?-?crit, rendu plus clair et mieux structur?.
- Nouvelle fonctionnalit? : \expandarg
le 1er lex?me de chaque argument est 1-d?velopp? avant que la
macro ne soit appel?e. Si un argument comporte plus qu'1 lex?me,
il faut passer par \scancs*[1] pour 1-d?velopper toutes les unit?s
syntaxiques.
- Correction de 2 erreurs dans le manuel anglais :  0 est la valeur par
d?faut dans \StrSubstitute et \StrDel
- Coh?rence dans les nom des s?quences de contr?les temporaires qui
sont d?sormais : \xs_reserved_A ? \xs_reserved_E
------------------------------------------------------------------------------
v1.4a  12/11/2008
- Correction d'un bug dans \xs_StrSplit dans le cas o? l'argument
num?rique est <1 : la 1ere coupure doit ?tre vide et le seconde doit
?tre ?gale ? l'argument.
------------------------------------------------------------------------------
v1.4b  16/11/2008
- Correction de 2 bugs dans \xs_returnfirstsyntaxunit
------------------------------------------------------------------------------
v1.5   31/12/2008
- Nouvelles fonctionnalit?s dans la recherche de groupes par un
identificateur caract?risant leur imbrication. Impl?mentation de :
1) \StrFindGroup
2) \groupID
- Ajout des nouvelles macros g?n?riques \xs_read_reserved_C et
\xs_read_reserved_D
- Correction d'un bug dans \StrSplit : \StrSplit{{a}bc}{1}[\truc] faisait
que \truc contenait ?a{a}?.
- Correction d'un bug dans \xs_newmacro : l'argument optionnel ?tait
d?tok?nis? ? tort dans les macros ?toil?es.
- Dans \xs_newmacro, on doit choisir le num?ro du dernier argument devant
?tre d?tok?nis? dans le cas d'une macro ?toil?e (sachant que
l'argument optionnel ne l'est jamais)
------------------------------------------------------------------------------
v1.5a  09/2/2009
- Nouvelle macro \StrExpand, sensible au mode d'exploration. La macro est
ind?pendante du mode d'exploration et dispose de ses propres commandes
d'exploration : \expandingroups et \noexpandingroups
- R?-?criture de \scancs, qui devient triviale puisque d?pendant de
\StrExpand. Il n'y a plus de version ?toil?e et d?sormais, \scancs
est sensible au mode d'exploration.
- Correction d'un bug dans \IfInteger : \IfInteger{2.0}{V}{F} affichait F
- Correction de bugs : mettre \let\xs_reserved_E\relax avant d'appeler
\xs_StrSplit_i
- Suppression des messages d'erreur, de warning et d'info. xstring devient
donc silencieux ;)
- Passage de 3 ? 2 compteurs
- Le manuel est d?sormais plus color?, en esp?rant qu'il sera un peu
plus agr?able ? lire !
------------------------------------------------------------------------------
v1.5b  13/3/2009
- Modification d'un grand nombre de macros de telle sorte que vraiment
n'importe quel code peut d?sormais ?tre plac? dans les arguments des
macros (comme par exemple des \if, \ifx ou autre, m?me sans leur \fi, ce
qui n'?tait pas possible jusqu'alors)
------------------------------------------------------------------------------
v1.5c  05/6/2009
- Correction d'un bug dans \IfBeginWith : il faut appeler
\xs_returnfirstsyntaxunit pour l'argument #2 puis pour l'argument #1 et
non pas l'inverse pour que \xs_toks refl?te ce qui se trouve dans #1
- Correction d'un bug dans \xs_returnfirstsyntaxunit au cas o? #1 commence
par un espace : mettre \xs_toks ? 0
- Correction d'un bug dans \xs_returnfirstsyntaxunit :
\xs_returnfirstsyntaxunit{{}}\truc
faisait que \truc se d?veloppait en un espace.
- Correction d'un bug dans \xs_removefirstsyntaxunit o? le cas
\xs_removefirstsyntaxunit{ {b}}\truc
donnait \truc se d?veloppant en ?b? au lieu de ?{b}?.
------------------------------------------------------------------------------
v1.5d  28/3/2010
- Correction d'un bug dans \IfInteger : \afterinteger ne donnait pas le
bon r?sultat. Par exemple avec 1.23 il renvoyait {} au lieu de {.23}
- \xs_formatnumber ne detokenize plus ses arguments (que m'est-il pass?
par la t?te pour que je code un truc comme ca ?), et donc
\afterinteger et \xs_afterdecimal ont des tokens ayant le bon
catcode
------------------------------------------------------------------------------
v1.6  24/10/2012
- Correction d'un bug dans \xs_cutafteroccur au cas o? #3<1
- \IfDecimal ne \detokenize plus l'argument.
- Nouvelle version de \tokenize qui enlevait les accolades si son argument
?tait entre accolades
- Nouvelle macro \StrCut
- \xs_cutafteroccur_i ne produit plus d'espace ind?sirable si #3 ?tait
?valu? par \numexpr
------------------------------------------------------------------------------
v1.7  13/1/2013
- Correction d'un manque de rigueur dans les assignations concernant
\groupID : elles sont toutes globales d?sormais
- Les macros de xstring sont \long
------------------------------------------------------------------------------
v1.7a 28/2/2013
- Correction d'un espace parasite dans \xs_removefirstsyntaxunit
------------------------------------------------------------------------------
v1.7b 29/7/2013
- La date contenue dans \xstringdate est d?sormais conforme
------------------------------------------------------------------------------
v1.7c 13/10/2013
- les macros impliqu?es dans \IfStrCase et \IfStrEqCase sont d?sormais \long
------------------------------------------------------------------------------
v1.8  07/12/2018
- affectations globales supprim?es (sauf pour \groupID) afin de ne pas
surcharger la pile de sauvegarde
- nettoyage du code, corrections de lourdeurs et maladresses
------------------------------------------------------------------------------
v1.81 09/12/2018
- bug dans \IfInteger et \IfDecimal, la macro \xs_afterdecimal est ind?finie
et doit ?tre remplac?e par \afterdecimal
------------------------------------------------------------------------------
v1.82 01/02/2019
- \xs_testopt n'est pas longue et provoque un bug dans \xs_IfStrCase et
\xs_IfStrCase lorsque #1 contient \par : \xs_testopt reste courte et
\xs_IfStringCase a ?t? modifi?e pour que cela fonctionne.
------------------------------------------------------------------------------
v1.83 06/02/2019
- mauvaise approche et mauvais fix dans la v1.82 : \xs_testopt devient
longue, pas le choix (et donc aussi \xs_ifnxttok)

